Local Optimization of Quantum Circuits (Extended Version)

Recent advances in quantum architectures and computing have motivated the development of new optimizing compilers for quantum programs or circuits. Even though steady progress has been made, existing quantum optimization techniques remain asymptotically and practically inefficient and are unable to offer guarantees on the quality of the optimization. Because many global quantum circuit optimization problems belong to the complexity class QMA (the quantum analog of NP), it is not clear whether quality and efficiency guarantees can both be achieved. In this paper, we present optimization techniques for quantum programs that can offer both efficiency and quality guarantees. Rather than requiring global optimality, our approach relies on a form of local optimality that requires each and every segment of the circuit to be optimal. We show that the local optimality notion can be attained by a cut-and-meld circuit optimization algorithm. The idea behind the algorithm is to cut a circuit into subcircuits, optimize each subcircuit independently by using a specified "oracle" optimizer, and meld the subcircuits by optimizing across the cuts lazily as needed. We specify the algorithm and prove that it ensures local optimality. To prove efficiency, we show that, under some assumptions, the main optimization phase of the algorithm requires a linear number of calls to the oracle optimizer. We implement and evaluate the local-optimality approach to circuit optimization and compare with the state-of-the-art optimizers. The empirical results show that our cut-and-meld algorithm can outperform existing optimizers significantly, by more than an order of magnitude on average, while also slightly improving optimization quality. These results show that local optimality can be a relatively strong optimization criterion and can be attained efficiently.

==> algorithm.tex <==
In \secref{lang}, we presented a rewriting semantics consisting of just
two rules (corresponding to optimization of a segment and compaction)
%
and
%
proved that any saturating rewrite that applies the two rules to
exhaustion yields a locally optimal circuit.
%
This result immediately suggests an algorithm: simply apply the
rewriting rules until they no longer may be applied, breaking ties
between the two rules arbitrarily.
%
Even though it might seem desirable due to its simplicity, such an
algorithm is not efficient, because searching for a segment to
optimize requires linear time in the size of the circuit (both in
worst and the average case), yielding a quadratic bound for
optimization.
%
For improved efficiency, it is crucial to reduce the search time
needed to find a segment that would benefit from optimization.

Our algorithm, called \algname{}, controls seach time by using a
circuit cutting technique, which has been studied for the purposes of
simulating quantum circuits on classical
hardware~\cite{circuit-cutting-2020,tang-cutqc-2021,bravyi-future-qc-2022}.
%
More specifically, the algorithm cuts the circuit hierarchically into
smaller subcircuits, optimizes each subcircuit independently.
%
The hierarchical cutting naturally reduces the search time for the
optimizations by ensuring that most of the optimizations take place in
the context of small circuits.
%
Because the algorithm optimizes each subcircuit independently, it can
miss crucial optimizations.
%
To compensate for this, the algorithm melds the optimized subcircuits
and optimizes further the melded subcircuits starting with
the \defn{seam}, or the boundary between the two subcircuits.
%
The meld operation guarantees local optimality and does so efficiently
by first optimizing the seam and further optimizing into each
subcircuit only if necessary.
%
By melding locally optimal subcircuits, the algorithm can guarantee
that the subcircuits or any of their ``untouched'' portions (what it
means to be ``untouched'' is relatively complex) remain optimal.
%
We make this intuitive explanation precise by proving that the
algorithm yields a locally optimal circuit.

The efficiency properties of the algorithm are far from obvious.
%
One specific complexity is data dependency: the execution of the
algorithm depends not only on the size of the circuits but the
specific gates in the circuit, and more generally the entire circuit
structure, because optimization themselves depend on the gates, which
in turn impact the run time of the algorithm.
%
We show that it is possible to account for this data dependency by
using a combination of cost-sensitive analysis and amortization
techniques.
%
Specifically, our bound amortizes optimization costs against the cost
improvement, defined as the difference between input and output costs.
%
Note that in cases where optimization concerns total gate count or the
count of certain gates (e.g., T gates or CNOT gates), the cost
improvement is upper bounded by the circuit size.




% In the rest of the section, we present our algorithm, prove that it always returns a locally optimal
% circuit, and analyze its efficiency.
% %
% \figref{lopt-code} shows the pseudocode the  \algname{}
% algorithm and its key subroutines.
% %
% We describe the \emph{meld} operation in \secref{algorithm::meld}, and prove its
% efficiency.
% %
% Then, in \secref{algorithm::soam}, we prove the efficiency of optimization phases.
% %
% Finally, in \secref{algorithm::lopt}, we prove the efficiency.
% %
% \todo{Update for new subsection structure in this section which changed recently}
%
% In \secref{algorithm::soam}, we describe \coam{}, and in
% \secref{algorithm::correctness} we prove that the \algname{} algorithm
% guarantees that the output is correct (locally optimal and equivalent to
% the input).
% %
% In \secref{algorithm::cost-analysis} we analyze cost and prove that \algname{}
% requires nearly linear time.
% %

% \todo{how is the cost assumption different than the semavtics?  Pull up top.}t

% The algorithm is parameterized by a cost function $\cost$, an oracle optimizer
% $\oracle$, and a segment span $\Omega$.
% %
% The algorithm works for cost functions that are additive under circuit
% concatenation, i.e., the cost of a circuit obtained by concatenating
% two circuits is equal to the sum of costs of the individual circuits
% (Definition~\ref{def:additive-cost}).
% %
% In particular, we note that the algorithm can guarantee local optimality for a variety of
% gate count metrics, such as total number
% of gates, or gates of a particular kind (e.g., T-gates).


% \subsection{The utility of larger windows}

% A key idea used by our algorithm is that the \oracle{} can be applied to segments that
% are a constant fraction longer than $\Omega$ to effectively optimize many $\Omega$-segments
% all at the same time.
% %
% In particular, in our algorithms in this section, we will apply the \oracle{} to segments of
% length at most $2\Omega$; from this, we desire the guarantee that the output is \emph{segment optimal},
% i.e., that every $\Omega$-segment of the output is optimal.
% %
% To prove this, we require the following assumption on the oracle.
% %
% \[
%   \costof{\oracle{}(C_1 ; C_2)} \leq \costof{\oracle{}(C_1)} + \costof{\oracle{}(C_2)}
% \]
% %
% Intuitively, this assumption states that \textbf{with more input, the oracle should
% only be able to do better}, which is a desirable property of any optimizer.
% %
% With this assumption in hand, we can then prove \lemref{suboptimize}.

% \begin{lemma}\label{lem:suboptimize}
% For any $C' = \oracle{}(C)$, if $\costof{C'} = \costof{C}$ then $\windowopt\Omega{C}$.
% \end{lemma}
% \begin{proof}
% Consider any $(P ; X ; S) = C$ where $\mathsf{length}(X) \leq \Omega$.
% %
% It suffices to show $\costof{\oracle{}(X)} = \costof X$.
% %
% \todo{This can be done inductively... it uses additivity, monotonicity (compatibility),
% and the assumption on the oracle}
% \end{proof}



\subsection{The algorithm}
\label{sec:opt-phase}

\input{fig/fig-opt}


\figref{lopt-code} shows the pseudo-code for our algorithm.
%
The algorithm (\lstinline{OAC}) organizes the computation into rounds,
where each round corresponds to a recursive invocation
of \lstinline{OAC}.
%
A round consists of a compaction phase (via function \lstinline{compact})
%
and
%
a segment-optimization phase, via function \lstinline{segopt}.
%
The rounds repeat until convergence, i.e., until no more optimization
is possible (at which point the final circuit is guaranteed to
be \emph{locally optimal}).
%
As the terminology suggests, the segment optimization phase always
yields a segment-optimal circuit, where each and every segment is
optimal (as defined by our rewriting semantics).
%
Compaction rounds ensure that the algorithm does not miss optimization
opportunities that arise due to compaction.
%
%% Our experiments show that the number of rounds is quite small, even
%% for large circuits, and the vast majority of all optimizations are
%% performed in the first round.
%% %
%% We specifically observe that the number of rounds does not exceed $3$ in the majority of cases, and does not exceed $11$
%% across all of our benchmarks.
%% %
We also present a relaxed version of our algorithm that stops early
when a user-specified \defn{convergence threshold}
$0 \leq \epsilon \leq 1$, is reached.
%




\myparagraph{Function \textsf{segopt}.}
The function \textsf{segopt} takes a circuit $C$ and produces
a segment optimal output.
%
To achieve this, it uses a divide-and-conquer strategy to cut the
circuit hierarchically into smaller and smaller circuits:
%
it splits the circuit into the
subcircuits $C_1$ and $C_2$, optimizes each recursively, and then
calls \textsf{meld} on the resulting circuits to join them back
together without losing segment optimality.
%
This recursive splitting continues until the circuit has been partitioned into
sufficiently small segments,
specifically where each piece is at most $2\Omega$ in length.
%
For such small segments, the function directly uses the oracle
and obtains optimal segments.

\myparagraph{Function \textsf{meld}.}
\figref{lopt-code} presents the pseudocode of the meld function.
%
The function takes segment-optimal inputs $C_1$ and $C_2$
and returns a segment-optimal circuit that is
functionally equivalent to the concatenation of the input circuits.
%

Given that the inputs $C_1$ and $C_2$ are segment optimal,
all $\Omega$-segments that lie completely within $C_1$ or $C_2$
are already optimal.
%
Therefore, the function only considers and optimizes
``boundary segments''
which have some layers from circuit $C_1$ and other layers from circuit $C_2$.
%

To optimize segments at the boundary,
the function creates a ``super segment'', named $W$,
by concatenating the last $\Omega$ layers of circuit $C_1$
with the first $\Omega$ layers of circuit $C_2$.
%
The function denotes this concatenation as
$C_1[d_1 - \Omega : d_1] + C_2[0 : \Omega]$ (see \lineref{combine}).
% where $C_1[d_1 - \Omega : d_1]$ represents the last $\Omega$ layers of circuit $C_1$
% and $C_2[0 : \Omega]$ represents the first $\Omega$ layers of circuit $C_2$.
The meld function calls the oracle on $W$
and retrieves the $W'$,
which is guaranteed to be segment-optimal because
its returned by the oracle.
%
The meld function then considers the costs of $W$ and $W'$.

%
If the costs of $W$ and $W'$ are identical, then $W$ is already
segment optimal.  Consequently, all $\Omega$-segments at the boundary
of $C_1$ and $C_2$ are also optimal.
%
The key point is that the ``super segment'' $W$ encompasses
all possible $\Omega$-segments at the boundary of $C_1$ and $C_2$.
%
To see this,
let's choose an $\Omega$-segment at boundary,
which takes the last $i > 0$ layers of circuit $C_1$
and the first $j > 0$ layers from of circuit $C_2$;
we can write this as $C_1[d_1 - i : d_1] + C_2[0 : j]$,
where $d_1$ is the number of layers in $C_1$.
%
Given that this is an $\Omega-$segment and has $i + j$ layers,
we get that $i + j = \Omega$ and $i < \Omega$ and $j < \Omega$.
%
Now observe that our chosen segment $C_1[d_1 - i : d_1] + C_2[0 : j]$
is contained within the super segment $W = C_1[d_1 - \Omega : d_1] + C_2[0 : \Omega]$ (\lineref{combine}),
because $i < \Omega$ and $j < \Omega$.
%
Given that $W$ is segment optimal, our chosen segment is also optimal (relative to the oracle).


Returning to the \textsf{meld} algorithm,
consider the case where
the segment $W'$ improves upon the segment $W$.
In this case, meld incorporates $W'$ into the circuit
and propagates this change to the neighboring layers.
%
To do this, meld works with three segment optimal circuits:
circuit $C_1[0 : d_1 - \Omega]$,
which contains the first $d_1 - \Omega$ layers of circuit $C_1$,
is segment optimal because $C_1$ is segment optimal;
%
the circuit $W'$ is segment optimal because it was returned by the oracle;
%
and the circuit $C_2[\Omega: d_2]$,
which contains the last $d_2 - \Omega$ layers of circuit $C_2$,
is segment optimal because $C_2$ is segment optimal.
%
Thus, we propagate the changes of window $W'$,
by recursively melding these segment optimal circuits.

In \figref{lopt-code},
the function meld first melds the remaining layers of circuit $C_1$ with the segment $W'$,
obtaining circuit $M$ (see \lineref{mrec}),
and then melds the circuit $M$ with the remaining layers of $C_2$.
%
%
Note that both recursive calls satisfy the precondition
that inputs to meld are segment optimal.
%
We now formalize the above intuition by proving,
in \lemref{meld-is-optimal}, that the meld algorithm
produces a segment optimal output if the inputs are segment optimal.


\myparagraph{Segment Optimal Outputs.}
We prove that our \textsf{segopt} and \textsf{meld}
algorithms produce segment optimal circuits.
%
The challenge here is proving that
\textsf{meld} produces segment optimal outputs even though it may decide not to optimize one or both of the subcircuits based on the outcome of an optimization.
% %
%Once we establish the segment optimality of meld,
%the proof that \textsf{segopt} produces segment optimal outputs
%is straightforward.

\begin{lem}[Segment optimality of meld]
  \label{lem:meld-is-optimal}
  Given any additive \cost{} function and any segment optimal circuits
  $C_1$ and $C_2$, the result of \lstinline{meld}$(C_1, C_2)$ is a
  segment optimal circuit $C$ and $\costof{C} \leq \costof{C_1} + \costof{C_2}$.
\end{lem}

\begin{proof}

  We show the lemma by induction on the total cost of the input, i.e.,
  $\costof {C_1} + \costof{C_2}$.
  %
  In the base case, the input cost is zero, and therefore all segments of
  the input circuits have zero cost, due to additivity of the \cost{} function.
  %
  The output of meld in this case is the concatenation $(C_1; C_2)$,
  because the oracle can not improve the boundary segment $W$.
  %
  For the inductive step,
  we consider two cases, depending on whether the oracle optimizes the boundary segment $W$.

  \paragraph{Case I}
  When the oracle finds no improvement in $W$, the output is the concatenation $C = (C_1; C_2)$.
  %
  % In this case, the output cost is $\costof{C_1} + \costof{C_2}$ because
  % our cost function is additive w.r.t. concatenation.
  %
  To prove that the output $C$ is segment optimal,
  we show that every $\Omega$-segment of the output is optimal relative to
  the oracle.
  %
  For any such $\Omega$-segment $X$, there are two cases.
  %
  \begin{itemize}
  \item If $X$ is a segment of either $C_1$ or $C_2$, then $X$ is optimal relative to the oracle
  because the input circuits are segment optimal and $X$ is of length $\Omega$.

  \item If $X$ is not a segment of either $C_1$ or $C_2$, then $X$ is a sub-segment of $W$,
  because the segment $W$ has length $2\Omega$ and contains all possible $\Omega$-segments at the boundary of $C_1$
  and $C_2$. Because the oracle could not improve segment $W$, it can not improve its sub-segment $X$.
  \end{itemize}

  Thus, all $\Omega$-segments of the output are optimal relative to the oracle,
  and the output is segment optimal.

  \paragraph{Case II}
  If the oracle improves the boundary segment $W$,
  then the cost of the optimized segment $W'$ is less than cost of segment $W$, i.e.,
  $\costof{W'} < \costof{W}$.
  %
  In this case, the function first melds the segment $C_1[0 : d_1 - \Omega]$ and the segment $W'$,
  by making a recursive call.
  %
  We apply induction on the costs of the inputs to prove that the output circuit $M$ is segment optimal.
  %
  Formally, we have the cost of inputs
  $\costof{C_1[0 : d_1 - \Omega]} + \costof{W'} < \costof{C_1[0 : d_1 - \Omega]} + \costof{W} \leq \costof{C_1} + \costof{C_2}$,
  because $W'$ has a lower cost than $W$.
  %
  Therefore, by induction, the output $M$ is segment optimal
  and $\costof{M} \leq \costof{C_1[0 : d_1 - \Omega]} + \costof{W'}$.
  % Therefore, by induction, the first recursive call
  % to \lstinline{meld} returns an segment optimal output of size at most
  %

  For the second recursive call $\mathsf{meld}(M, C_2[\Omega : d_2])$,
  we can apply induction because $\costof{M} + \costof{C_2[\Omega : d_2]} < \costof{C_1} + \costof{C_2}$.
  %
  This inequality follows from the cost bound on circuit $M$ above and using that
  $W'$ has a lower cost than $W$.
  %
  Specifically,
  $\costof{M} + \costof{C_2[\Omega : d_2]} \leq \costof{C_1[0 : d_1 - \Omega]} + \costof{W'} + \costof{C_2[\Omega : d_2]}$,
   which is strictly less than
    $\costof{C_1[0 : d_1 - \Omega]} + \costof{W} + \costof{C_2[\Omega : d_2]} = \costof{C_1} + \costof{C_2}$.
  %
  Therefore, by induction on the second recursive call,
  we get that meld returns a segment optimal circuit
  that is bounded in cost by $\costof{C_1} + \costof{C_2}$.
  %
  Note that for both recursive calls, the induction relies on the fact that $W'$ has a lower cost than $W$,
  showing that the algorithm works because the recursion is tied to cost improvement.
  %
\end{proof}

Based on \lemref{meld-is-optimal}, we can show the following theorem.
We leave the proof to
\iffull
\appref{thm-opt}.
\else
the Appendix.
\fi
%We now prove that the hierarchical segment optimization via the
%divide-and-conquer technique always yields a segment optimal circuit.

\begin{theorem}[Segment optimality algorithm] \label{thm:opt}
  For any circuit $C$, the function $\mathsf{segopt}(C)$ outputs
  a segment optimal circuit.
  \end{theorem}


\subsection{Efficiency of segment optimality}
\label{sec:opt-analysis}

% TODO: We can implement the semantics as follows.  We scan the circuit to find a segment that can be optimized, optimize it, and repeat until convergence.  this algorithm can require at least quadratic time, because scanning the circuit takes linear time, and each optimization can reduce as little as a single gate.
% In quadratic time, we can also do compression, by compressing after each optimization.  We want to improve on this, reaching ideally linear time.  To this end, we propose an algorithm that operates in rounds.  In each round, the algorithm only applies optimization rules, and in between rounds it compresses the entire circuit.

% TODO: Highlight the "search" part of the rule: we have to find where to apply

% TODO: add the CircuitCompression algorithm
% idea: take a circuit and construct a new one by incrementally addiing each gate

% In this section,
% we describe our local optimization algorithm \algname{},
% which takes a circuit finds an locally optimal equivalent circuit.
% %
% The local optimality is parameterized by a cost function $\cost$,
% an oracle optimizer $\oracle$, and a segment span $\Omega$.
% %
% Our algorithm assumes these parameters
% and uses the oracle to optimize $(2*\Omega)$-segments of the given
% circuit w.r.t. the cost function.
% %
% The algorithm proceeds in rounds
% and in one round,
% it uses a subroutine called \coam{} to perform local optimizations
% and \emph{compresses} the circuit to fill any gaps that may be created
% due to optimizations.
% %
% The algorithm repeats until no more optimizations can be found
% and at the end,
% it guarantees that the circuit is locally optimal.


% The runtime of the algorithm


% The algorithm works for cost functions that are additive under circuit
% concatenation, i.e., the cost of a circuit obtained by concatenating
% two circuits is equal to the sum of costs of the individual circuits
% (Definition~\ref{def:additive-cost}).
% %
% In particular, the \coam{} algorithm can guarantee (relative) local
% optimality for a variety of gate count metrics, such as total number
% of gates, or gates of a particular kind (e.g., T-gates).
% %



% This section presents an algorithm, called \coam{}, that ensures
% local optimality for a certain class of cost functions.
% %
% The algorithm is parameterized by an \defn{oracle} optimizer that it
% uses to optimize $\Omega$-segments (subcircuits with at most $2\Omega$
% depth).
% %

% One way to guarantee (relative) local optimality is to proceed iteratively.
% %
% At each step, we find a segment of the circuit that is not optimal and
% optimize it by calling the oracle, and repeat until convergence.
% %
% Even though this approach is relatively simple, it would require
% significant time, because each iteration scans the whole
% circuit to find the next segment to optimize.
% %
% Our \coam{} algorithm achieves asymptotically better runtime
% by carefully propagating optimizations.

Having shown that the functions \textsf{segopt} and \textsf{meld}
produce segment optimal outputs,
we now analyze the runtime efficiency of these functions.
%
The runtime efficiency of both functions is data-dependent and varies with the number of optimizations found throughout the circuit.
%
To account for this,
we charge the running time to the cost improvement between the input and the output,
represented by $\Delta$.
%
We prove the following theorem.


\begin{theorem}[Efficiency of segment optimization] \label{thm:cost}
  % Consider a segment length $\Omega$, an oracle that optimizes for the cost function $\mathbf{cost}$,
  % and a circuit $C$.
  The function $\mathsf{segopt}(C)$ calls the oracle at most
  $\mathsf{length}(C) + 2\Delta$ times on segments of length at most $2\Omega$,
  where $\Delta$ is the improvement in the cost of the output.
  \end{theorem}

The theorem shows that our segment optimality algorithm is productive in its use of the oracle.
%
Consider the terms, $\mathsf{length}(C)$ and $2\Delta$, in the bound on the number of oracle calls:
%
The first term, $\mathsf{length}(C)$, is for checking segment
optimality---even if the input circuit is already optimal,
the algorithm needs to call the oracle on each segment and confirm it.
%
The second term $2\Delta$,
shows that all further calls result from optimizations,
with each optimization requiring up to two oracle calls in the worst case.
%
This shows that our algorithm (alongside meld)
carefully tracks the segments on which the oracle needs to be called
and avoids unnecessary calls.


The theorem also highlights one of the key features of our $\mathsf{segopt}$ function:
it only uses the oracle on small circuit segments of length $2\Omega$.
%
Suppose $q$ is the number of qubits in the circuit.
%
Then the $\mathsf{segopt}$ function only calls the oracle on
manageable circuits of size less than or equal to $q * 2\Omega$,
which is significantly smaller than circuit size.
%
This has performance impacts because, for many oracles,
it is faster to invoke the oracle many times on small circuits
rather than invoking the oracle a single time on the full circuit (see \secref{eval}).
%

Since we bound number of oracle calls in terms of the cost improvement $\Delta$,
an interesting question is how large can $\Delta$ be?
%
When optimizing for gate-counting metrics
such as $\mathsf{T}$ count (number of $\mathsf{T}$ gates), $\mathsf{CNOT}$ count (number of $\mathsf{CNOT}$ gates),
gate count (total number of gates),
the cost improvement is trivially bounded by the circuit size,
i.e., $\Delta \leq \sizeof{C}$.
%
This observation shows that our \textsf{segopt}
function only makes a linear number of calls (with depth and gate count)
to the oracle.


\begin{corollary}[Linear calls to the oracle]
  When optimizing for gate count, our $\mathsf{segopt}(C)$ makes a linear,
  $O(\mathsf{length}(C) + \sizeof{C})$, number of calls to the oracle.
\label{cor:linear-calls}
\end{corollary}

We experimentally validate this corollary in \secref{eval-calls},
where we study the number of oracle calls made by our algorithm
for many circuits.
The crux of the proofs of \thmref{cost} and the corollary 
is bounding the number of calls in the \textsf{meld} function,
because it can propagate optimizations through the circuit.
%
We state bound below and leave the proofs to 
\iffull
\appref{thm-meld-num-oracles}.
\else
the Appendix.
\fi
%



% \begin{corollary}
%   Given an optimizer that takes $T(q, \sizeof{C})$ time on a circuit $C$ with $q$ qubits and size \sizeof{C},
%   computing $C' = \mathsf{segopt}(C)$ requires at most $O(T(q, \sizeof{C}) * (\mathsf{length}(C) + \Delta))$ time,
%   where $\Delta = \costof{C} - \costof{C'}$ is the improvement in cost.
% \end{corollary}

% \begin{corollary}
%   Given an optimizer that takes $T(q, \mathsf{length}(C))$ time on a circuit $C$ with $q$ qubits,
%   computing $C' = \mathsf{segopt}(C)$ takes $O((\mathsf{length}(C) + 2\Delta) * T (q, 2\Omega))$ time
% \label{cor:linear-calls}
% \end{corollary}

% The corollary demonstrates that when optimizing for gate count,
% our \textsf{segopt} function scales linearly with both the number of gates and the length/depth
% of the circuit.
% %
% Furthermore, our \textsf{segopt} function and the oracle
% exhibit similar scaling behavior in the number of qubits.


% The corollary shows that when optimizing for gate count,
% our \textsf{segopt} function scales linearly
% with the number of gates and depth of the circuit.
% %
% Both the oracle and our \textsf{segopt} function scale similarly with the number of qubits.

% %


\begin{lem}[Bounded calls to oracle in meld]
  \label{lem:meld-num-oracles}
Computing $C =$ \lstinline{meld}$(C_1, C_2)$
makes at most $1 + 2\Delta$ calls to the oracle,
where $\Delta$ is the improvement in cost,
i.e., $\Delta = \left(\costof {C_1} + \costof{C_2} - \costof{C}\right)$.
\end{lem}




  %

% The meld function and its running time are data dependent,
% as the function decides to make the two recursive calls
% depending on the output of the oracle.
% %
% The recursion tree for a single meld call can be deep,
% as the melding may continue if the oracle continues to find optimizations,
% possibly calling the oracle on segments from  the whole circuit.
% %
% But, because the algorithm recurses only if the oracle finds an optimization,
% we can charge the cost of recursion to the optimization.
% %
% This is formalized in \lemref{meld-num-oracles}.





% ?

% \paragraph{Meld Example.}
% Returning to the example in \figref{propagate},
% we can see the algorithm in action.
% %
% The example we uses $\Omega = 2$ and gate count as the cost function.
% %
% In the first step,
% the function optimizes the $2\Omega-$segment at the boundary of inputs;
% this corresponds to optimizing the $4-$segment in the figure and reducing the gate count.
% %
% Then, the function melds the preceding layers of circuit $C_1$ with the window $W'$,
% corresponding to the second step in \figref{propagate},
% which propagates the optimization
% by considering both the old and new CNot gates.
% %
% Finally, the function melds the remaining layers of $C_2$,
% which corresponds to the third step in \figref{propagate},
% which merges the rotation gates.
%


% \subsection{SOAM Algorithm}

% \figref{lopt-code} presents the pseudocode of the \coam{} algorithm.
% %
% %
% The function $\mathsf{SOAM}$ takes a circuit $C$ and
% returns an segment optimal circuit, where the segment optimality is relative to the oracle.
% %
% To do so,
% the function checks if the circuit is small,
% i.e., its its depth is less than $2\Omega$.
% %
% In this case, the function sends the circuit to the oracle,
% and returns the output of the oracle, which is segment optimal by definition.
% %
% For larger circuits, the function
% $\mathsf{SOAM}$ splits the circuit into two halves
% $C_1$ and $C_2$, and recursively optimizes the two halves,
% retrieving the segment optimal versions $C'_1$ and $C'_2$.
% %
% Then it calls the function $\mathsf{meld}$ which stitches $C'_1$ and $C'_2$
% to produce the segment optimal output circuit.
% %

% We prove that $\mathsf{segopt}(C)$ produces an segment optimal output
% and does so in a bounded number of oracle queries,
% where each query is for small segments, i.e.,
% segments whose length is bounded by $2\Omega$.
% %


% \todo{exponential oracle can be viewed as oversell.  use quadratic. }
% \todo{do not use "huge" in writing to prevent oversell reaction.}
% The corollary shows that the $\mathsf{segopt}$ function can have asymptotic benefits
% for gate count (or T-count) optimization.
% %
% For example, suppose the oracle complexity is exponential in the number of qubits and circuit length,
% i.e., suppose $T(q, d) = O(2 ^ {qd})$.
% %
% Then, using the above corollary,
% the time complexity of the $\mathsf{segopt}$ function is $O(2 ^{2q\Omega}\sizeof{C})$,
% which is bounded by $O(2 ^{2q\Omega}qd)$ (using $\sizeof{C} \leq qd$).
% %
% In this example,
% the base complexity $T(q, d)$ is exponential in circuit length $d$,
% but the $\mathsf{segopt}$ function is effectively linear in the length,
% which is a huge reduction.
% %
% More generally, we can derive a meaningful reduction in complexity if the oracle
% has at least quadratic (in length) time complexity,
% because the $\mathsf{segopt}$ function only sends a linear number of fixed-length circuits to the oracle.
% %
% % This efficiency, however, comes at a potential cost to circuit quality,
% % because the $\mathsf{segopt}$ function guarantees segment optimality whereas
% % the base optimizer can work on the whole circuit and, in principle, find more optimizations.
% % %
% % Our experiments, however, suggest that this potential cost does not show up in practice (\secref{eval}).
% %

% \footnote{We can derive a meaningful, but less pronounced reduction in complexity even when the oracle has quadratic cost}.


% As another corollary of the above theorems,
% we get that if we have an optimizer that returns globally optimal circuits,
% then the $\mathsf{segopt}$ function can produce circuits that are segment optimal
% in an absolute sense,
% i.e., every $\Omega-$segment of the output is globally optimal.

% \begin{corollary}
% Given an oracle that produces optimal circuits,
% the $\mathsf{segopt}$ function produces segment optimal circuits using the oracle
% only on segments of size $2\Omega$.
% \end{corollary}


%\subsection{Putting the pieces together: the \algname{} algorithm}
%\label{sec:full-algorithm}
%

The \algname{} algorithm
uses the segment optimality guarantee, given by \textsf{segopt},
to produce a locally optimal circuit.
%
In \figref{lopt-code}, the function \algname{} takes the input circuit $C$
and computes the circuit $C' = \mathsf{segopt}(\mathsf{compact}(C))$.
%
It then checks if $C'$ differs from the input $C$ and if so,
it recurses on $C'$.
% It then checks if $C'$ differs from the input $C$.
% %
% If $C'$ differs from $C$---which could be due to optimization, or compaction, or
% both---then \algname{} continues recursively on $C'$.
% %
% Otherwise, if $C'$ and $C$ are identical,
% it returns the circuit $C'$ because no optimization or compaction occured.
The function repeats this until convergence, i.e.,
until the circuit does not change.
%
In the process, it
computes a sequence of segment optimal circuits $\{C_i\}_{1 \leq i \leq \kappa}$,
where $\kappa$ is the number of rounds until convergence:
\[C \to C_1 \to C_2 \to \ldots \to C_\kappa \quad\text{where}\quad
\begin{array}{c}
\costof{C_i} > \costof{C_{i+1}} \\
\windowopt\Omega{C_i} \\
\locallyopt{\Omega}{C_\kappa}
\end{array}
\]
%
Each intermediate circuit $C_i$ is segment optimal
and gets compacted before optimization in the next round.
%
Given that \algname{} continues until convergence,
the final circuit, $C_\kappa$, is locally optimal.

% This argument subtly hinges upon a property of our segment optimality algorithm, in particular,
% that $\mathsf{segopt}(C)$ differs from $C$ only if the cost has improved.
% %
% The function $\mathsf{segopt}$ and its key subroutine, meld, are careful to ensure this
% by guarding the oracle calls:
% %
% if applying the oracle does not improve the cost, then the output of the oracle is discarded
% (see lines \ref{line:guard1start}-\ref{line:guard1stop} and \ref{line:guard2start}-\ref{line:guard2stop}
% in \figref{lopt-code}).
% %
% (This aligns with the rewriting semantics of \secref{lang}, which only performs optimization
% rewrites if the cost decreases.)
% %

Using \thmref{cost},
we observe that the number of oracle calls in each round is bounded by
$\mathsf{length}(C_i) + 2\Delta_i$,
where $\Delta_i$ is the improvement in cost (i.e., $\Delta_i = \costof{C_i} - \costof{C_{i+1}}$).
%
Thus, the total number of oracle calls performed by \algname{} can be bounded by
$O(\Delta + \mathsf{length}(C) + \sum_{1 \leq i \leq \kappa} \mathsf{length}(C_i))$
where $\Delta = \costof{C} - \costof{C_\kappa}$ is the overall improvement in cost between the input and output.

\begin{theorem}
\label{thm:local-opt}
Given an additive cost function,
the output of $\algname{}(C)$ is locally optimal
and requires $O(\Delta + \mathsf{length}(C) + \sum_{1 \leq i \leq \kappa} \mathsf{length}(C_i))$ oracle calls,
where $C_i$ denotes the circuit after $i$ rounds,
$\kappa$ is the number of rounds,
and $\Delta$ is the end-to-end cost improvement.
\end{theorem}


The bound on the number of oracle calls in \thmref{local-opt} is very general
because it applies to any oracle (and gate set).
%
For particular cost functions, we can use it to deduce a more precise bound.
%
Specifically, in the case of gate count, where
$\costof C = \sizeof C$, we get the following bound.

\begin{corollary}\label{cor:oac-linear-calls}
When optimizing for gate count,
$\algname{}(C)$ performs at most $O(\sizeof{C} + \kappa \cdot \mathsf{length}(C))$ oracle calls.
\end{corollary}

An interesting question is whether or not it is possible to bound the number of rounds, $\kappa$.
%
In general, this will depend on a number of factors,
such as the quality of the oracle and how quickly the optimizations it performs converge
across compactions.
%
In practice (\secref{eval}), we find that the number of rounds required is small, and that
nearly all optimizations are performed in the first round itself.
%
For gate count optimizations in particular, Corollary~\ref{cor:oac-linear-calls} tells us
that when only a small number of rounds are required, the scalability of \algname{} is
effectively linear in circuit size.

%
\begin{wrapfigure}{r}{0.33\textwidth}
\definecolor{mPurple}{rgb}{0.58,0,0.82}
\lstset{
  basicstyle=\footnotesize\fontfamily{ttfamily}\selectfont, % set the font
  keywordstyle={\color{mPurple}}, % set the keyword style
  morecomment=[l]{//},
  commentstyle=\rmfamily\slshape,
  % commentstyle=\itshape, % set the comment style
  showstringspaces=false, % don't show spaces in strings
  columns=fullflexible, % use proportional spacing
  morekeywords={fun,func,let,val,in,end,case,of,SOME, NONE, and, structure, if, or, else, then, return, def}, % define additional keywords
  mathescape=true, % enable math mode
  escapechar={@},
  keepspaces=true,
  breaklines=true,
  numbers=none,
  numbersep=0pt,
  xleftmargin=0em}
\begin{lstlisting}
def $\mathsf{\algname{}}^*(f, C)$:
  $C'$ = segopt(compact$(C)$)
  if $1 - \frac{\costof{C'}}{\costof{C}} \leq f$:
    return $C'$
  else:
    return $\mathsf{\algname{}}^*(f, C')$
\end{lstlisting}
\caption{$\algname{}^*$ terminates when
the cost improvement ratio falls below the \emph{convergence threshold}, $f$.}
\label{fig:oac-star}
\end{wrapfigure}
%
\subsection{\algname{}*: controlling convergence}
\label{sec:convergence-thresh}
%
We observe that, except for the very last round,
each round of our \algname{} algorithm improves the cost of the circuit.
%
This raises a practical question: how does the
improvement in cost vary across rounds?
%
For the vast majority of our evaluation,
we observed that nearly all optimization (> 99\%) occur in the
first round itself (see \secref{converge});
the subsequent rounds have a small impact on the quality.
% which suggests that local optimality and segment optimality are quite similar
% in practice.
%
Based on this observation,
we propose $\mathsf{\algname{}}^*$ which uses a
convergence threshold $0 \leq \epsilon \leq 1$
to provide control over how quickly the algorithm converges.
%

The $\algname{}^*$ algorithm, in \figref{oac-star},
terminates as soon as the cost is reduced
by a smaller fraction than $f$.
%
For example, if we measure cost as the number of gates and $\epsilon = 0.01$,
then $\algname{}^*$ will terminate as soon as an
optimization round removes fewer than $1\%$ of the remaining gates.
%
Note that $\algname{}^*$ gives two guarantees:
1) the output circuit is segment optimal,
and 2) the fractional cost improvement in the last round is less than $\epsilon$.
%
%
In addition, setting $\epsilon = 0$
results in identical behavior to \algname{} and guarantees local optimality.


\if 0
\input{fig/fig_quadratic_lower_bound}

\subsection{Worst-case number of rounds for \algname{}}
%
Fig.~\ref{fig:quadratic_lower_bound} gives an example showing that a linear number of compactions is necessary in the worst case.
%
The example uses $\Omega=3$.
%
We optimize the solid green segment from (a) to (b) by canceling the two CNOTs.
%
However, at (b), no more optimization can be applied.
%
Although the dashed green segment is not optimal, the two CNOTs are separated enough so that we cannot optimize them.
%
So, we must apply a compaction step to bring the two CNOTs together and then optimize them, as shown in (c).
%
This pattern will continue and can require a number of compactions proportional to the number of qubits.
\fi
% \myparagraph{Linear cost.}
% %
% The algorithm runs in time linear to the size of the circuit,
% including the cost of $\mathsf{meld}$.
% %
% We prove this by counting the number of calls to the oracle.
% %
% All other operations (e.g., \lstinline{split} and \lstinline{concat})
% take $O(1)$ time and there are a constant number of such operations per
% call to the oracle.




% \myparagraph{Oracle complexity.}
% We assume that the oracle takes constant time to optimize its input
% as long as the size of the input is bounded by $2n\Omega$,
% where $n$ is the number of qubits.
% %
% In this model,
% the cost of an algorithm is the number of oracle calls.
% %
% For example,
% the following algorithm verifies segment optimality in linear (in size) number of calls to the oracle:
% the algorithm sends all $\Omega-$segments to the oracle; if the oracle can not improve any of them,
% then the circuit is segment optimal and otherwise, the circuit is not segment optimal.
% %
% This algorithm makes only $(d - \Omega + 1)$ number of calls to the oracle.

% Our goal is to design an algorithm
% that produces segment optimal circuits
% by only making a linear number of calls to the oracle.
% %
% Each call to the oracle may improve a segment by reducing an abstract cost.
% %
% Our algorithm works for the following cost functions.

% We prove that for any circuit $C$, the output
% of $\mathsf{SOAM}(C)$ is segment optimal.
% %
% We start by establishing the key lemma, which shows
% that \lstinline{meld} preserves segment optimality.

% For two circuits $C_1$ and $C_2$,
% the number of times the function $\mathsf{meld}$ invokes
% the oracle is bounded by $1 + \sizeof {C_1} + \sizeof{C_2} - \sizeof {C}$


% \begin{proof}
% We can prove this by induction on the sum $\sizeof{C_1} + \sizeof{C_2}$.
% %
% The function $\mathsf{meld}$ first partitions the circuits $C_1$ and $C_2$
% into three parts: $P$, $W$, and $S$,
% where $P$ is the prefix of circuit $C_1$,
% $W$ is the segment crossing the boundary of $C_1$ and $C_2$,
% and $S$ is the suffix of circuit $C_2$.
% %
% We have $\sizeof{P} + \sizeof{W} + \sizeof{S} = \sizeof{C_1} + \sizeof{C_2}$.
% %
% The function then invokes the oracle on segment $W$.
% %
% If the oracle does not improve the size of the segment,
% the function just returns,
% thereby only making the one call to the oracle and satisfying the lemma.

% When the oracle optimizes the segment and returns $W'$,
% we have that $\sizeof{W'} < \sizeof {W}$.
% %
% From the above equality, we get,
% $\sizeof{P} + \sizeof {W'}  + \sizeof{S} < \sizeof {C_1} + \sizeof {C_2}$.
% %
% In this case,
% the function makes two recursive calls.
% %
% The first call melds the prefix $P$ and the segment $W$.
% %
% Because $\sizeof {P} + \sizeof{W} < \sizeof{C_1} + \sizeof{C_2}$,
% we apply the inductive hypothesis to prove that the first
% call to $\mathsf{meld}$ makes $O(\sizeof {P} + \sizeof{W})$ calls
% to the oracle, which is bounded by $O(\sizeof{C_1} + \sizeof{C_2})$.
% %
% The second call to melds the output of the first call with the suffix $S$.
% %
% Note that the output of meld is never larger than the sum of inputs.
% %
% Thus, the cumulative size of inputs to the second call is bounded by
% $\sizeof{P} + \sizeof {W'}  + \sizeof{S}$.
% %
% Because $\sizeof{P} + \sizeof {W'}  + \sizeof{S} < \sizeof{C_1} + \sizeof{C_2}$,
% we apply the inductive hypothesis to prove that the second call to $\mathsf{meld}$
% makes $O(\sizeof{C_1} + \sizeof{C_2})$ calls to the oracle.
% %
% Because both recursive calls only make $O(\sizeof{C_1} + \sizeof{C_2})$ calls to the oracle,
% the total number of calls is also $O(\sizeof{C_1} + \sizeof{C_2})$.
% \end{proof}
% %

% \begin{lem}[Bounded calls to oracle by SOAM]
% \label{lem:optimize-num-oracles}
%   Computing $C' = \mathsf{SOAM}(C)$ makes at most
%   $\sizeof{C} + 2 * (\costof{C} - \costof{C'}) - 1$ calls to the oracle, assuming
%   $\costof C \geq 2$ and $\Omega \geq 2$.
% \end{lem}
% \begin{proof}
% By induction, in a similar manner to \lemref{meld-num-oracles}. Full proof
% in the Supplementary material.
% \end{proof}


% \begin{theorem}[SOAM takes linear time] \label{thm:time}
%   For any circuit $C$, the algorithm $\mathsf{SOAM}(C)$ runs in time $O(\sizeof{C})$,
%   assuming that the oracle takes constant time on segments of depth $2\Omega$.
% \end{theorem}
% \begin{proof}
% By \lemref{optimize-num-oracles}, the number of calls to the oracle is
% at most $O(\sizeof C)$.
% %
% All other operations (including \lstinline{split}, \lstinline{concat}) take
% $O(1)$ time, and a constant number of such operations are performed per call to
% the oracle.
% %
% Every call to the oracle is on a segment of depth $2\Omega$ or smaller and
% takes constant time, by assumption.
% %
% The overall time is therefore $O(\sizeof C)$.
% \end{proof}




% The function $\mathsf{meld}$ takes two segmenttt optimal circuits $C_1$ and
% $C_2$, and returns an segment optimal circuit that is functionally equivalent to
% their concatenation.
% %
% Since the inputs $C_1$ and $C_2$ are segment optimal,
% all $\Omega$-segments that lie completely in $C_1$,
% or completely in $C_2$ are already optimal by definition.
% %
% The meld only considers those $\Omega$-segments that span the boundary
% between circuits $C_1$ and $C_2$,
% i.e., those segments which have some layers from circuit $C_1$ and other layers from $C_2$.
% %


% As shown in \figref{lopt-code},
% the function $\mathsf{meld}$ creates a $2\Omega$-segment, named $W$,
% by concatenating the last $\Omega$ layers of circuit $C_1$
% with the first $\Omega$ layers of circuit $C_2$,
% leaving behind a prefix $P$ of $C_1$ and a suffix $S$ of $C_2$.
% %
% Note that the $2\Omega$-segment $W$ covers all possible $\Omega$-segments
% at the boundary of $C_1$ and $C_2$.
% %
% This is because an $\Omega$-segment that crosses the boundary between the two circuits
% must contain at least one layer from both sides and has $\Omega$ layers in total.
% %
% Since each segment can contain at most $\Omega$ layers from both circuits,
% the total range of all $\Omega$-segments is $2\Omega$ layers.


% After creating the segment $W$,
% the meld algorithm invokes the oracle on it,
% which returns an segment optimal circuit $W'$.
% %
% If the costs of $W$ and $W'$ are identical,
% then $W$ is segment optimal and there are no optimizations at
% the boundary of $C_1$ and $C_2$.
% %
% In this case, the function $\mathsf{meld}$ returns
% concatenation of layers in $P$, $W$, and $S$.
% %
% Otherwise, the segment $W'$ improves the segment $W$.
% %
% In this case,
% the function meld calls itself recursively, twice:
% first, to meld the prefix $P$ with the (optimized) segment $W'$,
% and then to meld the result of the first recursive call with the suffix $S$.
%

% Note that both recursive calls satisfy the precondition of meld, i.e.,
% its inputs are segment optimal.
% % ?
% In the first recursive call, the circuit $P$ is segment optimal because its a subcircuit
% of circuit $C_1$, and the segment $W'$ is segment optimal
% because it is the returned by the oracle.
% %
% In the second recursive call,
% the circuit $\mathsf{meld}(P, W')$ is segment optimal because $\mathsf{meld}$
% returns an segment optimal circuit and the circuit $S$ is segment optimal
% because its a subcircuit of circuit $C_2$.
% %
% In the next subsection,
% we prove this formally and show that
% the output $\mathsf{meld}(C_1, C_2)$  is segment optimal (\lemref{meld-is-optimal}).
% %
% The overall running time of \coam{} algorithm is $O(\sizeof{C} + \costof{C})$,
% where $\sizeof{C}$ is the number of gates in the circuit.




% each recursive call to $\mathsf{meld}$ is performed
% only after



% Given a quantum circuit, circuit optimizers attempt to find the best
% circuit among functionally equivalent circuits~\cite{quartz-2022, queso-2023}.
% %
% However, the sheer number of these equivalent circuits presents a
% formidable challenge, because it grows exponentially with the size of the
% circuit.
% %
% State-of-the-art optimizers buckle under this exponential growth and
% have to be artifically terminated, typically by using timeouts.
% %
% As a result, the state-of-the-art optimizers are unable to make any
% guarantees on the quality of the optimized circuits and may miss
% available optimizations.


% To tackle this challenge, we propose an algorithm that prunes the
% search space of equivalent circuits by targeting fixed-size
% subcircuits within a given circuit.
% %
% Our algorithm leverages off-the-shelf optimization techniques to
% optimize individual subcircuits,
% and utilizes the obtained results to determine new subcircuits for further
% optimization.
% %
% It proceeds iteratively until there are no subcircuits that can be optimized.


% Our algorithm operates on circuits represented as sequences of layers, and
% considers subcircuits that are contiguous subsequences of layers.
% %
% To control the size of subcircuits,
% we incorporate a parameter $\Omega$, and only choose
% $O(\Omega)$-width subcircuits for optimization, where the \defn{width} of
% a subcircuit is the number of layers.
% %
% When it finishes,
% the algorithm guarantees that the output circuit is
% ${{\boldsymbol{\mathit{\Omega}}}}$\defn{-optimal},
% i.e., all $\Omega$-width subcircuits are optimal w.r.t. the optimizer.


% The algorithm scales linearly with the \defn{size} (number of gates) of the
% circuit, making only $O(\sizeof{C})$ calls to the optimizer and
% using at most $O(\sizeof{C})$ time for identifying and replacing subcircuits.


% \myparagraph{Oracle.}
% %
% Our algorithm uses an off-the-shelf optimizer on small ($O(\Omega)$-width)
% subcircuits.
% %
% We refer to the off-the-shelf optimizer as the \defn{oracle}, to disambiguate
% it from our optimization algorithm.
% %
% For our optimality guarantee, the only assumption we make is that the
% oracle is depth-preserving: i.e., for any circuit $C$, if the oracle optimizes
% this and produces $C'$, then $\textit{depth}(C') \leq \textit{depth}(C)$.


% \myparagraph{Bounded-size subcircuits: $\boldsymbol{k}$-segments.}
% %
% Our algorithm consults the oracle on small subcircuits that we call
% $k$-\emph{segments}, where $k$ is the \defn{width} of the segment.
% %
% A ${{\boldsymbol{\mathit{k}}}}$\defn{-segment} is a contiguous subsequence of
% $k$ layers of the circuit (using all $n$ qubits).
% %
% The total number of a gates in a $k$-segment therefore is at most $kn$.



% We represent a circuit $C = \langle L_0, L_1, \ldots \rangle$ as a sequence of
% layers $L_i$, and each layer is a set of gates, $g$.
% %
% A \defn{subcircuit} is a contiguous subsequence of layers.
% %
% The \defn{width} of a (sub)circuit is the number of layers, and the
% \defn{size} of a (sub)circuit $C$, denoted $|C|$, is the total number of gates,
% i.e., $|C| = \sum_i |L_i|$.


% \myparagraph{Circuit graph.}
% We represent a circuit $C$ with a directed acyclic graph
% consisting of five components
% $(Q_\textsf{src} \with Q_\textsf{snk} \with G \with E \with \Delta)$.
% %
% The graph has three kinds of vertices: sources, sinks, and gates.
% %
% For $n$ qubits, a circuit has $n$ distinguished source vertices
% $Q_\textsf{src}$, and $n$ distinguished sink vertices $Q_\textsf{snk}$,
% representing the input (source) and output (sink) qubit states.
% %
% The gates of the circuit are denoted $G$, and the edges $E$ are the ``wires''
% of the circuit.
% %
% In particular, each edge represents an intermediate qubit
% state which flows between two gates (or between a gate and a source/sink
% vertex).
% %
% The map $\Delta$ labels each edge with its associated qubit.
% %
% % The map $\Delta$ labels each edge of the graph with a qubit in set $Q$.
% %
% Note that for each gate in the set $G$,
% the number of incoming edges is equal to the number of outgoing edges, and
% the sets of incoming and outgoing labels are identical.

% \myparagraph{Subcircuits.}
% A circuit $C'$ is a \defn{subcircuit} of another circuit $C$ if
% it consists of a subset of gates and edges that respects dependencies between
% gates.
% %
% That is, for any two gates in $C'$, all paths between them in $C$ are also in
% $C'$.
% %
% Formally, for $C' = (Q_\textsf{src}' \with Q_\textsf{snk}' \with G' \with E' \with \Delta')$
% and $C = (Q_\textsf{src} \with Q_\textsf{snk} \with G \with E \with \Delta)$, we
% say $C'$ is a subcircuit of $C$ iff:
% \begin{itemize}
%   \item It is a subgraph, i.e., $Q_\textsf{src}' \subseteq Q_\textsf{src}$
%   and $Q_\textsf{snk}' \subseteq Q_\textsf{snk}$
%   and $G' \subseteq G$
%   and $E' \subseteq E$
%   and $\forall e \in E'. \Delta'(e) = \Delta(e)$.
%   \item For every path of gates
%   $p = \{(g_i, g_{i+1})\}_{0 \leq i < k} \subseteq E$,
%   if the endpoints $g_0$ and $g_k$ are in $G'$, then
%   $p \subseteq E'$.
% \end{itemize}
% %
% Intuitively, subcircuits are suitable units for circuit substitution, i.e.,
% any subcircuit can be replaced by an equivalent subcircuit.


% \myparagraph{Vertical circuit splitting.}
% Our algorithm splits circuits vertically, across all qubits.
% %
% To perform a vertical split, edges across the split need to be updated.
% %
% For each edge $(u,v)$ across the split, the edge is
% replaced with $(u, q_\textsf{snk})$ in the left subcircuit, and replaced with
% $(q_\textsf{src}, v)$ in the right subcircuit, where $q_\textsf{src}$ and
% $q_\textsf{snk}$ are the appropriate source and sink vertices for $\Delta(u,v)$.


% \sr{TODO: anything formal needed here for segments?}


% \myparagraph{segment optimality.}
% %
% The segment optimality guarantee, defined below, is a guarantee
% for all subcircuits of width at most $\Omega$.
% %
% \begin{definition}
%   A circuit is \defn{$\boldsymbol{\mathit{\Omega}}$-optimal} w.r.t. an oracle
%   optimizer if the oracle can not improve any subcircuit of width $\Omega$ or
%   smaller.
% \end{definition}


% \begin{figure}
% \includegraphics[width=0.95\columnwidth]{media/split-example.pdf}
% \caption{Example split. Single-lined circles are qubit sources, and double-lined
% circles are qubit sinks. Rectangles are gates. Note that concatenation is
% the inverse operation.}
% \label{fig:split-example}
% \end{figure}



% \myparagraph{$\Omega$-segments.}
% %
% The algorithm proceeds by selecting subcircuits and passing these to the oracle.
% %
% To guarantee segment optimality, the subcircuits selected by the algorithm
% are larger than $\Omega$.
% %
% In particular, the algorithm selects subcircuits that we call
% \emph{$\Omega$-segments}.


% An \defn{$\Omega$-segment} is a subcircuit of size at most $n\Omega$ (where $n$
% is the number of qubits), and is either \emph{initial} or
% \emph{final}.
% %
% An \defn{initial $\Omega$-segment} is the union of all subcircuits of size
% $\Omega$ that begin at the left edge of a circuit; such a segment can be
% constructed by performing a graph traversal starting at the source vertices of
% the circuit, picking at most $\Omega$ edges for each qubit.
% %
% A \defn{final $\Omega$-segment} is defined symmetrically for the right
% edge of a circuit, and can be constructed by performing a backwards graph
% traversal starting at the sink vertices.

% \begin{proof}
% We establish this by counting the number of calls to the oracle
% because other operations such as split and concat take $O(1)$ time.
% %
% The number of times the function $\mathsf{segopt}$ invokes the oracle is bounded
% by $O(\sizeof{C})$.
% %
% We prove this by induction on the size of circuit $\sizeof{C}$.
% %
% The function first partitions the circuit into circuits $C_1$ and $C_2$
% and calls itself recursively on both.
% %
% We can use induction to show that the function calls
% invoke the oracle $O(\sizeof{C_1})$ and $O(\sizeof{C_2})$ times respectively.
% %
% Thus, the total is $O(\sizeof{C_1} + \sizeof{C_2}) = O(\sizeof{C})$.
% %
% The function then calls function $\mathsf{meld}$ on the resulting circuits $C'_1$ and $C'_2$.
% %
% By \lemref{lem:meld-time},
% we have that this call invokes the oracle $O(\sizeof{C'_1} + \sizeof{C'_2})$ times,
% which is bounded by $O(\sizeof{C_1} + \sizeof{C_2})$ because the algorithm
% never increases the circuit sizes.
% %
% Thus, the total number of calls to the oracle is $O(\sizeof{C})$.
% %
% \end{proof}


% \subsection{Discussion}


% \jremark{discuss limitations of omega optimality here}
% \myparagraph{Different cost functions} \\
% \myparagraph{Local minima, and thoughts on global optima}
% meld is neither associative nor commutative.
% \myparagraph{Termination}

% \begin{theorem}

% \end{theorem}
%


\subsection{Circuit Representation and Compaction}
\ur{Maybe move to this to the end.  Say, for the analysis, we assume that split and concat are constant.  We describe in section x, how to achieve this by using a specific circuit representation.

UPDATE: I moved this here.  But I am not sure where it is used.  We
seem to be proving only the number of oracle calls and not end-to-end
run time.

}

Our algorithm represents circuits using a hybrid data structure that
switches between sequences and linked lists for splitting and
concatenating circuits in $O(1)$ time.
%
Initially, it represents the circuit as a sequence of layers,
enabling circuit splits in $O(1)$ time.
%
Later during optimization
when circuit concatenation is required,
the algorithm switches to a linked list of layers,
enabling $O(1)$ concatenation.
%
At the end of each optimization round,
the algorithm uses a function $\mathsf{compact}(C)$
to revert to the sequence of layers representation.
%

The function $\mathsf{compact}(C)$ ensures that the resulting circuit
is equivalent to $C$ while eliminating any unnecessary ``gaps'' in the layering,
meaning that every gate has been shifted left as far as possible.
%
For brevity, we omit the implementation of the $\mathsf{compact}$ function from \figref{lopt-code}.
%
Our implementation in practice is straightforward: we use a single left-to-right
pass over the input circuit and build the output by iteratively adding gates.
%
The time complexity is linear, i.e., $\mathsf{compact}(C)$ requires $O(|C| + \mathsf{length}(C))$ time.
%
%
% Local optimality requires that a layered circuit be as compact as possible,
% and the function $\mathsf{compact}(C)$ satisfies this condition.
%
%


% %
% In particular, if $C' = \mathsf{compact}(C)$ then we have $\compressed{C'}$, using the
% definition of compactness from \secref{lang}; the resulting circuit $C'$ is identical
% to $C$ except that every gate has been shifted left as far as possible.
%
% Our \algname{} algorithm uses this $\mathsf{compact}$ function in two ways.
% \begin{enumerate}
%     \item The output of every \oracle{} call is compacted. The cost of this compaction can be charged
%     against the oracle, because compaction is no more expensive than reading and writing the
%     input and output circuits. In this sense, compacting the output of every oracle call is ``free''
%     from an efficiency perspective.
%     Note that these compactions are not essential for any of our theorems; we include these in the
%     algorithm description because they are useful in practice, helping ensure that every optimization
%     phase is as productive as possible.
%     \item After every optimization phase, the entire circuit is compacted. Note that these compactions
%     are essential for guaranteeing local optimality.
% \end{enumerate}



\subsection{Meld Example}

We present an example of how \lstinline{meld} joins two circuits by
optimizing from the ``seam'' out, and only as needed.
%

\begin{figure}
  % \begin{minipage}[b]{0.5\linewidth}
  %     \includegraphics[width=1.3\linewidth, left]{media/transforms.pdf}
  % \end{minipage}%
  % \begin{minipage}[b]{0.5\linewidth}
  %   \includegraphics[width=1.3\linewidth]{media/circuits.pdf}
  % \end{minipage}
  \includegraphics[width=\linewidth]{media/new-ex.pdf}
  \caption{
  The figure shows a three-step meld operation and illustrates
  how it propagates optimizations at the boundary of two optimal circuits.
  %
  At the top, the figure shows specific optimizations ``1'' and ``2'',
  and towards the bottom,
  the figure shows the optimization steps of meld.
  %
  Before the first step,
  two individual circuit segments that are optimal are separated by a dashed line.
  %
  Each meld step considers a segment, represented by a box with solid/dotted/shaded lines,
  and applies an optimization to it, reducing the gate count.
  %
  The first step focuses on the boundary segment within the solid green box,
  overlapping with both circuits,
  and applies ``Optimization 1''.
  %
  This step introduces a flipped $\mathsf{CNOT}$ gate,
  which interacts with a neighboring $\mathsf{CNOT}$ gate
  and triggers ``Optimization 2'' in the purple dotted box.
  %
  The third step merges two neighboring rotation gates in the yellow shaded box.
  %
  }
  \label{fig:propagate}
\end{figure}


%
%
\figref{propagate} shows a three-step meld operation
that identifies optimizations at the boundary of two circuits.
%
All the circuits in the figure are expressed using
the $\mathsf{H}$ gate (Hadamard gate),
the $\mathsf{R_Z}$ gate (rotation around $\mathsf{Z}$),
and the two-qubit $\mathsf{CNOT}$ gate (Controlled Not gate),
which is represented using a dot and an XOR symbol.
%
We first provide background on the optimizations used by meld
and label them ``Optimization 1'' and ``Optimization 2''.
%
Optimization 1 shows that when a $\mathsf{CNOT}$ gate is surrounded by
four $\mathsf{H}$ gates,
all of these gates can replaced by a single
$\mathsf{CNOT}$ gate whose qubits are flipped.
%
Optimization 2 shows that when two $\mathsf{CNOT}$ gates
are separated by a $\mathsf{R_Z}$ gate as shown, they may be removed.
%

The steps in the figure describe a meld operation
on the two circuits separated by a dashed line, which represents their seam.
%
To join the circuits, the meld operation proceeds outwards in both directions
and
and optimizes the boundary segment, represented as a green box with solid lines.
%
The meld applies Optimization 1 to the green segment
and this introduces a flipped $\mathsf{CNOT}$ gate.
%

The meld propagates this change in step 2,
by considering a new segment,
which includes a neighboring layer.
%
We represent this segment by a purple box with dotted lines,
and it contains two $\mathsf{CNOT}$ gates,
one of which was introduced by the first optimization.
%
The meld then applies Optimization 2,
removing the $\mathsf{CNOT}$ gates and
bringing the two rotation gates next to each other.
%
Note that Optimization 2 became possible only because of Optimization 1,
which introduced the flipped the $\mathsf{CNOT}$ gate.
%
In the final step,
the meld considers the segment represented by a yellow box with shaded lines
and performs a third optimization, merging the two rotation gates.
%
Overall,
this sequence of optimizations,
at the boundary of two circuits,
reduces the gate count by seven.
%



==> app_linearity.tex <==
\section{Data for plots demonstrating linearity of the \coam{} algorithm}

\begin{table}[h]
  \centering
  \begin{tabular}{|c|c|}
  \hline
  Circuit Size & Time  \\
  \hline
  773 & 1.253099 \\
  6760 & 10.702689 \\
  79070 & 130.980059 \\
  \hline
  \end{tabular}
  \caption{Grover Algorithm}
  \end{table}


  \begin{table}[h]
  \centering
  \begin{tabular}{|c|c|}
  \hline
  Circuit Size & Time (s) \\
  \hline
  823 & 1.419056 \\
  3017 & 4.99482 \\
  6637 & 12.605396 \\
  18429 & 37.259161 \\
  26729 & 60.976757 \\
  36717 & 87.932398 \\
  62013 & 166.329584 \\
  \hline
  \end{tabular}
  \caption{HHL Algorithm}
  \end{table}


  \begin{table}[h]
  \centering
  \begin{tabular}{|c|c|}
  \hline
  Circuit Size & Time (s) \\
  \hline
  2040 & 4.868088 \\
  4190 & 9.218806 \\
  8476 & 17.38445 \\
  17020 & 37.453373 \\
  34084 & 72.494401 \\
  68174 & 142.821594 \\
  136320 & 300.366302 \\
  \hline
  \end{tabular}
  \caption{VQE Algorithm}
  \end{table}


  \begin{table}[h]
  \centering
  \begin{tabular}{|c|c|}
  \hline
  Circuit Size & Time (s) \\
  \hline
  640 & 1.390497 \\
  2494 & 9.433012 \\
  9294 & 31.65895 \\
  14230 & 46.774648 \\
  20190 & 66.723428 \\
  35182 & 11176746 \\
  \hline
  \end{tabular}
  \caption{Shor's Algorithm}
  \end{table}

  \begin{table}[h]
    \centering
    \begin{tabular}{|c|c|}
    \hline
    Circuit Size & Time (s) \\
    \hline
    640 & 1.390497 \\
    2494 & 9.433012 \\
    9294 & 31.65895 \\
    14230 & 46.774648 \\
    20190 & 66.723428 \\
    35182 & 111.076746 \\
    \hline
    \end{tabular}
    \caption{QFT Algorithm}
    \end{table}

    \begin{figure}
      \centering

      \subfloat[HHL]{\includegraphics[width=\columnwidth]{plots/linearityhhl0.01.png}}

      \caption{
      The figure plots the optimization times for the HHL quantum algorithm
      against the corresponding circuit sizes.}
      \label{fig:linear}
    \end{figure}

\cleardoublepage


==> eval-with-queso.tex <==
\ur{Meta: justify why we chose the cutoffs we did (0.6) etc}

This section describes the implementation of the \coam{} algorithm,
the integration of the implementation with two different optimizers,
and presents an evalution.
%
For the evaluation, we consider the time performance and scalability
as well as the circuit quality on a range of quantum circuits.
%
As our primary baseline, we consider the \quartz{}~\cite{quartz-2022}
optimizer, a super optimizer for quantum circuits that uses rule-based
substitutions to optimize circuits.
%
We also demonstrate the applicability of our implementation to the
QUESO optimizer~\cite{queso-2023}, which also uses rule-based optimizations
with different algorithms and heuristics.
%

\subsection{Implementation} \label{sec:impl}
We implement the \coam{} algorithm (\secref{algorithm}) in SML
(Standard ML), which comes with an optimizing compiler, MLton, that
can generate fast executables.
%
Our implementation represents circuits as an array of arrays, where
each array denotes a ``layer'' of the circuit.
%
To split the first and last $\Omega-$window of a circuit,
we split the first and last $\Omega$ layers of the circuit respectively.
%
Other circuit management operations are simple operations on this array representation.


As with the algorithm, our implementation can work with any oracle,
allowing also using existing optimizers.
%
We consider two existing optimizers as oracles: \quartz{}
and \queso{}.
%
We chose these optimizers  for two reasons.
%
First, these optimizers are both the state of the art among the recent
optimizers.
%
Second, they exemplify two entirely different conditions in terms of
integrating with our work: \quartz{} naturally integrates with our
work whereas \queso{} is challenging to do so.


The \quartz{} optimizer~\cite{quartz-2022}, which is written in C++,
integrates naturally with our implementation, because we are able to
call C++ codes directly from our implementation through a
cross-language integration feature.
%
Specifically, to optimize a subcircuit, we translate the subcircuit to
the QASM format and make a direct (cross-language) function call to
C++ that takes a QASM string and a timeout.
%
The function runs the \quartz{} optimizer and returns a QASM string
that represents the possibly optimized version of the input.
%
The \quartz{} optimizer, in turn, translates the QASM string to a
DAG-based representation, loads the rewrite rules, and applies them
according to its pattern matching algorithm.
%
We translate the QASM output of \quartz{} into our array-based
representation and update the circuit.
%
Note that this introduces overhead to the running time
of our algorithm
because each call to \quartz{} changes the circuit representation
and also pays for the initialization cost of \quartz{}.
%

To mitigate this overhead,
we send subcircuits of size $10*\Omega*n$ to \quartz{},
instead of the size $2*\Omega*n$ described in the algorithm,
where $\Omega$ represents \coam{}'s parameter and $n$ is the
number of qubits.
%
By sending larger circuits to \quartz{},
we ensure that the overhead does not dominate
the time to execute one function call to \quartz{}.
%
%This reduces the number of calls and thus reduces the cross-language
%overhead.
%
When the per call timeout is large enough, we send subcircuits of
size $2*\Omega*n$ as described in the algorithm.
%
% We also cache the rules used by quartz to reduce this overhead.
\ur{I did not understand the last sentence with 2Omega.}

\jr{revisit}

The \queso{} optimizer~\cite{queso-2023}, which is written in Java, does
not naturally integrate with our implementation, because our
implementation language does not cross-operate with Java.
%
We therefore integrate \queso{} via the operating system.
%
Specifically, to invoke \queso{} on a subcircuit, our \coam{}
implementation writes the QASM representation to a file and
calls \queso{} by using a system call.
%
This system call, in turn, writes its output to another file, which
our \coam{} implementation reads.
%
Because the overhead is large and difficult amortize by increasing
subcircuit sizes, our integration with \queso{} incurs significant
overhead.
%
Nevertheless, this integration demonstrates the feasibility of
integrating with existing optimizers either through cross-language
interoperability features (when feasible) or through systems calls.
%

% For this reasons, we compare with \queso{} only on a few benchmarks.
%
% \ur{This last sentence does not sound right.  It can be interpreted as ``the results were not good, so we are not showing you everything'' }


\paragraph{\coam{} configuration}

For our experiments, we configure several different configurations
of \coam{}

\begin{itemize}

\item \coamwith{\quartzt{0.06}}
refers to our implementation of \coam{} with \quartz{} running as oracle
where each call to \quartz{} is capped to complete in 0.06 seconds.

\item \coamwith{\quartzt{0.6}}: \coam{} with \quartz{} oracle,
with upto 0.6 seconds per call

\item \coamwith{\quartzt{6}}: \coam{} with \quartz{} oracle,
with upto 6 seconds per call

\item \coamwith{\quesot{1}} refers to our implementation of \coam{} with \queso{} running
as oracle where each call to \queso{} is capped to complete in 1 second.
\footnote{1 second is the minimum timeout \queso{} supports.}
\end{itemize}
%

%% We then run vanilla \quartz{} on the whole circuit
%% for the same end-to-end time as our algorithm
%% and compare the circuit quality.
%% %
%% We perform this experiment with three different timeouts ($t = 0.06$s, $0.6$s, $6$s),
%% each of which increases the end-to-end running time ten fold.
%

For all our experiments, we set the window width of \coam{} to $6$,
i.e., $\Omega = 6$.
%
We choose this value because
it aligns with the default optimization behavior of \quartz{} and \queso{},
both of which only focus on sub circuits of size $6$ at any optimization step.
%
As described in their respective papers,
the size $6$ is a sweet spot for both the tools,
since increasing the size hinders time performance,
and decreasing it harms circuit optimizations~\cite{quartz-2022, queso-2023}.
%
By setting the window width to $6$,
our algorithm feeds all subcircuits of size $6$ to \quartz{}/\queso{},
giving them enough scope to apply their optimizations.
\footnote{We note that this size $6$ is for the Nam gate set that we use in this paper.}

\myparagraph{Benchmarks.}
\input{benchmarks.tex}


\subsection{\coam{} scales linearly with the size of circuits}
\input{fig/linearity.tex}

To optimize circuits,
both \quartz{} and \queso{} execute a search algorithm
by maintaining a search queue of candidate circuits.
%
At each step,
they pop a circuit from the queue and discover ways to rewrite parts of the circuit
by referring to their database of equivalent circuits.
%
Then,
they insert the new circuits back to the queue and repeat the process
until the queue becomes empty.
%
Since the number of circuits to consider grows exponentially with the size of the circuit,
both tools use a ``beam search algorithm'',
a search algorithm that limits the size of the search queue
and appropriately drops circuits after the limit is reached.
%
Because beam search limits the size of the search queue,
its space usage is linear in the size of circuit
(it only stores a fixed number of circuits at any point).
%

However, despite dropping circuits,
\quartz{} and \queso{} deliver poor time scalability,
because the number of the circuits that need to be considered
increases exponentially with the size
of the circuits
and so does the running time of both the tools.
%
For instance,
\queso{} takes eighteen seconds to terminate on a circuit of size 48,
which jumps to an hour on a circuit of size 96 (a $20$x increase),
and further jumps to around six hours for a circuit of size 326 (a $6$x increase).
%
\quartz{} on the other hand does not terminate on the $48$ sized circuit within $24$ hours.
%
Because of their exponential time complexity,
both approaches deliver poor time scalability and
in practice, provide no quality guarantee.
%
With the \coam{} algorithm,
our goal is to deliver a quality guarantee in reasonable running times
that scale linearly with the size of circuits.

In this section,
we demonstrate the scalability of the \coam{} algorithm
by measuring its execution time across different sizes of benchmarks.
%
For this experiment, we use $\quartzt{0.06}$ as our oracle
(i.e., each sub circuit is optimized by calling \quartz{} for a duration of $0.06$ seconds).
%
We consider four quantum algorithms: Grover, VQE, QPE, and QFT,
and plot the results in \figref{linear}.
%
The Y-axis shows the execution time and the X-axis shows the size of benchmarks.
%
We vary the size of circuits by changing the number of qubits in the corresponding algorithms.
%
The plots show that the execution time scales linearly
across sizes ranging from a few hundreds of gates to circuits as large as $0.14$ millions
of gates.
%
For example,
in case of the VQE algorithm,
the \coam{} algorithm takes around five seconds for the smallest circuit of size two thousand
and takes around 300 seconds for the largest circuit of size one hundred thousand ($136000$ precisely).
%
We provide the data points for our plots in the Appendix.
%

One of the key benefits of our algorithm
is that runs in a predictable amount of time and within that time,
guarantees $\Omega-$optimality.
%
In the next subsection,
we establish that ensuring $\Omega-$optimality leads to good circuit quality.

% \cleardoublepage
% \cleardoublepage
\subsection{Scalable optimization using \coam{} with \quartz{}} \label{sec:quartz}
In this section, we study the benefits of our \coam{} algorithm
when used with \quartz{}.
%
We optimize the circuit with the \coam{} algorithm using \quartz{} as the oracle,
where each oracle call is capped by a fixed amount of time.
%
Then,
we run the default \quartz{} on the whole circuit for the same end-to-end time
%
and compare the circuit quality.

%
\begin{figure*}
  \centering
  \input{fig/prelim.0.01}
  \caption{The figure compares the performance of $\coamt{\quartzt{0.06}}$ against standard \quartz{}.
  The label ``S'' represents $\coamt{\quartzt{0.06}}$ and the label ``Q'' represents \quartz{}.
  %
  The figure compares the circuit sizes (lower is better) and the optimization rates (higher is better) of both approaches.
  %
  The optimization rate measures the number of optimizations performed per second of execution.
  %
  Both the approaches execute for the same end-to-end time and the figure presents the running time in the ``Time'' column (in seconds).
  }
  \label{fig:comp-small}
\end{figure*}

\figref{comp-small} shows the result of this comparison,
where each call to \quartz{} is limited to $0.06$ seconds,
i.e., the figure shows results of configuration $\coamwith{\quartzt{0.06}}$.
%
The figure shows the original circuit sizes
and displays the circuit sizes after optimization.
%
The figure labels the results of the \coam{} algorithm as ``S'' and
the standard \quartz{} approach as ``Q''.
%
In the cases where one approach performs better,
the figure uses bold numbers, with lower numbers indicating better circuit quality.
%
The `C/Q' ratio column quantifies the improvement using the \coam{} algorithm w.r.t. standard \quartz{}.
%
The figure also provides and compares the \defn{optimization rate} of both approaches,
where the optimization rate is the number of gates optimized per second of execution.
%
A higher rate indicates faster optimizations.
%
The time column shows the execution time
for both cases.



\myparagraph{Quality.}
We observe that in seventeen cases,
using the \coam{} algorithm improves the quality of circuits w.r.t. standard \quartz{}
and sometimes does so by a wide margin.
%
In the other seven cases,
both approaches output the same quality of circuits.
%
For the hhl circuits,
the \coam{} algorithm finds reductions ranging from $23\%$ to $27\%$,
where \quartz{} does not find many optimizations
within this time (less than $5\%$).
%
In the case of grover circuits,
the \coam{} algorithm optimizes gate count by $10\%$ across the various sizes.
%
However, the efficacy of \quartz{} reduces from $9\%$ to $0\%$ with increasing sizes.
%
In the qpe circuits,
neither approach finds any optimizations.
%
This is because the core of these circuits
is a modular exponentiation circuit which is already well optimized.
%
For the vqe family,
the \coam{} algorithm reduces the gate count by around $60\%$ and
the optimizations by \quartz{}
are around $10\%$ of the circuit in the same time.
%
Overall, we observe that \coam{} generates $0.73$x smaller circuits on average.

\myparagraph{Scalability.}
Across the board,
we observe that the gap between the two approaches widens with increasing circuit sizes.
%
This is because the efficiency of \quartz{},
quantified by optimization rates,
reduces with increasing circuit sizes,
whereas the \coam{} algorithm scales to larger sizes.

For example,
across different sizes of qft,
the \coam{} algorithm achieves optimization rates
ranging from $50$ to $85$ and the rates in fact increase as the circuit size grows.
%
In contrast,
the optimization rate for \quartz{} reduces from around $28$ to $16$.
%
The 'C/Q' ratio of optimization shows how many more optimizations (per second)
the \coam{} algorithm identifies compared to \quartz{}.
%
Compared to \quartz{},
the \coam{} algorithm yields $1.78$x and $5.19$x more optimizations per second
for the smallest and largest qft instances
respectively (see the ratio column in \figref{comp-small}).
%
Similarly,
in the case of vqe,
the gap in their optimization rates
rises from around $2$x on the smallest instance to $42$x
on the largest instance.

All families of circuits follow a similar trend:
the optimization rate ratio between the \coam{} approach and the \quartz{} optimizer
increases with the circuit size,
demonstrating the scalability advantages of the \coam{} algorithm.
%
This scalability advantage of the \coam{} approach is built into the algorithm
because it calls \quartz{} only on small circuits,
where \quartz{} delivers excellent results.
%
The algorithm never sends large circuits to \quartz{},
where  \quartz{} struggles,
and instead, stitches together small circuits by melding them (\secref{algorithm}).
% Because the \coam{} algorithm runs in linear time,
% it delivers good scalability as circuit sizes increase.
% %
% %
% %
% Because the execution time is equal for both approaches,
% the ratio column additionally represents the ratio of total optimizations.
%
% %
% For example,
% consider the ratio column of \figref{comp-small} which compares the optimization rates
% of the \coam{} algorithm with \quartz{}.
%
\begin{figure*}
  \centering
  \input{fig/prelim.0.1}
  \caption{
    The figure compares the performance of $\coamwith{\quartzt{0.6}}$ against standard \quartz{}.
    %
  The label ``S'' represents $\coamwith{\quartzt{0.6}}$ and the label ``Q'' represents \quartz{}.
  %
  The figure compares the circuit sizes (lower is better) and the optimization rates (higher is better) of both approaches
  after running them for the same end-to-end time.
  }
  \label{fig:comp-med}
\end{figure*}

\myparagraph{Consistency.}
Since the \coam{} algorithm partitions the circuit into pieces
and melds them together,
it raises the question whether the splitting and melding loses any optimizations.
%
We evaluate this question by running the standard \quartz{},
which operates on the whole circuit, for a longer running time
and comparing the quality achieved.

We extend the running time by increasing the per-call timeout to \quartz{}
to $0.6$s, i.e.,
we consider the configuration \coamwith{\quartzt{0.6}}.
%
We note that the end-to-end running time becomes at least ten fold in this configuration,
and we run the standard \quartz{} for the extended time.
%
The figure shows that the \coam{} algorithm consistently generates better quality circuits
in all families.
%
We note that the gap between the approaches has reduced.
%
This occurs because as optimizers operate for longer times,
their optimization rates diminish due to the
increasing difficulty of finding further optimizations~\cite{quartz-2022, queso-2023}.
%
The difference in optimization rates between \figref{comp-small} and \figref{comp-med}
exemplifies this.
%
For example, the optimization rate in vqe\_n12 for \quartz{} reduces from around $30$ to $12$
when its execution time increases from $37$ seconds to $640$ seconds.
%
The many fold extension of execution time decreases the optimization rates of both approaches
and moderates the scalability advantages of the \coam{} algorithm.
%
On average,
circuits generated by the \coam{} algorithm are $0.9$ times smaller than those generated by
\quartz{}.
%/
In the Appendix,
we include a third configuration (\coamwith{\quartzt{6}})
where we further increase the time ten fold and observe a similar trend,
where \coam{} continues to deliver better quality circuits.
%

We conclude that, in practice,
the \coam{} algorithm comes at no cost to circuit quality
even with the extended runtime,
as it never generates a worse quality circuit.
%

% To summarize,
% \figref{fig:comp-small} demonstrates that the \coam{} algorithm
% drastically improves the speed of optimization for each circuit.
% %
% It shows that the algorithm scales well with circuit size,
% achieving excellent optimization rates across a range of sizes.
% %
% \figref{fig:comp-med} shows that this performance
%

%


% \input{fig/prelim2.0.01}



% To summarize,
% \figref{fig:comp-small} demonstrates that the \coam{} algorithm
% drastically improves the speed of optimization for each circuit.
% %
% It shows that the algorithm scales well with circuit size,
% achieving excellent optimization rates across a range of sizes.
% %
% \figref{fig:comp-med} shows that this performance comes at no cost to circuit quality
% even with the extended runtime,
% as the \coam{} algorithm never generates a worse quality circuit.
% %


\subsection{Scalable optimization using \coam{} with \queso{}}

\begin{figure*}
  \centering
  \input{fig/queso}
  \caption{
  The figure compares the performance of $\coamwith{\quesot{1}}$ against standard \queso{}.
  %
The label ``S'' represents $\coamwith{\quesot{1}}$ and the label ``Q'' represents \queso{}.
%
The figure compares the circuit sizes (lower is better) and the optimization rates (higher is better) of both approaches
after running them for the same end-to-end time.
}
  \label{fig:comp-queso}
\end{figure*}

In this section,
we evaluate the \coam{} algorithm using the \queso{} optimizer.
%
We integrate the \queso{} optimizer into our algorithm as an oracle
and impose a one second time out for each call.
%
We note that \queso{} does not follow the given timeout strictly
and often takes longer to run and return the result (around $4/5$ seconds per call).

To evaluate the algorithm,
we run it with \queso{} and compute the final circuit
and the overall execution time, excluding time for file I/O (\secref{impl}).
%
Then, we execute default \queso{} on the whole circuit for the same total runtime
and compare the quality of circuits produced.
%
For this experiment,
we filter benchmarks based on their sizes and
opt for benchmarks whose sizes are less than ten thousand gates.
%
This size limitation arises from file I/O overheads which make restrict our ability
to run larger circuits within reasonable times.

\figref{comp-queso} shows the results of the evaluation for seven benchmarks
coming from four families of algorithms.
%
The ``QS'' column denotes \queso{} and the ``S'' column represents the \coam{} algorithm
using \queso{} as the oracle.
%
In all cases, the \coam{} approach generates smaller circuits than the baseline \queso{}.
%
Similar to the case with \quartz{} (\secref{quartz}),
we observe that the gap between the \coam{} approach and default \queso{} increases
with circuit size.
%
Foe example,
in the grover family,
the ratio of optimization rate between \coam{} and \queso{}
increases from $1.14$x for grover\_n7 to $1.4$x in grover\_n9.
%
For the circuit vqe\_n12,
which is the largest circuit on the table,
the final circuit size is $0.78$ times smaller compared to \queso{},
which demonstrates the scalability of the \coam{} approach.
%
On average,
the algorithm's circuits are $0.92$x smaller than those generated by \queso{}
and the algorithm makes $1.27$x as many optimizations per second.
%

The evaluation demonstrates that the \coam{} algorithm
improves the scalability of the \queso{} optimizer and
consistently delivers better quality circuits.


\subsection{CNOT and T count reduction}
\begin{figure*}
  \centering
  \input{fig/clifft}
  \caption{Evaluating $\coamt{\quartzt{6}}$ on metrics
  T count and CNOT count for benchmarks in \clifft{} gate set }
  \label{fig:comp-cliff}
\end{figure*}

% IT IS WELL KNOWN That xxx. IN principle, we could have an optimizer. We therefore to evaluate.
We have evaluated benchmarks with gate count
as the quality metrics
because our oracles, \quartz{} and \queso{}, directly support it.
%
However, it is well known that depending on the gate set,
other metrics become more important.
%
For example, in the \clifft{} gate set,
T count is an important metric of circuit quality
because T gates they are not as computationally efficient
compared as the Clifford gates (T gates roughly cost 50x other gates in practice \cite{Nam_2018}).
%
Similarly, CNOT count is another important metric because CNOT
gates operate on two qubits and are expensive to implement.
%


In this section,
we evaluate the benefit of our current configuration, i.e. $\coamwith{\quartzt{6}}$,
for metrics ``T count'' and ``CNOT count''.
%
Note that, in principle,
we could plug in an optimizer which is designed for these metrics,
but here we evaluate the benefit with \quartz{} that is designed with circuit size
as the metric.
%
To do so, we translate our benchmark suite, expressed in the Nam gate set,
to the \clifft{} gate set.
%
We then translate the optimized version of our benchmarks
and compare the unoptimized and optimized translation.
%
%

To translate a benchmark from the Nam gate set to the \clifft{} gate set,
we use gridsynth,
a tool that translates parameterized $\mathsf{R_Z}$ gates
to the \clifft{} gate set in provably optimal fashion~\cite{gridsynth}.
%
We also decompose the $\mathsf{X}$ gate to \clifft{} circuits
using the Qiskit compiler.
%
We run Qiskit  in the mode where it does not perform any optimizations.
%
Note that the translation does not change the CNOT count because
it only removes single qubit nam gates and replaces them with single qubit Clifford gates.
%
Thus, the CNOT count comparison stays the same for both, the Nam and the \clifft{} gate sets.

\figref{comp-cliff} shows the results of this evaluation.
%
The figure compares
the circuit size, the T count, and CNOT count,
of the unoptimized translation and the optimized translation
with columns labelled ``U'' and ``O'' respectively.
%
Across the board,
we observe that the implementation finds reductions in size and
they correlate with reductions in T count and CNOT count.
%
In case of the ham15-med circuit,
the implementation reduces the T count by $7\%$
and the CNOT count by $6\%$;
the larger variant, circuit ham15-high,  also shows similar numbers.
%
For qft circuits,
we observe that gate count reduction and T count reduction
is perfectly correlated,
as both are reduced by the same percentage on all the qft instances.
%
On average,
the implementation reduces the circuit size by around $11.8\%$,
the T count by $6.8\%$, and the CNOT count by $5.68\%$.



% \input{prelim}

% \cleardoublepage
% \subsection{Eval half 2}
% \input{prelim2.tex}
% \subsection{Plots}
% \input{plots_greedy.tex}
% \cleardoublepage
% \subsection{Cliff Eval half 1}
% \input{prelim1.clifft}
% \cleardoublepage
% \subsection{Cliff Eval half 2}
% \input{prelim2.clifft}
% \subsection{Plots Cliff}
% \input{plots_greedy_cliff.tex}


==> evaluation_old.tex <==

In this section,
we evaluate the \coam{} algorithm by instantiating it with three oracle
optimizers (\feyntool{}, \quartz{}, and \queso{}), as outlined in \secref{impl}.
%
We denote the resulting optimizers as
\coamwith{\feyntool}, \coamwith{\quartz}, and \coamwith{\queso} respectively,
and describe how these are configured in \secref{methodology}.
%
Our evaluation covers 21 quantum circuits from seven quantum algorithms.
%
We organize the results into the following parts:
%
\begin{itemize}
  \item In \secref{comp-feyn}, we evaluate our \coamwith{\feyntool} optimizer
   on T count reduction.
  %
  We observe that the $\Omega-$optimal circuits produced by our optimizer
  match the output quality of \feyntool{},
  suggesting that $\Omega-$optimality is good optimization criterion for T count optimization.
  %
  Our optimizer runs faster than \feyntool{} in almost all cases
  and we observe that the speedup increases with circuit size.
  %

  \item In \secref{comp-quartz} and \secref{comp-queso},
  we evaluate our optimizers \coamwith{\quartz} and \coamwith{\queso{}}
  for optimizing gate count.
  %
  We observe that the \coam{} algorithm effectively utilizes the base optimizers,
  delivering significant size reduction across a range of quantum circuits.

  \item In \secref{var-segment}, we study the impact of $\Omega$ on the output quality and running time of \coam{}.
\end{itemize}


% the integration of the implementation with \quartz{}, an off-the-shelf optimizer,
% and present an evaluation.
% %
% For the evaluation, we consider the time performance and scalability
% as well as the circuit quality on a range of quantum circuits.
% %
% As our baseline, we consider the \quartz{}~\cite{quartz-2022}
% optimizer, a super optimizer for quantum circuits that uses rule-based
% substitutions to optimize circuits.








%
% We also demonstrate the applicability of our implementation to the
% QUESO optimizer~\cite{queso-2023}, which also uses rule-based optimizations
% with different algorithms and heuristics.
%

%
% Because of the exponential time complexity, both approaches
% deliver poor time scalability, and in practice, provide no quality guarantee.
%
% With the \coam{} algorithm,
% our goal is to deliver a quality guarantee in reasonable running times
% that scale linearly with the size of circuits.
%


\subsection{Methodology}
\input{methodology.tex}

\subsection{Benchmarks}
% \myparagraph{Benchmarks.}
\input{benchmarks.tex}

\subsection{\coam{} with the \feyntool{} optimizer}
\label{sec:comp-feyn}
In this section,
we study the performance of our \coamwith{\feyntool} optimizer,
which runs the \coam{} algorithm with \feyntool{} as the oracle optimizer.
%
We evaluate the running time and output quality of our optimizer
by running the baseline \feyntool{}.
%
For all our benchmarks,
we set the segment depth $\Omega$ to be $120$.
%
The output of our \coamwith{\feyntool{}} is $\Omega-$optimal with $\Omega = 120$
and the cost function is the T count of the circuit.
%

\begin{figure}
  \centering\small
  \input{fig/prelim.feyn.120.tex}
  \caption{
  The figure shows the optimization results of our $\coamwith{\feyntool{}}$ tool and \feyntool{},
  using T count as the cost metric.
  %
  The labels ``S'' and ``F'' represent $\coam{}$ and \feyntool{} respectively.
%
  The figure presents T counts (lower is better) and
  running time (lower is better) for both optimizers.
%
The results demonstrate that optimizer $\coamwith{\feyntool{}}$,
which guarantees $\Omega-$optimality delivers a similar quality of circuits as \feyntool{}.
%
The figure also calculates the speedup of the \coam{} approach using the ``T(F)/T(S)'' ratio.
%
On average, the$\coamwith{\feyntool{}}$ delivers excellent time performance
and runs in $6.9$x less time, compared to \feyntool{}.
%
We impose an end-to-end timeout of 10 hours (36000 seconds).
%
}
  \label{fig:feynopt}
  % \setlength{\belowcaptionskip}{-20pt}
\end{figure}



\figref{feynopt} shows the results of this experiment.
%
The figure separates circuit families with horizontal lines
and sorts circuits within families by their size/number of qubits.
%
The figure calculates the metric T count for the input circuit and for
the circuits returned by \feyntool{} and \coamwith{\feyntool{}},
or \coam{} for short, labelled by ``F'' and ``S'' respectively.
%
The ``F/S'' represents the quality ratio of the two approaches.
%
The figure also shows the running times of both approaches and computes
the ratio ``F/S'', measuring the relative speedup from the \coam{} algorithm.
%
The results shows our \coam{} algorithm generates reliable quality circuits
in short running times.

\myparagraph{Optimization  Quality.}
The results show that our optimizer \coam{} matches the output quality of \feyntool{}.
%
There are a few cases where there is a difference of less than $1\%$,
such as the ``hhl'' circuit with $7$ qubits.
%
But overall, there is no noticeable difference and
the quality ratio of the outputs is $1$.
%
%
This experiment shows that $\Omega-$optimality, as guaranteed by
our \coam{} algorithm is a reliable quality criterion for T count optimization.
%for the \feyntool{} optimizer.
% This consistent output quality demonstrates
% that $\Omega-$optimality is a reliable quality guarantee for the optimizer \feyntool{}.
%
Note that the baseline \feyntool{} can, in principle, discover more optimizations
because it operates on the full circuit.
%
But in practice, we observe that optimizing the circuit in piecewise
fashion,
on circuit segments of size $\Omega$ and guaranteeing $\Omega-$optimality
finds similar optimizations.
%
In \secref{var-segment}, we confirm this for a range of $\Omega$ values.
%

\myparagraph{Run time.}
The figure also shows the running time of both approaches,
and calculates the speedup of the \coam{} approach using the ``T(F)/T(S)'' ratio.
%
Our \coam{} algorithm is slower by about factor two in one benchmark,
``grover'', but in all other benchmarks it performs better than \feyntool{},
running $6.9$x faster on average,
%
with no noticeable impact on the optimization quality (``F/S'' column).
%
For any given family, our \coam{} algorithm's speedup increases
consistently with the circuit sizes.
%
For example,
in the ``hwb'' family,
our \coam{} algorithm is $1.2$x faster for the smallest instance (with 8 qubits)
and runs $83$x faster for the largest instance (12 qubits)
%
;
%
For the ``hhl'' family,
our \coam{} algorithm is $23$x faster for the smallest instance (7 qubits)
and runs at least $94$x faster for the largest instance (9 qubits)
(on 9 qubits \feyntool{} does not terminate within our timeout of ten hours).
%
%

\myparagraph{Summary.}
The experiments suggest that local optimality is an effective
optimization criteria for T-count optimization. By focusing on local
optimizations, our \coam{} algorithm (with \feyntool{} as an oracle)
can optimize for T-count effectively and efficiently.
%

%% \todo{We observe...
%% %
%% Our theoretical results suggest that this gap could be understood as an
%% asymptotic gap,
%% %
%% for the following reasons....}

\if0
%%% THIS IS HARD TO READ FOR ME (UMUT)
Given that the speedup consistently increases with the circuit size,
the performance results indicate an asymptotic difference in running time of both
approaches.
%
We can confirm this difference using the theory results in \secref{algorithm}.
%
Specifically,
the \feyntool{} optimizer takes polynomial (at least quadratic) time
both in the number of qubits and the depth of the circuit.~\cite{amy2019formal}.
%
The optimizer \coamwith{\feyntool} is also polynomial in the number of qubits,
but scales linearly in the depth/size of the circuit.
%
From \corref{linear-calls},
using the fact that the cost function is T count,
we get that \coamwith{\feyntool} makes $O(\sizeof{C})$ calls to \feyntool{},
where $\sizeof{C}$ is the size of circuit $C$;
each call runs on small circuits of depth at most $2\Omega$ (\thmref{cost})
and therefore, each call to \feyntool{}
takes polynomial time in the number of qubits (the depth is constant).
%
Because the number of oracle calls is linear,
the total runtime of \coamwith{\feyntool} is linear in the size and polynomial in the number of qubits,
which is asymptotically different from \feyntool{}, which takes polynomial in both.
%
\fi

% %
% Because each such call only runs the optimizer on ``small circuits'' of depth at most $2\Omega$,
% the cost of each \feyntool{} call only depends on the number of qubits, which are roughly constant
% for most qubits in the figure.
% %
% Thus, the \coamwith{\feyntool} optimizer practically shows linear scalability.


% Thus, roughly speaking, the optimizer \coamwith{\feyntool} decomposes the complexity
% of optimization using \feyntool{} and makes it scale linearly (instead of quadratically)
% in the size of the circuit.
% %
% In summary,
% the optimizer \coamwith{\feyntool} consistently
% delivers reliable quality circuits with excellent scalability.
% %
% %
% The results demonstrate that $\Omega-$optimality is a practical and reliable
% quality criterion in circuit optimization with \feyntool{} optimizer.
% asymptotically improves the running time of optimization using \feyntool{}.
% \coamwith{\feyntool} delivers linear running time
% without compromising circuit quality.
%
% \secref{linear} discusses the linear running time of \coamwith{\feyntool} in more detail.


% % IT IS WELL KNOWN That xxx. IN principle, we could have an optimizer. We therefore to evaluate.
% We have evaluated benchmarks with gate count
% as the quality metric
% because our oracle, \quartz{}, directly supports it.
% %
% However, it is well known that depending on the gate set,
% other metrics become more important.
% %
% For example, in the \clifft{} gate set,
% T count is an important metric of circuit quality
% because T gates they are not as computationally efficient
% compared as the Clifford gates (T gates roughly cost 50x other gates in practice \cite{Nam_2018}).
% %
% Similarly, CNOT count is another important metric because CNOT
% gates operate on two qubits and are expensive to implement.
% %


% In this section,
% we evaluate the benefit of our configuration $\coamwith{\quartzt{6}}$,
% for metrics ``T count'' and ``CNOT count''.
% %
% Note that, in principle,
% we could plug in an optimizer which is designed for these metrics,
% but here we evaluate the benefit with \quartz{} that is designed with circuit size
% as the metric.
% %
% To do so, we translate our benchmark suite, expressed in the Nam gate set,
% to the \clifft{} gate set.
% %
% We then translate the optimized version of our benchmarks
% and compare the unoptimized and optimized translation.
% %
% %

% To translate a benchmark from the Nam gate set to the \clifft{} gate set,
% we use gridsynth,
% a tool that translates parameterized $\mathsf{R_Z}$ gates
% to the \clifft{} gate set in provably optimal fashion~\cite{gridsynth}.
% %
% We also decompose the $\mathsf{X}$ gate to \clifft{} circuits
% using the Qiskit compiler.
% %
% We run Qiskit  in the mode where it does not perform any optimizations.
% %
% Note that this translation does not change the CNOT count because
% it only replces single qubit nam gates with single qubit \clifft{} gates.
% %
% Thus, a CNOT count comparison applies to both the Nam and the \clifft{} gate sets.

% \figref{comp-cliff} compares
% the circuit size, the T count, and CNOT count,
% of the unoptimized translation and the optimized translation
% with columns labelled ``Input'' and ``Output'' respectively.
% %
% Across the board,
% we observe that the implementation finds reductions in size and
% they correlate with reductions in T count and CNOT count.
% %
% In case of the ham15-med circuit,
% the implementation reduces the T count by $7\%$
% and the CNOT count by $6\%$;
% the larger variant, circuit ham15-high,  also shows similar numbers.
% %
% For qft circuits,
% we observe that gate count reduction and T count reduction
% is perfectly correlated,
% as both are reduced by the same percentage on all the qft instances.
% %
% On average,
% the implementation reduces the circuit size by around $11.8\%$,
% the T count by $4\%$, and the CNOT count by $6.2\%$.


% \cleardoublepage
% \cleardoublepage

\subsection{\coam{} with the \quartz{} optimizer}
\label{sec:comp-quartz}

% In this subsection,
% we establish that ensuring $\Omega$-optimality leads to good circuit quality.
%
% Additionally, we study the benefits of our \coam{} algorithm when used with
% \quartz{}.

% One of the key benefits of our algorithm
% is that runs in a predictable amount of time, and (within that time)
% guarantees $\Omega$-optimality.
%
% In this section, we show how the \coam{} algorithm
% improves the \quartz{} optimizer.
% %
% We optimize circuits using the optimizer  $\coamwith{\quartzt{t}}$
% with segment depth $\Omega$ equal to $6$
% and
% The optimizer $\coamwith{\quartzt{t}}$ runs the \coam{} algorithm
% using \quartz{} as the oracle,
% where each call to \quartz{} is roughly allocated $t$ amount of time per gate,
% i.e., if the \coam{} algorithm calls \quartz{} for a circuit of size $k$,
% the timeout we give to \quartz{} is $k*t$.
% %
% We use the timeout functionality in \quartz{} to implement this.
% %
% We present results with the per-gate timeout $t = 0.01s$,
% but we also provide results of timeouts $t = 0.1s$ and $t = 1s$ in the Appendix.
% %
% % We chose the segment depth as $6$ because the default \quartz{} optimizer uses
% equivalence rules for circuits upto size $6$.
% %
% With segment depth as $6$,
% the algorithm feeds all segments of size $6$ to \quartz{}
% giving it enough scope to apply its optimizations.
%


% \begin{figure}
%   \centering
%   \small
%   \input{fig/prelim.0.01}
%   \caption{
%   The figure displays the number optimizations and running time of our optimizer $\coamt{\quartzt{0.01}}$
%   and also shows the optimizations by baseline \quartz{} in the same end-to-end time.
%   %
%   The label ``S'' represents the $\coam{}$ approach and the label ``Q'' represents \quartz{}.
%   %
%   The $S/Q$ column shows how many more optimizations \coam{} finds w.r.t \quartz{} for the same running time.
%   %
%   The figure shows that our \coam{} algorithm finds significant reductions ranging
%   from $20\% - 60\%$ in short runtimes.
%   %
%   Time column shows the runtime in seconds.
%   }
%   \label{fig:comp-quartz}
%   % \setlength{\belowcaptionskip}{-20pt}
% \end{figure}



\begin{figure}
  \centering
  \small
  \input{fig/prelim.compress}
  \caption{
  The figure displays the number optimizations and running time of our optimizer $\coamt{\quartzt{0.01}}$
  and also shows the optimizations by baseline \quartz{} in the same end-to-end time.
  %
  The label ``S'' represents the $\coam{}$ approach and the label ``Q'' represents \quartz{}.
  %
  The $S/Q$ column shows how many more optimizations \coam{} finds w.r.t \quartz{} for the same running time.
  %
  The figure shows that our \coam{} algorithm finds significant reductions ranging
  from $20\% - 60\%$ in short runtimes.
  %
  Time column shows the runtime in seconds.
  }
  \label{fig:comp-quartz}
  % \setlength{\belowcaptionskip}{-20pt}
\end{figure}

In this section, we evaluate our $\coamwith{\quartzt{0.01}}$ optimizer,
which runs the \coam{} algorithm using \quartz{} as the oracle.
%
To evaluate its optimizations,
we run our optimizer on all the circuits and record its output and the running time.
%
Then,
we run default \quartz{} on the each input circuit for the same end-to-end time,
%
and analyze the number of optimizations discovered.

\figref{comp-quartz} shows the results for circuits taken from six families of quantum algorithms.
%
In the figure,
the label ``S'' denotes the number of optimizations discovered by our \coam{} algorithm
and label ``Q'' denotes the same with baseline \quartz{} (higher is better).
%
In cases where one approach finds more optimizations,
the figure uses bold numbers.
%
The label ``S/Q'' computes the \defn{optimization ratio} which is
the ratio of number of optimizations.
%
A higher ratio represents that our algorithm finds more optimizations.
%
The results show that the \coam{} approach produces
well optimized circuits in short running times.


\myparagraph{Quality.}
We observe that in all but two cases (ham15 with 17 qubits and gf with 48 qubits),
using our \coam{} approach
discovers more optimizations than baseline \quartz{}.
%
For the hhl circuits,
the \coam{} algorithm reduces gate count by $23\%$ to $27\%$,
which is excellent considering that \quartz{} reduces the size by less than $5\%$
within the same time.
%
For the vqe family,
our \coam{} algorithm reduces the gate count by around $60\%$ and
the optimizations by \quartz{} are less than $10\%$.
%
Overall, we observe that by using \coam{} algorithm with \quartz{} as an oracle,
we can effectively reduce gate count for circuits with thousands of gates
within seconds and optimize circuits with hundreds of thousands of gates within minutes
(the Time column displays the running time).
%
In the Appendix,
we verify that our optimizer \coamwith{\quartz{}} does not generate a worse quality circuit
even when the running time for both algorithms is scaled
by $100$x (by increasing the per call timeout 100x; see \secref{methodology} for more details on running time).

\myparagraph{Scalability.}
Note that our \coam{} optimizer
excels at finding optimizations for large circuits.
%
The figure illustrates this using the ``S/Q'' column,
which computes the optimization ratio of both approaches.
%
For all families, the optimization ratio increases with increasing circuit size.
%
In the case of hhl circuits, for example,
the ratio rises from around $5$x to $1000$x with increasing circuit size;
%
In the case of grover circuits,
the optimization ratio steadily increases from $1.12$x on the smallest instance (7 qubits)
to $54.29$x on the largest instance (15 qubits).
%
Similarly, for vqe, the ratio increases from $6.5$x to $44.34$x with increasing circuit size
and for qft, it increases from $1.78$x to $5.19$x.
%
We identify three key reasons for this scalability.
%
First, because baseline \quartz{} searches for optimizations on the whole circuit,
it struggles to find optimizations,
because the search space is exponential.
%
Second, our optimizer \coam{} algorithm
utilizes \quartz{} by focusing it on small segments ($\Omega = 6$),
where it delivers excellent results.
%
Third,
the \coam{} algorithm ensures that it applies \quartz{} to all
$\Omega-$segments and misses no local optimizations.

\myparagraph{Summary.}
The experiments demonstrate that our \coam{} algorithm scales with circuit sizes
when using \quartz{} as the oracle.
%
The results suggest that our algorithm uses \quartz{} effectively,
finding significant reductions in circuit size and producing good quality circuits.
%

%

% For example,
% across different sizes of grover circuits,
% the \coam{} algorithm reduces gate count consistently by $10\%$;
% in contrast the gate count reduction by \quartz{} drops from $9\%$ to $0\%$.
%

%
% The 'S/Q' column shows the improvement
% in optimization rates due to \coam{}, i.e.,
% it shows how many more optimizations (per second)
% the \coam{} algorithm identifies compared to \quartz{}.
% %
% %
% Compared to \quartz{},
% the \coam{} algorithm yields $1.78$x and $5.19$x more optimizations per second
% for the smallest and largest qft instances
% respectively (see the ratio column in \figref{comp-quartz}).
% %
% Similarly,
% in the case of vqe,
% the gap in their optimization rates
% rises from around $2$x on the smallest instance to $42$x
% on the largest instance.

% %
% This is because the efficiency of \quartz{},
% quantified by optimization rates,
% reduces with increasing circuit sizes,
% whereas the \coam{} algorithm scales to larger sizes.

% Across the board,
% we observe that the optimization ratio is never less than one,
% establishing that the \coam{} approach never generates a worse quality circuit
% in the same running time.
% %
% For instance,



% we first optimize all circuits with $\coamwith{\quartzt{t}}$, where each oracle call is capped by a
% fixed amount of time $t$, and record how long the entire algorithm takes to
% complete.
% %
% Then,
% we run the default \quartz{} on the same input circuit for the same end-to-end
% time,
% %
% and compare the resulting circuit quality and optimization rate.


% number of gates optimized per second by
% \coam{} using \quartz{} as an oracle is higher than just running \quartz{}
% alone.

% % when using \quartz{} as an oracle,
% % \coam{} is able to accelerate the \defn{optimization rate} of \quartz{}.
% %

% %
% As a result, \coam{} is able to deliver better quality circuits within
% a given time limit.

% , due to its combination of linear time complexity and
% $\Omega$-optimality guarantee.
%


% \figref{comp-quartz} shows the result of this comparison
% using the configuration $\coamwith{\quartzt{0.06}}$, i.e., where
% each oracle call is limited to $0.06$ seconds.
% %
% The figure shows the input circuit sizes
% and displays the circuit sizes after optimization.
% %
% The figure labels the results of the \coam{} configuration as ``S'' and
% the standard \quartz{} approach as ``Q''.
% %
% In the cases where one approach performs better,
% the figure uses bold numbers, with lower numbers indicating better circuit quality.
% %
% The `Q/S' ratio column quantifies the improvement in circuit quality
% using the \coam{} algorithm w.r.t. standard \quartz{} (higher is better).
% %
% The figure also provides and compares the \emph{optimization rate} of both
% approaches, where the optimization rate is the number of gates optimized per
% second of execution.
% %
% A higher rate indicates faster optimizations.
% %
% The time column shows the execution time for both cases.



% \myparagraph{Quality.}
% We observe that in seventeen cases,
% using the \coam{} algorithm improves the quality of circuits w.r.t. standard \quartz{}
% and sometimes does so by a wide margin.
% %
% In the other seven cases,
% both approaches output the same quality of circuits.
% %
% For the hhl circuits,
% the \coam{} algorithm finds reductions ranging from $23\%$ to $27\%$,
% where \quartz{} does not find many optimizations
% within this time (less than $5\%$).
% %
% In the case of grover circuits,
% the \coam{} algorithm optimizes gate count by $10\%$ across the various sizes.
% %
% However, the efficacy of \quartz{} reduces from $9\%$ to $0\%$ with increasing sizes.
% %
% In the qpe circuits,
% neither approach finds any optimizations.
% %
% %
% For the vqe family,
% the \coam{} algorithm reduces the gate count by around $60\%$ and
% the optimizations by \quartz{} are less than $10\%$.
% %
% On average,
% the outputs of the \coam{} configuration are smaller by $1.37$x,
% when compared to the outputs of standard \quartz{}.

% \myparagraph{Scalability.}
% Across the board,
% we observe that the gap between the two approaches widens with increasing circuit sizes.
% %
% This is because the efficiency of \quartz{},
% quantified by optimization rates,
% reduces with increasing circuit sizes,
% whereas the \coam{} algorithm scales to larger sizes.

% For example,
% across different sizes of qft,
% the \coam{} algorithm achieves optimization rates
% ranging from $50$ to $85$ and the rates in fact increase as the circuit size grows.
% %
% In contrast,
% the optimization rate for \quartz{} reduces from around $28$ to $16$.
% %
% The 'S/Q' column shows the improvement
% in optimization rates due to \coam{}, i.e.,
% it shows how many more optimizations (per second)
% the \coam{} algorithm identifies compared to \quartz{}.
% %
% %
% Compared to \quartz{},
% the \coam{} algorithm yields $1.78$x and $5.19$x more optimizations per second
% for the smallest and largest qft instances
% respectively (see the ratio column in \figref{comp-quartz}).
% %
% Similarly,
% in the case of vqe,
% the gap in their optimization rates
% rises from around $2$x on the smallest instance to $42$x
% on the largest instance.
% %
% On average,
% we observe that the \coam{} algorithm finds $7.35$x many more optimizations
% than \quartz{} per second.


% All families of circuits follow a similar trend:
% the optimization rate ratio between the \coam{} approach and the \quartz{} optimizer
% increases with the circuit size,
% demonstrating the scalability advantages of the \coam{} algorithm.
% %
% This scalability advantage of the \coam{} approach is built into the algorithm
% because it calls \quartz{} only on small circuits,
% where \quartz{} delivers excellent results.
% %
% The algorithm never sends large circuits to \quartz{},
% where \quartz{} struggles
% because it chases potential optimizations in large spaces.
% %
% Because the \coam{} algorithm runs in linear time,
% it delivers good scalability as circuit sizes increase.
% %
% %
% %
% Because the execution time is equal for both approaches,
% the ratio column additionally represents the ratio of total optimizations.
%
% %
% For example,
% consider the ratio column of \figref{comp-quartz} which compares the optimization rates
% of the \coam{} algorithm with \quartz{}.
%

% First, because they can take a very long time,
% existing super op- timizers such as Quartz are used with a hard deadline (e.g., several hours)
% by which they have to be terminated. When not run to completion,
% they are unable to offer any quality guarantees whatsover, because they can get “lost” chasing potential optimizations
% in exponentially large search spaces.


% Second, most circuit optimizations naturally involve a small number of contiguous gates.
% Our algorithm (provably) does not miss such optimizations, but other optimizers could.
% \myparagraph{Consistency.}
% Since the \coam{} algorithm splits the circuit into pieces
% and melds them together,
% it is important to evaluate whether
% splitting and melding lose any optimizations in practice.
% %
% In theory, our algorithm guarantees $\Omega-$optimality.
% %
% To evaluate this guarantee,
% we compare to standard \quartz{} with extended running times.
% %
% We extend the running time by increasing the per-call timeout to \quartz{}
% to $0.6$s, i.e.,
% we consider the configuration \coamwith{\quartzt{0.6}}.
% %
% We note that the end-to-end running time becomes at least ten fold in this configuration,
% and we run the standard \quartz{} for the extended time.
% %
% This ensures that \quartz{} has a larger amount of
% time to find optimizations.
% %
% We present these results in the Appendix, and summarize them here.
% % /
% Overall, the gap between both approaches reduces with extended running time
% because when optimizers operate for longer times,
% their optimization rates diminish due to the
% increasing difficulty of finding further optimizations~\cite{quartz-2022, queso-2023}.
% %
% This extended running time allows \quartz{} to somewhat catch up to the \coam{}.
% %
% However, \coam{} never generates a worse quality circuit.
% %
% We also increase the running time further by ten fold,
% verifying that \coam{} consistently delivers better quality circuits.
% %
% We conclude from these experiment with extended running times
% that $\Omega$-optimality is a good quality guarantee because,
% in practice,
% the \coam{} algorithm never generates a worse quality circuit.
% %



%
% Overall, we note that the gap between the approaches has reduced,
% when compared to the previous configuration.
% %
% This occurs because as optimizers operate for longer times,
% their optimization rates diminish due to the
% increasing difficulty of finding further optimizations~\cite{quartz-2022, queso-2023}.
% %
% The difference in optimization rates between \figref{comp-quartz} and \figref{comp-queso}
% exemplifies this.
% %
% For example, the optimization rate in vqe\_n12 for \quartz{} reduces from around $30$ to $12$
% when its execution time increases from $37$ seconds to $640$ seconds.
% %
% The many fold extension of execution time decreases the optimization rates of both approaches
% and moderates the scalability advantages of the \coam{} algorithm.
% %
% On average,
% circuits generated by the \coam{} algorithm are $1.1$ times smaller
% than those generated by \quartz{}.
% %/
% In our Supplementary,
% we include a third configuration (\coamwith{\quartzt{6}})
% where we further increase the time ten fold and observe a similar trend,
% where \coam{} consistently delivers better quality circuits.
% %
% We conclude from these experiment with extended running times
% that $\Omega$-optimality is a good quality guarantee because,
% in practice,
% the \coam{} algorithm never generates a worse quality circuit.
%

\subsection{\coam{} with the \queso{} optimizer}
\label{sec:comp-queso}
% guarantees $\Omega$-optimality.
%
In this section, we evaluate our optimizer $\coamwith{\quesot{0.005}}$,
which runs our \coam{} algorithm using \queso{} as the oracle.
%
Our optimizer depth uses segment size $\Omega = 6$
and gives each call to \queso{} is a timeout (see \secref{methodology} for the more details).
%
We run $\coamwith{\quesot{0.005}}$,
or \coam{} for short,
on all the circuits and record
the output quality and running time.
%
We then run default \queso{} on each input circuit for the same end-to-end time,
%
and evaluate the number of optimizations.


\begin{figure}
  \centering
  \small
  \input{fig/prelim.queso.0.005.tex}
  \caption{
  The figure compares the performance of our $\coamwith{\quesot{0.005}}$ optimizer with standard \queso{}.
  %
  The label ``S'' represents the number of optimization discovered by our \coam{} approach
  and the label ``Q'' denotes optimizations found by \queso{}.
  %
  The ``S/Q'' column measures how many more optimizations \coam{} finds relative to \queso{};
  we avoid divide by zero issues by adding $+1$ optimization to both tools.
  %
  For the results in this figure, we impose an end-to-end timeout of ten hours.
  }
  \label{fig:comp-queso}
  % \setlength{\belowcaptionskip}{-10pt}
\end{figure}

\figref{comp-queso} shows the results of this experiment
for circuits from six families of quantum algorithms.
%
Each family is separated by a horizontal line
and contains circuits which differ number of qubits and are sorted by input size.
%
The figure shows the number of optimizations performed by our \coam{} approach and by \queso{}
in the columns labeled ``S'' and ``Q'' respectively;
the columns also list the percentage of gates removed in parentheses.
%
The figure uses bold numbers when one tool finds more optimizations than the other.
%
The time column shows the running time of each benchmark.
%
The results show that our optimizer consistently finds significant reductions
in gate count, across all families and circuit sizes.

%
\myparagraph{Quality.}
Across the board, we observe that using \queso{} with our \coam{} algorithm discovers
more optimizations than baseline \queso{}.
%
For the gf circuits,
the \coam{} approach reduces the gate count by $54\%$ the large instance (96 qubits)
and \queso{} does not discover any optimizations in same the running time.
%
For the vqe circuits,
our \coam{} algorithm delivers excellent results,
reducing the gate count by around around $60\%$ on all instances;
\queso{} reduces the gate count of the smallest instance by $48\%$ but
does not find optimizations for others in this amount of running time.
%
%
For the qft circuits, both approaches find similar reductions in the gate count.
%
Overall, we see that using \queso{} with the \coam{} algorithm finds substantial
reductions in gate count, across a range of quantum algorithms and circuit sizes.
%

\myparagraph{Scalability.}
The figure also shows that our \coamwith{\queso} optimizer scales well with circuit size.
%
The column ``S/Q'' computes the ratio of optimizations found by the tools,
and the ratio typically increases with circuit size.
%
For example,
in the case of ham circuits,
the ratio increases from 1.19x to 2x with increasing circuit size.
%
For grover circuits,
the optimization ratio increases from $1.3$x to $72$x.
%
Similarly, for hhl circuits, the ratio increases from 1.21x on the smallest instance (7 qubits)
to 1.94x on the medium sized instance (9 qubits);
for the largest instance of hhl (11 qubits),
using \queso{} with our \coam{} algorithm finds 17\% reduction and baseline \queso{}
does not discover any optimizations.
%
Similarly, \coam{} delivers increasing optimization ratios for the ``vqe'' family.
%

\myparagraph{Summary.}
The results show that many optimizations are local
and are found by our algorithm because it focuses \queso{} on small segments.
%
Our algorithm's approach to optimize circuits in a piecewise fashion and melding them together
finds significant reductions using \queso{} as the oracle.

% Because \coamwith{\queso} finds these optimizations by only sending segments of size $2\Omega$ to \queso{},
% the results demonstrate that many optimizations are local
% and can be found by focusing the baseline optimizer on small segments.

% The evaluation suggests that the \coam{} algorithm utilizes the \queso{} optimizer effectively,
% by splitting the circuit into small segments, optimizing them with \queso{} and finding
% the optimizations at the boundaries by melding the resulting circuits.




% \input{linearity}

\subsection{Experimenting with segment size}
\label{sec:var-segment}
\input{fig/segment}
In this section,
we evaluate the quality and efficiency guaranteed by the \coam{} algorithm
for different values of parameter $\Omega$.
%
We use our optimizer $\coamwith{\feyntool}$ for this evaluation,
which guarantees $\Omega-$optimality relative to the \feyntool{} optimizer.

%
\figref{vary-segment} plots the output T count (number of T gates) and the running
time of the optimizer against $\Omega$.
%
The figure shows the results for $\Omega$ values $2, 5, 15, 30, 60, 120 \dots 7680$;
we present the full table in the Appendix.
%
The red dotted line in the plots
shows the results of the the baseline optimizer \feyntool{}.
%
For the experiment,
we run the our optimizer on the hhl circuit with $7$ qubits, which initially contains 61246 T gates.
%
The results show that for a wide range of $\Omega$ values,
our optimizer produces a similar quality circuit as the baseline $\feyntool$
and typically does so in significantly less time
(at the extremities, there are two values of $\Omega$ for which \coam{} takes more time: $2$ and $7680$).
%

%
\myparagraph{T count.}
The plot for T count shows that when $\Omega$ is small (around $2$),
increasing it has quality benefits.
%
This is because quality guarantee of the $\coam{}$ algorithm becomes
stronger with increasing $\Omega$ as it requires larger segments to be optimal.
%
%
However, the benefits of increasing $\Omega$
become very incremental especially when $\Omega$ reaches around $60$,
where T count reaches around 42140 (20 gates away from being optimal).
%
This shows that $\Omega-$optimality is a good quality criterion,
as it generates good quality circuits
even with relatively small values of $\Omega$ (around $60$).

\myparagraph{Run time.}
One would perhaps expect that the running time of \coam{}
increases by increasing the segment size $\Omega$ because
1) each oracle call operates on larger segments
and 2) the algorithm generates a better quality circuit (provably and practically).
%
Indeed, the intuition is correct, for a majority of the values.
%
For values of $\Omega$ ranging from $120$ to $7860$,
the running time of the algorithm increases with increasing $\Omega$.
%
In this range,
the (non-linear) complexity of the oracle dominates the running time,
and it is faster to split, optimize and meld, calling the oracle many times
on smaller segments,
instead of querying the oracle on larger segments.


But, when $\Omega$ is very small,
we observe the opposite, i.e.,
increasing $\Omega$ reduces the running time.
\begin{wrapfigure}{r}{0.4\textwidth}
  \centering
  \includegraphics[width=0.39\textwidth]{omega_vs_time_zoom.png}
  \caption{Zooming in: Time vs. Omega plot}
  \label{fig:zoom-plot}
\end{wrapfigure}
%
For reference,
we draw \figref{zoom-plot},
which zooms the running time plot from \figref{vary-segment}
for initial values of $\Omega$, ranging from $2, 5, 15 \dots 120$.
%
For these smaller values of $\Omega$,
even though each oracle call is cheap,
the number of oracle calls dominates the time cost.
%
The \coam{} algorithm splits the circuit into a large number of small segments
and queries the oracle on each one, making many calls to the optimizer.
%
When a circuit segment is small,
it is more efficient to directly call \feyntool{},
which optimizes it in one pass.
%
For this reason, $\Omega = 120$ is a good value for our optimizer $\coamwith{\feyntool{}}$,
as it does not send large circuits to the oracle,
and also does not split the circuit into a large number of really small segments.
%

Overall,
we observe that for a wide range of $\Omega$ values,
our \coam{} algorithm outputs good quality circuits
and does so in a shorter running time than the baseline.
%
\input{fig/fig_oracle_call_vs_input_size}


% Furthermore, it increases the number of meld operations
% and almost every meld of the algorithm finds optimizations,
% because the oracle optimizes the boundary segments in a piecewise fashion
% rather than finding optimizing them in one step.
%
%
% We measured that, for $\Omega = 2$,
% \coamwith{\feyntool} makes around ten thousand calls to the base optimizer \feyntool{},
% taking around four hundred seconds.
% %
% Thus, at the very start,
% increasing $\Omega$ reduces the running time because it reduces
% the number of oracle calls.
% %
% \figref{zoom-plot}
% The plot shows how the running time decreases with increasing the parameter.


% When the segment size becomes slightly larger, around $\Omega = 60$,
% the running time reduces to twenty seconds and does not vary much for
% some intermediate values.
% %
% For most intermediate values, around $\Omega = 30$ to $\Omega = 480$,
% we observe good time performance, where the algorithm takes around thirty seconds.
% %
% Beyond these intermediate values,
% the running time starts increasing because the algorithm sends larger segments to the oracle
% and oracle complexity becomes the dominating cost.
% %
% It is then much
% faster to split, optimize, and meld rather than use the oracle.

% When $\Omega$ is small, increasing it reduces the running time of the algorithm.
% %
% This is perhaps counterintuitive because small segment sizes
% generate a worse quality circuit and also use the oracle on smaller segments.
% %
% But, it reduces the number of oracle calls, which becomes the dominating cost in this case.
% %
% Furthermore, for small segment sizes,
% almost every meld is finding optimizations
% %




% Also note, that the initial T count for this circuit is 61246,
% implying that different values of $\Omega$ do not have a large impact on quality.
% %






% %
% But slowly the benefits become incremental and eventually $\Omega$ is large enough where
% the output of \feyntool{} matches the optimizer  $\coamwith{\feyntool}$,
% as shown with the dotted red line.
% To summarize,
% \figref{fig:comp-quartz} demonstrates that the \coam{} algorithm
% drastically improves the speed of optimization for each circuit.
% %
% It shows that the algorithm scales well with circuit size,
% achieving excellent optimization rates across a range of sizes.
% %
% \figref{fig:comp-queso} shows that this performance
%

%


% \input{fig/prelim2.0.01}



% To summarize,
% \figref{fig:comp-quartz} demonstrates that the \coam{} algorithm
% drastically improves the speed of optimization for each circuit.
% %
% It shows that the algorithm scales well with circuit size,
% achieving excellent optimization rates across a range of sizes.
% %
% \figref{fig:comp-queso} shows that this performance comes at no cost to circuit quality
% even with the extended runtime,
% as the \coam{} algorithm never generates a worse quality circuit.
% %


% \subsection{Scalable optimization using \coam{} with \queso{}}

% \begin{figure*}
%   \centering
%   \input{fig/r}
%   \caption{
%   The figure compares the performance of $\coamwith{\quesot{1}}$ against standard \queso{}.
%   %
% The label ``S'' represents $\coamwith{\quesot{1}}$ and the label ``Q'' represents \queso{}.
% %
% The figure compares the circuit sizes (lower is better) and the optimization rates (higher is better) of both approaches
% after running them for the same end-to-end time.
% }
%   \label{fig:comp-queso}
% \end{figure*}

% In this section,
% we evaluate the \coam{} algorithm using the \queso{} optimizer.
% %
% We integrate the \queso{} optimizer into our algorithm as an oracle
% and impose a one second time out for each call.
% %
% We note that \queso{} does not follow the given timeout strictly
% and often takes longer to run and return the result (around $4/5$ seconds per call).

% To evaluate the algorithm,
% we run it with \queso{} and compute the final circuit
% and the overall execution time, excluding time for file I/O (\secref{impl}).
% %
% Then, we execute default \queso{} on the whole circuit for the same total runtime
% and compare the quality of circuits produced.
% %
% For this experiment,
% we filter benchmarks based on their sizes and
% opt for benchmarks whose sizes are less than ten thousand gates.
% %
% This size limitation arises from file I/O overheads which make restrict our ability
% to run larger circuits within reasonable times.

% \figref{comp-queso} shows the results of the evaluation for seven benchmarks
% coming from four families of algorithms.
% %
% The ``QS'' column denotes \queso{} and the ``S'' column represents the \coam{} algorithm
% using \queso{} as the oracle.
% %
% In all cases, the \coam{} approach generates smaller circuits than the baseline \queso{}.
% %
% Similar to the case with \q{} (\secref{quartz}),
% we observe that the gap between the \coam{} approach and default \queso{} increases
% with circuit size.
% %
% Foe example,
% in the grover family,
% the ratio of optimization rate between \coam{} and \queso{}
% increases from $1.14$x for grover\_n7 to $1.4$x in grover\_n9.
% %
% For the circuit vqe\_n12,
% which is the largest circuit on the table,
% the final circuit size is $0.78$ times smaller compared to \queso{},
% which demonstrates the scalability of the \coam{} approach.
% %
% On average,
% the algorithm's circuits are $0.92$x smaller than those generated by \queso{}
% and the algorithm makes $1.27$x as many optimizations per second.
% %

% The evaluation demonstrates that the \coam{} algorithm
% improves the scalability of the \queso{} optimizer and
% consistently delivers better quality circuits.


% \input{prelim}

% \cleardoublepage
% \subsection{Eval half 2}
% \input{prelim2.tex}
% \subsection{Plots}
% \input{plots_greedy.tex}
% \cleardoublepage
% \subsection{Cliff Eval half 1}
% \input{prelim1.clifft}
% \cleardoublepage
% \subsection{Cliff Eval half 2}
% \input{prelim2.clifft}
% \subsection{Plots Cliff}
% \input{plots_greedy_cliff.tex}


==> fig/clifft.tex <==
\begin{tabular}{rcccccc}
  &   \multicolumn{2}{c}{Circuit Size} &  \multicolumn{2}{c}{T Count} & \multicolumn{2}{c}{CNOT Count}  \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
   Benchmark & Input & Output & Input & Output & Input & Output \\

 \midrule
  ham15-med                     &    1468 & 1305 (-11.1\%)    &    362 & 336 (-7.18\%)     &   398 & 372 (-6.53\%)   \\
  ham15-high                    &    5977 & 5377 (-10.04\%)   &   1511 & 1423 (-5.82\%)    &  1499 & 1457 (-2.8\%)   \\
  hhl\_n7            &  169819 & 153328 (-9.71\%)  &  63964 & 58973 (-7.8\%)    &   880 & 782 (-11.14\%)  \\
  hhl\_n9            & 1919962 & 1856308 (-3.32\%) & 721843 & 717290 (-0.63\%)  & 11968 & 11856 (-0.94\%) \\
  gf2\^{}16\_mult                   &    4295 & 4272 (-0.54\%)    &   1040 & 1040 (0.0\%)      &  1581 & 1558 (-1.45\%)  \\
  gf2\^{}32\_mult                   &    9226 & 5102 (-44.7\%)    &   1028 & 1028 (0.0\%)      &  6299 & 2237 (-64.49\%) \\
  grover\_n7         &    4114 & 3675 (-10.67\%)   &   1064 & 1046 (-1.69\%)    &   912 & 904 (-0.88\%)   \\
  grover\_n9         &   14768 & 13109 (-11.23\%)  &   3927 & 3781 (-3.72\%)    &  3366 & 3294 (-2.14\%)  \\
  grover\_n11        &   44546 & 40142 (-9.89\%)   &  12005 & 11853 (-1.27\%)   & 10290 & 10240 (-0.49\%) \\
  grover\_n15        &  295378 & 267935 (-9.29\%)  &  80514 & 80326 (-0.23\%)   & 69012 & 68949 (-0.09\%) \\
  qft\_n48           &  533171 & 443566 (-16.81\%) & 209266 & 173926 (-16.89\%) &  1572 & 1572 (0.0\%)    \\
  qft\_n64           &  762887 & 671736 (-11.95\%) & 299675 & 263797 (-11.97\%) &  2236 & 2236 (0.0\%)    \\
  qft\_n80           &  991797 & 902605 (-8.99\%)  & 390035 & 354305 (-9.16\%)  &  2900 & 2900 (0.0\%)    \\
  qft\_n96           & 1222936 & 1135932 (-7.11\%) & 480571 & 446235 (-7.14\%)  &  3564 & 3564 (0.0\%)    \\
  qpe\_n8  &    5509 & 5243 (-4.83\%)    &   1842 & 1721 (-6.57\%)    &   798 & 797 (-0.13\%)   \\
  qpe\_n10 &   21130 & 21096 (-0.16\%)   &   6954 & 6871 (-1.19\%)    &  3315 & 3315 (0.0\%)    \\
  vqe\_n12           &   73927 & 59065 (-20.1\%)   &  21838 & 21844 (0.03\%)    &  2400 & 1959 (-18.38\%) \\
  vqe\_n16           &  142711 & 114301 (-19.91\%) &  41678 & 41704 (0.06\%)    &  5712 & 5241 (-8.25\%)  \\
  vqe\_n20           &  234541 & 188126 (-19.79\%) &  67888 & 67905 (0.03\%)    & 11136 & 10655 (-4.32\%) \\
  vqe\_n24           &  348969 & 280835 (-19.52\%) & 100187 & 100386 (0.2\%)    & 19184 & 18590 (-3.1\%)  \\
 \midrule
 \textbf{geomean} & & 12.48\% & & 4.08\% & & 6.26\%
 \end{tabular}

==> fig/fig-meld-diagram.tex <==
\begin{figure}
\includegraphics[width=0.6\linewidth]{media/meld-diagram.pdf}
\caption{Illustration of the meld operation, with inputs at the bottom at
output at the top. The inputs must be $\Omega$-optimal, and meld guarantees
the output is $\Omega$-optimal.}
\label{fig:meld-diagram}
\end{figure}

==> fig/fig-meld.tex <==
\begin{figure}[!htp]
\centering


\definecolor{mPurple}{rgb}{0.58,0,0.82}
\lstset{
  basicstyle=\footnotesize\fontfamily{ttfamily}\selectfont, % set the font
  keywordstyle={\color{mPurple}}, % set the keyword style
  morecomment=[l]{//},
  commentstyle=\rmfamily\slshape,
  % commentstyle=\itshape, % set the comment style
  showstringspaces=false, % don't show spaces in strings
  columns=fullflexible, % use proportional spacing
  morekeywords={fun,func,let,val,in,end,case,of,SOME, NONE, and, structure, if, else, then, return, def}, % define additional keywords
  mathescape=true, % enable math mode
  keepspaces=true,
  breaklines=true,
  numbers=left,
  xleftmargin=20pt
}

\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting}[escapechar=@]
$\Omega$: int
Oracle: circuit $\rightarrow$ circuit
cost: circuit $\rightarrow$ int

def meld$(C_1, C_2)$:
  $d_1, d_2$ = (depth($C_1$), depth($C_2$))
  $W$ = $C_1 [d_1 - \Omega : d_1] + C_2 [0 : \Omega]$ @\label{line:combine}@
  $W'$ = Oracle$(W)$
  if $\costof{W'} = \costof{W}$:
    return $C_1 + C_2$
  else:
    $M$ = meld$(C_1[0 : d_1 - \Omega], W')$
    return meld ($M, C_2[\Omega : d_2]$)@
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting}[firstnumber = 14, escapeinside={@}{@}]
def $\mathsf{SOAM}$($C$):
  $d$ = depth$(C)$
  if $d \leq 2\Omega$:
    return Oracle$(C)$
  else:
    $m$ = $\lfloor d/2 \rfloor$
    $C_1$, $C_2$ = ($C[0 : m]$, $C[m : d]$)
    $C_1'$ = $\mathsf{SOAM}$($C_1$)
    $C_2'$ = $\mathsf{SOAM}$($C_2$)
    return meld$(C_1', C_2')$@
\end{lstlisting}
\end{minipage}

\caption{
The function $\mathsf{SOAM}$ shows the algorithm for optimizing a circuit
$C$, using an off-the-shelf oracle optimizer, such that the circuit is
$\Omega-$optimal w.r.t. the oracle.
%
It uses the function $\mathsf{meld}$, which takes two $\Omega$-optimal
circuits and merges them such that the result is $\Omega$-optimal.
%
}
% \vspace{-1.5in}
\label{fig:algo}
\end{figure}



==> fig/fig-overlap.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{media/overlap.pdf}
\caption{
The figure shows a circuit in the layer representation
and defines $\Omega-$optimality.
%
$\Omega-$optimality requires that all $\Omega-$segments are optimal relative
a given oracle optimizer.
%
An $\Omega-$segment $W_i$ starts at layer $i$ and goes up layer $i + \Omega$.
%
The dashed lines are separated by $\Omega$ layers.
%
To verify $\Omega$-optimality, an algorithm must check that every $\Omega-$segment
is optimal (relative to the oracle).
%
% Confirming $\Omega$-optimality using many overlapping $2\Omega$-segments.
% Every possible $\Omega$-segment
% (for example, two such segments are highlighted in red) is entirely contained
% within at least one $2\Omega$-segment sent to the oracle.
}
\label{fig:overlap}
\end{figure}

==> fig/fig-ref-algo.tex <==

\definecolor{mPurple}{rgb}{0.58,0,0.82}
\lstset{
  language=SML, % set the programming language
  basicstyle=\footnotesize\fontfamily{ttfamily}\selectfont, % set the font
  keywordstyle={\color{mPurple}}, % set the keyword style
  commentstyle=\itshape, % set the comment style
  showstringspaces=false, % don't show spaces in strings
  columns=fullflexible, % use proportional spacing
  morekeywords={fun,let,val,in,end,case,of,SOME, NONE, and, structure, if, else, then, return}, % define additional keywords
  mathescape, % enable math mode
  breaklines=true,
  numbers=left,
  xleftmargin=15pt
}

\begin{lstlisting}[escapechar=@]
val $\Omega$ : int
val $\mathrm{opt}$ : circuit $\rightarrow$ circuit
val allSubckts : (circuit * int) $\rightarrow$ circuit list

fun optimize ($c$) =
  subckts = allSubckts($c$, $\Omega$)
  for (sbckt : subckts) {
    subckt' = $\mathsf{opt}$(subckt)
    if ($\mathsf{cost}$ (subckt') < $\mathsf{cost}$(subckt)) {
      c' = c[subckt'/subckt]
      return optimize ($c'$)
    }
  }

fun absorb (copt, crem) =
  $p_1 + s_1$ = copt
  $p_2 + s_2$ = crem
  wd = $(s_1 + p_2)$
  wd' = $\mathsf{opt} (s_1 + p_2)$
  if wd = wd' then
    return absorb ($p_1 +$  wd, $s_2$)
  else
  // this wastes work, because it dissects wd' piece by piece.
  return absorb (absorb($p_1$, wd'), $s_2$)
  // this is ok.
  return absorb (meld($p_1$, wd'), $s_2$)

\end{lstlisting}

% \begin{lstlisting}
% fun meld (c1, c2) =
%   let
%     val (c1s, c1p) = C.splitEnd (c1, $\Omega$)
%     val c2' = C.merge (c1p, c2)
%   in
%     case opt_prefix (2*$\Omega$, c2') of
%       SOME c2'' => meld (c1s, c2'')
%     | NONE => C.merge (c1, c2')
%   end

% and fun opt_prefix (prefix_size, c) =
%   let
%     val (cp, cs) = C.split (c, prefix_size)
%   in
%     case $\mathcal{O}$(cp) of
%       SOME cp' => SOME (meld (cp', cs))
%     | NONE => NONE
%   end
% \end{lstlisting}


==> fig/fig-rewrite-converge.tex <==
\begin{figure}
\[
\begin{array}{c}

\infer[]
{
  \locallyopt\Omega{C}
}
{
  C \Downarrow^\Omega C
}

\quad

\infer[]
{
  \localstep \Omega C {C'}
  \\
  C' \Downarrow^\Omega C^\text{OPT}
}
{
  C \Downarrow^\Omega C^\text{OPT}
}

\end{array}
\]
\caption{Rewrites converging upon a locally optimal circuit.}
\label{fig:rewrite-converge}
\end{figure}

==> fig/fig-unopt.tex <==
\begin{figure}[!htp]
  \input{fig/fig-ref-algo.tex}
  \caption{ Reference algorithms}
  % \vspace{-1.5in}
  \label{fig:wd-opt}
  \end{figure}



==> fig/fig_quadratic_lower_bound.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{media/quadratic_lower_bound.pdf}
    \vspace{-20pt}
    \caption{A worst case example showing why linear number of compressions are needed.}
    \label{fig:quadratic_lower_bound}
    % \vspace{-15pt}
\end{figure}


==> fig/linearity.tex <==
\begin{figure}
	\centering

	\subfloat[Grover]{\includegraphics[width=0.5\columnwidth]{plots/linearitygrover0.01.png}}
	\subfloat[VQE]{\includegraphics[width=0.5\columnwidth]{plots/linearityvqe0.01.png}}

	\subfloat[VPE]{\includegraphics[width=0.5\columnwidth]{plots/linearityshor0.01.png}}
	\subfloat[QFT]{\includegraphics[width=0.5\columnwidth]{plots/linearityqft0.01.png}}

	\caption{
	\textbf{X-axis: circuit size in thousands.}
	\textbf{Y-axis: time in seconds.}
	The figure plots the optimization times for four quantum algorithms
	against the corresponding circuit sizes.
	The figure confirms that our algorithm scales linearly with the size of the circuit.
	}
	\label{fig:linear}

\end{figure}


% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.9\columnwidth]{plots/linearity0.01.png}\quad
% 	\scriptsize
% \caption{
% 	The figure plots the optimizer times for five quantum algorithms
% 	as their size varies.
% 	%
% 	The X-axis shows the relative size of a circuit for each algorithm.
% 	%
% 	The Y-axis shows the time taken to optimize the circuit.
% 	%
% 	The figure confirms that our algorithm scales linearly with the size of the circuit.
% }
% \end{figure}

==> fig/plots.tex <==
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/adder_8.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/barenco_tof_10.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/barenco_tof_3.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/barenco_tof_4.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/barenco_tof_5.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/csla_mux_3.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/csum_mux_9.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/grover_5.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/grover_n15_from_python.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/grover_n21_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/grover_n3_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/grover_n5_from_python.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/grover_n9_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/ham15-high.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/ham15-low.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/ham15-med.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/hhl_n10.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/hhl_n11_from_python.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/hhl_n13_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/hhl_n5_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/hhl_n7.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/hhl_n7_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/hhl_n9_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/hwb6.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/mod5_4.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/mod_adder_1024.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/mod_mult_55.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/mod_red_21.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/multiplier_n45.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/multiplier_n75.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/qaoa_n24_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/qaoa_n6.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/qaoa_n6_from_python.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/qaoa_n8_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/qcla_com_7.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/qcla_mod_7.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/qft_n160.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/qft_n16_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/qft_n18.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/qft_n24_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/qft_n29.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/qft_n30_from_python.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/qft_n320.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/qft_n4_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/qft_n63.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/qft_n8_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/rc_adder_6.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/shor_7_mod_15_n12_from_python.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/shor_7_mod_15_n16_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/shor_7_mod_15_n8_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/tof_10.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/tof_3.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/tof_4.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/tof_5.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/vbe_adder_3.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/vqe_n16_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/vqe_n24.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/vqe_n24_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/vqe_n28_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/vqe_n4_from_python.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/vqe_n6_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/vqe_n8_from_python.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/vqe_uccsd_n28.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.3\linewidth]{plots/vqe_uccsd_n4.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/vqe_uccsd_n6.inset.png}\quad
	\includegraphics[width=0.3\linewidth]{plots/vqe_uccsd_n8.inset.png}\quad
\caption{Size vs. Time plots}
\end{figure*}

==> fig/prelim.0.005.tex <==
\begin{tabular}{rrrrrrrr}
  &   \multicolumn{3}{c}{Circuit Size} &  \multicolumn{3}{c}{Optimization Rate} &  \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
   Name & Original & Quartz & Lopt & Quartz &   Lopt & Ratio  & Time (s) \\

 \midrule
  ham15-med       &   1061 & 899 (-15\%)  & \textbf{869} (-18\%)    & 26.24 &  31.1  & 1.18x  &    6.1746  \\
  ham15-high      &   4365 & 3597 (-18\%) & \textbf{3373} (-23\%)   & 26.85 &  34.69 & 1.28x  &   28.5988  \\
  hhl\_n7         &   5319 & 5000 (-6\%)  & \textbf{3878} (-27\%)   & 28.26 & 127.66 & 4.4x   &   11.2879  \\
  hhl\_n9         &  63392 & 63238 (0\%)  & \textbf{47714} (-25\%)  &  1.13 & 115.21 & 54.56x &  136.081   \\
  hhl\_n11        & 629247 & 629096 (0\%) & \textbf{484809} (-23\%) &  0.08 &  77.83 & 72.99x & 1855.81    \\
  gf2\^{}16\_mult &   2694 & 2694 (0\%)   & 2694 (0\%)              &  0    &   0    & 1.0x   &    9.20895 \\
  gf2\^{}32\_mult &   7553 & 5495 (-27\%) & \textbf{3429} (-55\%)   & 24.37 &  48.84 & 1.96x  &   84.4336  \\
  grover\_n7      &   2479 & 2257 (-9\%)  & \textbf{2227} (-10\%)   & 23.47 &  26.64 & 1.13x  &    9.45873 \\
  grover\_n9      &   8968 & 8902 (-1\%)  & \textbf{8092} (-10\%)   &  2.19 &  29.11 & 9.44x  &   30.0916  \\
  grover\_n11     &  27136 & 27031 (0\%)  & \textbf{24493} (-10\%)  &  1.3  &  32.6  & 14.61x &   81.0636  \\
  grover\_n15     & 180497 & 180195 (0\%) & \textbf{162909} (-10\%) &  0.56 &  32.36 & 21.38x &  543.551   \\
  qft\_n48        &   4626 & 3944 (-15\%) & \textbf{3870} (-16\%)   & 39.95 &  44.29 & 1.11x  &   17.0702  \\
  qft\_n64        &   7402 & 6566 (-11\%) & \textbf{5510} (-26\%)   & 25.42 &  57.52 & 2.21x  &   32.8908  \\
  qft\_n80        &  10690 & 9786 (-8\%)  & \textbf{7150} (-33\%)   & 18.15 &  71.09 & 3.76x  &   49.7953  \\
  qft\_n96        &  14490 & 13252 (-9\%) & \textbf{8790} (-39\%)   & 17.63 &  81.16 & 4.41x  &   70.2343  \\
  shor\_n8        &   2040 & 2040 (0\%)   & 2040 (0\%)              &  0    &   0    & 1.0x   &    4.9326  \\
  shor\_n10       &   8476 & 8476 (0\%)   & 8476 (0\%)              &  0    &   0    & 1.0x   &   20.5313  \\
  shor\_n12       &  34084 & 34084 (0\%)  & 34084 (0\%)             &  0    &   0    & 1.0x   &   78.4735  \\
  shor\_n14       & 136320 & 136320 (0\%) & 136320 (0\%)            &  0    &   0    & 1.0x   &  293.562   \\
  vqe\_n16        &  22374 & 21913 (-2\%) & \textbf{8031} (-64\%)   &  5.22 & 162.44 & 26.28x &   88.2949  \\
  vqe\_n24        &  59798 & 59053 (-1\%) & \textbf{24767} (-59\%)  &  2.45 & 115.27 & 33.7x  &  303.891   \\
  vqe\_n28        &  86894 & 86201 (-1\%) & \textbf{38111} (-56\%)  &  1.42 & 100.06 & 41.76x &  487.531   \\
 \midrule
 \end{tabular}

==> fig/prelim.0.01.tex <==
\begin{tabular}{rcccccc}
  &  &  & \multicolumn{3}{c}{Number of optimizations} &  \\ \cmidrule(lr){4-6}
   Family & Qubits & Input Size & Q & S & S/Q & Time (s) \\


  \midrule\multirow{2}{*}{ham15}  & 17 &   1061 & 202 (19\%)  & 202 (19\%)             & 1.0x     &    8 \\
                          & 20 &   4365 & 342 (8\%)   & \textbf{992} (23\%)    & 2.9x     &   22 \\
  \midrule\multirow{3}{*}{hhl}    &  7 &   5319 & 290 (5\%)   & \textbf{1441} (27\%)   & 4.96x    &   10 \\
                          &  9 &  63392 & 145 (0\%)   & \textbf{15678} (25\%)  & 107.39x  &  130 \\
                          & 11 & 629247 & 131 (0\%)   & \textbf{144438} (23\%) & 1094.23x & 1702 \\
  \midrule\multirow{2}{*}{gf}     & 48 &   2694 & 0 (0\%)     & 0 (0\%)                & 1.0x     &    8 \\
                          & 96 &   7553 & 2078 (28\%) & \textbf{4124} (55\%)   & 1.98x    &  137 \\
  \midrule\multirow{4}{*}{grover} &  7 &   2479 & 224 (9\%)   & \textbf{252} (10\%)    & 1.12x    &    9 \\
                          &  9 &   8968 & 66 (1\%)    & \textbf{876} (10\%)    & 13.09x   &   28 \\
                          & 11 &  27136 & 105 (0\%)   & \textbf{2643} (10\%)   & 24.94x   &   78 \\
                          & 15 & 180497 & 323 (0\%)   & \textbf{17588} (10\%)  & 54.29x   &  583 \\
  \midrule\multirow{4}{*}{qft}    & 48 &   4626 & 424 (9\%)   & \textbf{756} (16\%)    & 1.78x    &   15 \\
                          & 64 &   7402 & 758 (10\%)  & \textbf{1892} (26\%)   & 2.49x    &   31 \\
                          & 80 &  10690 & 744 (7\%)   & \textbf{3540} (33\%)   & 4.75x    &   46 \\
                          & 96 &  14490 & 1098 (8\%)  & \textbf{5700} (39\%)   & 5.19x    &   66 \\
  \midrule\multirow{4}{*}{vqe}    & 12 &  11022 & 1127 (10\%) & \textbf{7407} (67\%)   & 6.57x    &   37 \\
                          & 16 &  22374 & 458 (2\%)   & \textbf{14343} (64\%)  & 31.25x   &   87 \\
                          & 20 &  38462 & 1019 (3\%)  & \textbf{23551} (61\%)  & 23.09x   &  166 \\
                          & 24 &  59798 & 789 (1\%)   & \textbf{35031} (59\%)  & 44.34x   &  316 \\

 \midrule
 \end{tabular}

==> fig/prelim.0.1.tex <==
\begin{tabular}{ccccccc}
  &  &  & \multicolumn{3}{c}{Number of optimizations} &  \\ \cmidrule(lr){4-6}
   Family & Qubits & Input Size & Q & S & S/Q & Time (s) \\


  \midrule\multirow{2}{*}{ham15}  & 17 &   1061 & 202 (19\%)   & 202 (19\%)             & 1.0x    &    97 \\
                          & 20 &   4365 & 992 (23\%)   & \textbf{1002} (23\%)   & 1.01x   &   383 \\
  \midrule\multirow{3}{*}{hhl}    &  7 &   5319 & 1443 (27\%)  & \textbf{1738} (33\%)   & 1.2x    &  1242 \\
                          &  9 &  63392 & 14739 (23\%) & \textbf{17950} (28\%)  & 1.22x   & 10803 \\
                          & 11 & 629247 & 1343 (0\%)   & \textbf{146256} (23\%) & 108.82x & 10798 \\
  \midrule\multirow{2}{*}{gf}     & 48 &   2694 & 0 (0\%)      & \textbf{3} (0\%)       & 4.0x    &   284 \\
                          & 96 &   7553 & 4124 (55\%)  & 4124 (55\%)            & 1.0x    &   380 \\
  \midrule\multirow{4}{*}{grover} &  7 &   2479 & 252 (10\%)   & 252 (10\%)             & 1.0x    &   229 \\
                          &  9 &   8968 & 876 (10\%)   & \textbf{877} (10\%)    & 1.0x    &   839 \\
                          & 11 &  27136 & 2649 (10\%)  & \textbf{2672} (10\%)   & 1.01x   &  2712 \\
                          & 15 & 180497 & 7710 (4\%)   & \textbf{17588} (10\%)  & 2.28x   & 10800 \\
  \midrule\multirow{4}{*}{qft}    & 48 &   4626 & 757 (16\%)   & \textbf{1102} (24\%)   & 1.46x   &  2217 \\
                          & 64 &   7402 & 1893 (26\%)  & \textbf{2366} (32\%)   & 1.25x   &  3329 \\
                          & 80 &  10690 & 3540 (33\%)  & \textbf{4144} (39\%)   & 1.17x   &  4272 \\
                          & 96 &  14490 & 5700 (39\%)  & \textbf{6448} (44\%)   & 1.13x   &  5236 \\
  \midrule\multirow{4}{*}{vqe}    & 12 &  11022 & 7407 (67\%)  & \textbf{7450} (68\%)   & 1.01x   &   619 \\
                          & 16 &  22374 & 14343 (64\%) & \textbf{14425} (64\%)  & 1.01x   &  1284 \\
                          & 20 &  38462 & 16061 (42\%) & \textbf{23604} (61\%)  & 1.47x   &  2002 \\
                          & 24 &  59798 & 10140 (17\%) & \textbf{35130} (59\%)  & 3.46x   &  3277 \\

 \midrule
 \end{tabular}

==> fig/prelim.1.tex <==
\begin{tabular}{ccccccc}
  &  &  & \multicolumn{3}{c}{Number of optimizations} &  \\ \cmidrule(lr){4-6}
   Family & Qubits & Input Size & Q & S & S/Q & Time (s) \\


  \midrule\multirow{2}{*}{ham15}  & 17 &   1061 & 202 (19\%)   & \textbf{260} (25\%)    & 1.29x   &  1198 \\
                          & 20 &   4365 & 992 (23\%)   & \textbf{1120} (26\%)   & 1.13x   &  6065 \\
  \midrule\multirow{3}{*}{hhl}    &  7 &   5319 & 1451 (27\%)  & \textbf{1859} (35\%)   & 1.28x   & 10767 \\
                          &  9 &  63392 & 14708 (23\%) & \textbf{16114} (25\%)  & 1.1x    & 10776 \\
                          & 11 & 629247 & 1338 (0\%)   & \textbf{144785} (23\%) & 108.13x & 10763 \\
  \midrule\multirow{2}{*}{gf}     & 48 &   2694 & 0 (0\%)      & \textbf{23} (1\%)      & 24.0x   &  3549 \\
                          & 96 &   7553 & 4124 (55\%)  & 4124 (55\%)            & 1.0x    &  3025 \\
  \midrule\multirow{4}{*}{grover} &  7 &   2479 & 252 (10\%)   & \textbf{270} (11\%)    & 1.07x   &  3066 \\
                          &  9 &   8968 & 876 (10\%)   & \textbf{1025} (11\%)   & 1.17x   & 10785 \\
                          & 11 &  27136 & 2649 (10\%)  & \textbf{2779} (10\%)   & 1.05x   & 10806 \\
                          & 15 & 180497 & 7700 (4\%)   & \textbf{17747} (10\%)  & 2.3x    & 10788 \\
  \midrule\multirow{4}{*}{qft}    & 48 &   4626 & 763 (16\%)   & \textbf{1119} (24\%)   & 1.47x   & 10786 \\
                          & 64 &   7402 & 1895 (26\%)  & \textbf{2259} (31\%)   & 1.19x   & 10805 \\
                          & 80 &  10690 & 3541 (33\%)  & \textbf{3906} (37\%)   & 1.1x    & 10810 \\
                          & 96 &  14490 & 5701 (39\%)  & \textbf{6046} (42\%)   & 1.06x   & 10763 \\
  \midrule\multirow{4}{*}{vqe}    & 12 &  11022 & 7407 (67\%)  & \textbf{7919} (72\%)   & 1.07x   & 10761 \\
                          & 16 &  22374 & 14343 (64\%) & \textbf{14828} (66\%)  & 1.03x   & 10771 \\
                          & 20 &  38462 & 23551 (61\%) & \textbf{23965} (62\%)  & 1.02x   & 10787 \\
                          & 24 &  59798 & 35031 (59\%) & \textbf{35474} (59\%)  & 1.01x   & 10775 \\

 \midrule
 \end{tabular}


==> fig/prelim.compress.tex <==
\begin{tabular}{ccccccc}
    &  &  & \multicolumn{3}{c}{Number of optimizations} &  \\ \cmidrule(lr){4-6} 
     Family & Qubits & Input Size & Q & S & S/Q & Time (s) \\ 
   
   
    \midrule\multirow{2}{*}{ham15}  & 17 &  1061 & 202 (19\%)  & 202 (19\%)            & 1.0x   &   3 \\
                            & 20 &  4365 & 800 (18\%)  & \textbf{992} (23\%)   & 1.24x  &  13 \\
    \midrule\multirow{2}{*}{hhl}    &  7 &  5319 & 373 (7\%)   & \textbf{1441} (27\%)  & 3.86x  &   8 \\
                            &  9 & 63392 & 260 (0\%)   & \textbf{15678} (25\%) & 60.07x & 113 \\
    \midrule\multirow{2}{*}{gf}     & 48 &  2694 & 0 (0\%)     & 0 (0\%)               & 1.0x   &   3 \\
                            & 96 &  7553 & 20 (0\%)    & 20 (0\%)              & 1.0x   &  41 \\
    \midrule\multirow{3}{*}{grover} &  7 &  2479 & 236 (10\%)  & \textbf{243} (10\%)   & 1.03x  &   6 \\
                            &  9 &  8968 & 618 (7\%)   & \textbf{858} (10\%)   & 1.39x  &  21 \\
                            & 11 & 27136 & 952 (4\%)   & \textbf{2604} (10\%)  & 2.73x  & 103 \\
    \midrule\multirow{4}{*}{qft}    & 48 &  4626 & 756 (16\%)  & 756 (16\%)            & 1.0x   &  12 \\
                            & 64 &  7402 & 1236 (17\%) & \textbf{1892} (26\%)  & 1.53x  &  20 \\
                            & 80 & 10690 & 1312 (12\%) & \textbf{3540} (33\%)  & 2.7x   &  33 \\
                            & 96 & 14490 & 1534 (11\%) & \textbf{5700} (39\%)  & 3.71x  &  51 \\
    \midrule\multirow{4}{*}{vqe}    & 12 & 11022 & 627 (6\%)   & \textbf{7407} (67\%)  & 11.8x  &  25 \\
                            & 16 & 22374 & 493 (2\%)   & \textbf{14343} (64\%) & 29.04x &  60 \\
                            & 20 & 38462 & 643 (2\%)   & \textbf{23551} (61\%) & 36.57x & 125 \\
                            & 24 & 59798 & 505 (1\%)   & \textbf{35031} (59\%) & 69.23x & 195 \\
   
   \midrule
   \end{tabular}

==> fig/prelim.feyn.grainless.tex <==
\begin{tabular}{cccccccccc}
  & &  & \multicolumn{3}{c}{Output T count and Ratio} &  \multicolumn{3}{c}{Time (s) and Speedup}  \\ \cmidrule(lr){4-6} \cmidrule(lr){7-9}
   Family & Qubits & Input T Count & F & S & F/S & F & S & F/S \\


  \midrule\multirow{4}{*}{hwb}    &   8 &    5887 & 4375   &   4375 & 1.0  &     4.1  &    3.19 &  1.29 \\
                          &  10 &   29939 & 21017  &  21017 & 1.0  &   250.77 &   24.63 & 10.18 \\
                          &  11 &   84196 & 57810  &  57810 & 1.0  &  4767.3  &  103.52 & 46.05 \\
                          &  12 &  171465 & 113023 & 113033 & 1.0  & 21880.4  &  252.47 & 86.67 \\
  \midrule\multirow{3}{*}{gf}     &  96 &    7168 & 5120   &   5172 & 0.99 &     3.96 &    3.99 &  0.99 \\
                          & 192 &   28672 & 20480  &  20612 & 0.99 &    71.24 &   75.73 &  0.94 \\
                          & 384 &  114688 & 81920  &  82322 & 1.0  &  5156.62 & 1040.91 &  4.95 \\
  \midrule\multirow{2}{*}{grover} &  11 &   12005 & 8155   &   8155 & 1.0  &     0.42 &    0.96 &  0.44 \\
                          &  15 &   80514 & 54670  &  54670 & 1.0  &     5.85 &    9.17 &  0.64 \\
  \midrule\multirow{2}{*}{hhl}    &   7 &   61246 & 42116  &  42148 & 1.0  &   409.78 &   22.45 & 18.25 \\
                          &   9 &  565183 & T.O.   & 372643 & N/A  & 36000    &  559.34 & 64.36 \\
  \midrule\multirow{4}{*}{qft}    &  48 &   44803 & 35731  &  35731 & 1.0  &   195.1  &   36.61 &  5.33 \\
                          &  64 &   61027 & 48659  &  48659 & 1.0  &   531.45 &   58.11 &  9.15 \\
                          &  80 &   77251 & 61587  &  61587 & 1.0  &  1083.36 &   87.94 & 12.32 \\
                          &  96 &   93475 & 74515  &  74515 & 1.0  &  1931.88 &  117.89 & 16.39 \\
  \midrule\multirow{4}{*}{shor}   &  12 &   20180 & 16086  &  16096 & 1.0  &    21    &    9.19 &  2.28 \\
                          &  14 &   70544 & 56070  &  56094 & 1.0  &   999.47 &   53.1  & 18.82 \\
                          &  16 &  266060 & 211254 & 211260 & 1.0  & 28382.3  &  307.86 & 92.19 \\
                          &  18 & 1042184 & T.O.   & 827432 & N/A  & 36000    & 2785.83 & 12.92 \\

 \midrule
 \textbf{geomean} & & & & & 1.0 & &  & 7.48 &
 \end{tabular}

==> fig/prelim.feyn.tex <==
\begin{tabular}{cccccccccc}
  & &  & \multicolumn{2}{c}{Time} & &  \multicolumn{2}{c}{T Count Reduction}  \\ \cmidrule(lr){4-5} \cmidrule(lr){7-8}
   Family & Qubits & Input T Count & \feyntool{} & \algname{} & \algname{} speedup & \feyntool{} & \algname{} \\


  \midrule\multirow{2}{*}{bwt}    & 17 & 169330 & 35730.0      & \textbf{354.8}  & 100.69 & -13.2\% & -13.2\% \\
                          & 21 & 214585 & 68301.4      & \textbf{569.1}  & 120.01 & -19.5\% & -19.4\% \\
  \midrule\multirow{4}{*}{grover} &  9 &   3927 & \textbf{2.6} & 3.3             &   0.79 & -31.2\% & -31.2\% \\
                          & 11 &  13720 & 12.0         & \textbf{10.5}   &   1.15 & -33.7\% & -33.7\% \\
                          & 13 &  36920 & 140.9        & \textbf{34.8}   &   4.05 & -33.1\% & -33.1\% \\
                          & 15 &  92016 & 2609.6       & \textbf{104.5}  &  24.97 & -32.7\% & -32.7\% \\
  \midrule\multirow{2}{*}{hhl}    &  7 &  61246 & 409.8        & \textbf{31.4}   &  13.03 & -31.2\% & -31.2\% \\
                          &  9 & 565183 & T.O.         & \textbf{535.4}  &  80.69 & T.O.    & -34.1\% \\
  \midrule\multirow{4}{*}{hwb}    &  8 &   5887 & \textbf{4.1} & 5.9             &   0.69 & -25.7\% & -25.7\% \\
                          & 10 &  29939 & 250.8        & \textbf{45.8}   &   5.48 & -29.8\% & -29.8\% \\
                          & 11 &  84196 & 4767.3       & \textbf{129.9}  &  36.7  & -31.3\% & -31.3\% \\
                          & 12 & 171465 & 21880.4      & \textbf{362.6}  &  60.35 & -34.1\% & -34.1\% \\
  \midrule\multirow{4}{*}{qft}    & 48 &  44803 & 195.1        & \textbf{77.1}   &   2.53 & -20.2\% & -20.2\% \\
                          & 64 &  61027 & 531.4        & \textbf{138.8}  &   3.83 & -20.3\% & -20.3\% \\
                          & 80 &  77251 & 1083.4       & \textbf{204.4}  &   5.3  & -20.3\% & -20.3\% \\
                          & 96 &  93475 & 1931.9       & \textbf{355.6}  &   5.43 & -20.3\% & -20.3\% \\
  \midrule\multirow{4}{*}{shor}   & 10 &   6104 & \textbf{2.0} & 4.0             &   0.51 & -19.7\% & -19.7\% \\
                          & 12 &  20180 & 21.0         & \textbf{16.5}   &   1.27 & -20.3\% & -20.3\% \\
                          & 14 &  70544 & 999.5        & \textbf{76.9}   &  12.99 & -20.5\% & -20.5\% \\
                          & 16 & 266060 & 28382.3      & \textbf{396.8}  &  71.53 & -20.6\% & -20.6\% \\
  \midrule\multirow{4}{*}{sqroot} & 42 &  25104 & 569.2        & \textbf{69.3}   &   8.21 & -37.4\% & -37.4\% \\
                          & 48 &  60366 & 5441.6       & \textbf{189.8}  &  28.67 & -39.9\% & -39.9\% \\
                          & 54 & 140830 & 36747.0      & \textbf{631.8}  &  58.16 & -41.7\% & -41.7\% \\
                          & 60 & 261308 & T.O.         & \textbf{1212.1} &  35.64 & T.O.    & -29.8\% \\

 \midrule
 \textbf{average} & & & & & 9.91 & -27.1\% & -27.5\%
 \end{tabular}

==> fig/prelim.queso.0.001.tex <==
\begin{tabular}{ccccccc}
  &  &  & \multicolumn{3}{c}{Number of optimizations} &  \\ \cmidrule(lr){4-6}
   Family & Qubits & Input Size & Q & S & S/Q & Time (s) \\


  \midrule\multirow{2}{*}{ham15}  & 17 &   1061 & 210 (20\%)   & \textbf{250} (24\%)    & 1.19x     &    35 \\
                          & 20 &   4365 & 650 (15\%)   & \textbf{1351} (31\%)   & 2.08x     &   138 \\
  \midrule\multirow{3}{*}{hhl}    &  7 &   5319 & 1501 (28\%)  & \textbf{1860} (35\%)   & 1.24x     &   213 \\
                          &  9 &  63392 & 10703 (17\%) & \textbf{16574} (26\%)  & 1.55x     & 16723 \\
                          & 11 & 629247 & 0 (0\%)      & \textbf{152846} (24\%) & 152847.0x & 17205 \\
  \midrule\multirow{2}{*}{gf}     & 48 &   2694 & 0 (0\%)      & 0 (0\%)                & 1.0x      &     8 \\
                          & 96 &   7553 & 0 (0\%)      & \textbf{4049} (54\%)   & 4050.0x   &   137 \\
  \midrule\multirow{4}{*}{grover} &  7 &   2479 & 244 (10\%)   & \textbf{304} (12\%)    & 1.24x     &   124 \\
                          &  9 &   8968 & 682 (8\%)    & \textbf{1142} (13\%)   & 1.67x     &   420 \\
                          & 11 &  27148 & 70 (0\%)     & \textbf{3515} (13\%)   & 49.52x    &  1095 \\
                          & 15 & 180497 & 282 (0\%)    & \textbf{22869} (13\%)  & 80.81x    &  6576 \\
  \midrule\multirow{4}{*}{qft}    & 48 &   4626 & 850 (18\%)   & \textbf{1211} (26\%)   & 1.42x     &   268 \\
                          & 64 &   7402 & 1936 (26\%)  & \textbf{2490} (34\%)   & 1.29x     &   372 \\
                          & 80 &  10690 & 0 (0\%)      & \textbf{3874} (36\%)   & 3875.0x   &   163 \\
                          & 96 &  14490 & 5700 (39\%)  & \textbf{6703} (46\%)   & 1.18x     &   787 \\
  \midrule\multirow{1}{*}{shor}   & 10 &   8476 & 457 (5\%)    & \textbf{502} (6\%)     & 1.1x      & 11504 \\
  \midrule\multirow{4}{*}{vqe}    & 12 &  11022 & 4620 (42\%)  & \textbf{7519} (68\%)   & 1.63x     &   173 \\
                          & 16 &  22374 & 0 (0\%)      & \textbf{14513} (65\%)  & 14514.0x  &   245 \\
                          & 20 &  38462 & 0 (0\%)      & \textbf{23775} (62\%)  & 23776.0x  &   415 \\
                          & 24 &  59798 & 0 (0\%)      & \textbf{35315} (59\%)  & 35316.0x  &   608 \\

 \midrule
 \end{tabular}

==> fig/prelim.queso.0.005.tex <==
\begin{tabular}{ccccccc}
  &  &  & \multicolumn{3}{c}{Number of optimizations} &  \\ \cmidrule(lr){4-6}
   Family & Qubits & Input Size & Q & S & S/Q & Time (s) \\


  \midrule\multirow{2}{*}{ham15}  & 17 &   1061 & 206 (19\%)   & \textbf{250} (24\%)    & 1.21x     &    26 \\
                          & 20 &   4365 & 650 (15\%)   & \textbf{1353} (31\%)   & 2.08x     &   130 \\
  \midrule\multirow{3}{*}{hhl}    &  7 &   5319 & 1509 (28\%)  & \textbf{1829} (34\%)   & 1.21x     &   289 \\
                          &  9 &  63392 & 10703 (17\%) & \textbf{20764} (33\%)  & 1.94x     & 12784 \\
                          & 11 & 629247 & 0 (0\%)      & \textbf{109353} (17\%) & 109354.0x & 35987 \\
  \midrule\multirow{2}{*}{gf}     & 48 &   2694 & 0 (0\%)      & 0 (0\%)                & 1.0x      &    19 \\
                          & 96 &   7553 & 0 (0\%)      & \textbf{4098} (54\%)   & 4099.0x   &   213 \\
  \midrule\multirow{4}{*}{grover} &  7 &   2479 & 244 (10\%)   & \textbf{326} (13\%)    & 1.33x     &   152 \\
                          &  9 &   8968 & 32 (0\%)     & \textbf{1043} (12\%)   & 31.64x    &   252 \\
                          & 11 &  27148 & 70 (0\%)     & \textbf{3357} (12\%)   & 47.3x     &  1081 \\
                          & 15 & 180497 & 282 (0\%)    & \textbf{20510} (11\%)  & 72.48x    &  4759 \\
  \midrule\multirow{4}{*}{qft}    & 48 &   4626 & 935 (20\%)   & \textbf{1228} (27\%)   & 1.31x     &   497 \\
                          & 64 &   7402 & 2034 (27\%)  & \textbf{2558} (35\%)   & 1.26x     &   834 \\
                          & 80 &  10690 & 3540 (33\%)  & \textbf{4451} (42\%)   & 1.26x     &  1270 \\
                          & 96 &  14490 & 5862 (40\%)  & \textbf{6808} (47\%)   & 1.16x     &  1597 \\
  \midrule\multirow{4}{*}{vqe}    & 12 &  11022 & 4620 (42\%)  & \textbf{7521} (68\%)   & 1.63x     &   150 \\
                          & 16 &  22374 & 0 (0\%)      & \textbf{14511} (65\%)  & 14512.0x  &   293 \\
                          & 20 &  38462 & 0 (0\%)      & \textbf{23777} (62\%)  & 23778.0x  &   518 \\
                          & 24 &  59798 & 0 (0\%)      & \textbf{35315} (59\%)  & 35316.0x  &   827 \\

 \midrule
 \end{tabular}

==> fig/prelimqueso.0.01.tex <==
\begin{tabular}{rccccccccc}
 &  & \multicolumn{3}{c}{Output Size and Improvement} &  \multicolumn{3}{c}{Optimization Rate (gates/sec)} & &  \\ \cmidrule(lr){3-5} \cmidrule(lr){6-8}
  Benchmark & Input Size & QS & S & QS/S & QS & S & S/QS  & Time (s) & QS Time (s) \\ 

\midrule
 ham15-med       &   1061 & \textbf{855} (-19\%) & 859 (-19\%)             & 1.0x  & 20.6  &  24.67 & 1.2x    &   8 &   10 \\
 ham15-high      &   4365 & 3715 (-15\%)         & \textbf{3373} (-23\%)   & 1.1x  & 12.5  &  44.64 & 3.57x   &  22 &   52 \\
 hhl\_n7         &   5319 & 4323 (-19\%)         & \textbf{3878} (-27\%)   & 1.11x & 76.62 & 134.64 & 1.76x   &  10 &   13 \\
 hhl\_n9         &  63392 & 62896 (-1\%)         & \textbf{47714} (-25\%)  & 1.32x &  3.31 & 119.7  & 36.16x  & 130 &  150 \\
 gf2\^{}16\_mult &   2694 & 2694 (0\%)           & 2694 (0\%)              & 1.0x  &  0    &   0    & 1.0x    &   8 &   38 \\
 gf2\^{}32\_mult &   7553 & 6527 (-14\%)         & \textbf{3429} (-55\%)   & 1.9x  &  5.97 &  29.93 & 5.01x   & 137 &  172 \\
 grover\_n7      &   2479 & 2293 (-8\%)          & \textbf{2227} (-10\%)   & 1.03x & 15.5  &  26.46 & 1.71x   &   9 &   12 \\
 grover\_n9      &   8968 & 8936 (0\%)           & \textbf{8092} (-10\%)   & 1.1x  &  0.8  &  30.77 & 38.46x  &  28 &   40 \\
 grover\_n11     &  27136 & 27078 (0\%)          & \textbf{24493} (-10\%)  & 1.11x &  0.52 &  33.64 & 64.69x  &  78 &  111 \\
 grover\_n15     & 180497 & 180215 (0\%)         & \textbf{162909} (-10\%) & 1.11x &  0.06 &  30.13 & 502.17x & 583 & 4720 \\
 qft\_n48        &   4626 & 3870 (-16\%)         & 3870 (-16\%)            & 1.0x  & 29.08 &  50.28 & 1.73x   &  15 &   26 \\
 qft\_n64        &   7402 & 5510 (-26\%)         & 5510 (-26\%)            & 1.0x  & 55.65 &  59.76 & 1.07x   &  31 &   34 \\
 qft\_n80        &  10690 & 7150 (-33\%)         & 7150 (-33\%)            & 1.0x  & 49.17 &  75.68 & 1.54x   &  46 &   72 \\
 qft\_n96        &  14490 & 8790 (-39\%)         & 8790 (-39\%)            & 1.0x  & 45.6  &  85.43 & 1.87x   &  66 &  125 \\
 qpe\_n8         &   2040 & \textbf{1984} (-3\%) & 2040 (0\%)              & 0.97x &  6.22 &   0    & 0.0x    &   4 &    9 \\
 qpe\_n10        &   8476 & \textbf{8230} (-3\%) & 8476 (0\%)              & 0.97x &  2.56 &   0    & 0.0x    &  17 &   96 \\
 vqe\_n12        &  11022 & 6402 (-42\%)         & \textbf{3615} (-67\%)   & 1.77x & 73.33 & 198.8  & 2.71x   &  37 &   63 \\
 vqe\_n16        &  22374 & 13442 (-40\%)        & \textbf{8031} (-64\%)   & 1.67x & 69.24 & 163.11 & 2.36x   &  87 &  129 \\
 vqe\_n20        &  38462 & 23810 (-38\%)        & \textbf{14911} (-61\%)  & 1.6x  & 86.7  & 141.59 & 1.63x   & 166 &  169 \\
 vqe\_n24        &  59798 & 38018 (-36\%)        & \textbf{24767} (-59\%)  & 1.54x & 56.57 & 110.56 & 1.95x   & 316 &  385 \\
\midrule
\textbf{geomean} & & & & 1.18 & &  & 5.15 & & 
\end{tabular}

==> fig/prelimqueso.0.1.tex <==
\begin{tabular}{rccccccccc}
 &  & \multicolumn{3}{c}{Output Size and Improvement} &  \multicolumn{3}{c}{Optimization Rate (gates/sec)} & &  \\ \cmidrule(lr){3-5} \cmidrule(lr){6-8}
  Benchmark & Input Size & QS & S & QS/S & QS & S & S/QS  & Time (s) & QS Time (s) \\ 

\midrule
 ham15-med       &   1061 & \textbf{821} (-23\%)  & 859 (-19\%)             & 0.96x & 2.42 &  2.08 & 0.86x  &    97 &    99 \\
 ham15-high      &   4365 & 3373 (-23\%)          & \textbf{3363} (-23\%)   & 1.0x  & 2.57 &  2.61 & 1.02x  &   383 &   386 \\
 hhl\_n7         &   5319 & 3793 (-28\%)          & \textbf{3581} (-33\%)   & 1.06x & 1.22 &  1.4  & 1.15x  &  1242 &  1253 \\
 hhl\_n9         &  63392 & 52689 (-17\%)         & \textbf{45442} (-28\%)  & 1.16x & 0.99 &  1.66 & 1.68x  & 10803 & 10824 \\
 gf2\^{}16\_mult &   2694 & 2694 (0\%)            & \textbf{2691} (0\%)     & 1.0x  & 0    &  0.01 & 1.0x   &   284 &   291 \\
 gf2\^{}32\_mult &   7553 & 7553 (0\%)            & \textbf{3429} (-55\%)   & 2.2x  & 0    & 10.84 & 1.0x   &   380 &   387 \\
 grover\_n7      &   2479 & 2234 (-10\%)          & \textbf{2227} (-10\%)   & 1.0x  & 1.06 &  1.1  & 1.04x  &   229 &   232 \\
 grover\_n9      &   8968 & 8254 (-8\%)           & \textbf{8091} (-10\%)   & 1.02x & 0.85 &  1.04 & 1.22x  &   839 &   843 \\
 grover\_n11     &  27136 & 27078 (0\%)           & \textbf{24464} (-10\%)  & 1.11x & 0.02 &  0.99 & 49.5x  &  2712 &  2727 \\
 grover\_n15     & 180497 & 180215 (0\%)          & \textbf{162909} (-10\%) & 1.11x & 0.01 &  1.63 & 163.0x & 10800 & 21921 \\
 qft\_n48        &   4626 & \textbf{3333} (-28\%) & 3524 (-24\%)            & 0.95x & 0.58 &  0.5  & 0.86x  &  2217 &  2228 \\
 qft\_n64        &   7402 & \textbf{4811} (-35\%) & 5036 (-32\%)            & 0.96x & 0.78 &  0.71 & 0.91x  &  3329 &  3341 \\
 qft\_n80        &  10690 & \textbf{6314} (-41\%) & 6546 (-39\%)            & 0.96x & 1.02 &  0.97 & 0.95x  &  4272 &  4282 \\
 qft\_n96        &  14490 & \textbf{7947} (-45\%) & 8042 (-44\%)            & 0.99x & 1.24 &  1.23 & 0.99x  &  5236 &  5278 \\
 qpe\_n8         &   2040 & \textbf{1956} (-4\%)  & 2035 (0\%)              & 0.96x & 0.08 &  0.02 & 0.25x  &   241 &  1058 \\
 qpe\_n10        &   8476 & \textbf{8155} (-4\%)  & 8474 (0\%)              & 0.96x & 0.36 &  0    & 0.0x   &   879 &   886 \\
 vqe\_n12        &  11022 & 5982 (-46\%)          & \textbf{3572} (-68\%)   & 1.67x & 8.08 & 12.02 & 1.49x  &   619 &   624 \\
 vqe\_n16        &  22374 & 13442 (-40\%)         & \textbf{7949} (-64\%)   & 1.69x & 6.75 & 11.23 & 1.66x  &  1284 &  1323 \\
 vqe\_n20        &  38462 & 23810 (-38\%)         & \textbf{14858} (-61\%)  & 1.6x  & 7.04 & 11.79 & 1.67x  &  2002 &  2080 \\
 vqe\_n24        &  59798 & 59798 (0\%)           & \textbf{24668} (-59\%)  & 2.42x & 0    & 10.72 & 1.0x   &  3277 &  3419 \\
\midrule
\textbf{geomean} & & & & 1.18 & &  & 2.92 & & 
\end{tabular}

==> fig/queso.tex <==
\begin{tabular}{rcccccccc}
 &   \multicolumn{4}{c}{Circuit Size} &  \multicolumn{3}{c}{Optimization Rate (gates/sec)} &  \\ \cmidrule(lr){2-5} \cmidrule(lr){6-8}
  Name & Original & QS & C & C/QS & QS & C & C/QS  & Time (s) \\ 

\midrule
 grover\_n7 &  2479 & 2172 & \textbf{2130} & 0.98 & 0.45 & 0.51 & 1.14x &  678.2 \\
 grover\_n9 &  8968 & 8109 & \textbf{7769} & 0.96 & 0.35 & 0.49 & 1.4x  & 2464   \\
 hhl\_n7    &  5319 & 3796 & \textbf{3355} & 0.88 & 1.38 & 1.78 & 1.29x & 1102   \\
 qft\_n48   &  4626 & 3539 & \textbf{3476} & 0.98 & 1.24 & 1.31 & 1.06x &  875   \\
 qft\_n64   &  7402 & 5144 & \textbf{4914} & 0.96 & 1.67 & 1.84 & 1.1x  & 1349   \\
 vqe\_n8    &  3894 & 1138 & \textbf{1069} & 0.94 & 8.89 & 9.11 & 1.03x &  310   \\
 vqe\_n12   & 11022 & 4374 & \textbf{3395} & 0.78 & 6.36 & 7.29 & 1.15x & 1046   \\
\midrule
\textbf{geomean} & & & & 0.92 & &  & 1.16 & 
\end{tabular}

==> fig/tab-main-ablation.tex <==
\begin{figure}[!ht]
  \small
\begin{tabular}{cccccc}
                          &        &            & \multicolumn{3}{c}{Optimizer}         \\\cmidrule(lr){4-6}
Benchmark                 & Qubits & Input Size & VOQC  & \algname{} & \algnameminus{} \\
 \midrule\multirow{4}{*}{boolsat}  & 28 &   75670 & -83.2\% & \textbf{-83.7\%} & -83.0\% \\
                           & 30 &  138293 & -83.3\% & \textbf{-83.7\%} & -83.1\% \\
                           & 32 &  262548 & -83.3\% & \textbf{-83.5\%} & -83.1\% \\
                           & 34 &  509907 & -83.3\% & \textbf{-83.4\%} & -83.1\% \\
 \midrule\multirow{4}{*}{bwt}      & 17 &  262514 & -30.0\% & \textbf{-31.1\%} & -28.3\% \\
                           & 21 &  402022 & -38.4\% & \textbf{-40.0\%} & -36.3\% \\
                           & 25 &  687356 & N.A.    & \textbf{-43.8\%} & -40.0\% \\
                           & 29 &  941438 & N.A.    & \textbf{-44.5\%} & -41.0\% \\
 \midrule\multirow{4}{*}{grover}   &  9 &    8968 & \textbf{-29.4\%} & \textbf{-29.4\%} & -26.1\% \\
                           & 11 &   27136 & -29.9\% & \textbf{-30.0\%} & -26.3\% \\
                           & 13 &   72646 & \textbf{-29.7\%} & \textbf{-29.7\%} & -26.0\% \\
                           & 15 &  180497 & \textbf{-29.5\%} & \textbf{-29.5\%} & -26.0\% \\
 \midrule\multirow{4}{*}{hhl}      &  7 &    5319 & \textbf{-55.4\%} & -55.3\% & -54.4\% \\
                           &  9 &   63392 & -56.3\% & \textbf{-56.5\%} & -55.6\% \\
                           & 11 &  629247 & \textbf{-53.7\%} & \textbf{-53.7\%} & -53.1\% \\
                           & 13 & 5522186 & N.A.    & \textbf{-52.6\%} & -52.1\% \\
 \midrule\multirow{4}{*}{shor}     &  10 &    8476 & \textbf{-11.1\%} & -11.0\% & -10.3\% \\
                           &  12 &   34084 & \textbf{-11.2\%} & \textbf{-11.2\%} & -10.7\% \\
                           &  14 &  136320 & \textbf{-11.3\%} & -11.2\% & -10.8\% \\
                           &  16 &  545008 & \textbf{-11.3\%} & \textbf{-11.3\%} & -10.9\% \\
 \midrule\multirow{4}{*}{sqrt}     & 42 &   79574 & \textbf{-33.0\%} & \textbf{-33.0\%} & -31.5\% \\
                           & 48 &  186101 & \textbf{-32.7\%} & -32.6\% & -31.2\% \\
                           & 54 &  424994 & \textbf{-32.4\%} & -32.3\% & -30.9\% \\
                           & 60 &  895253 & N.A.    & \textbf{-34.3\%} & -32.9\% \\
 \midrule\multirow{4}{*}{statevec} &  5 &   31000 & -78.8\% & \textbf{-78.9\%} & -78.1\% \\
                           &  6 &  129827 & \textbf{-78.4\%} & \textbf{-78.4\%} & -77.9\% \\
                           &  7 &  526541 & \textbf{-78.1\%} & \textbf{-78.1\%} & -77.8\% \\
                           &  8 & 2175747 & N.A.    & \textbf{-78.7\%} & -78.6\% \\
 \midrule\multirow{4}{*}{vqe}      & 12 &   11022 & -63.0\% & \textbf{-69.5\%} & -62.7\% \\
                           & 16 &   22374 & -60.1\% & \textbf{-66.3\%} & -59.7\% \\
                           & 20 &   38462 & -57.4\% & \textbf{-63.4\%} & -57.2\% \\
                           & 24 &   59798 & -54.9\% & \textbf{-60.6\%} & -54.8\% \\
\midrule
avg                       &        &           & -48.1\% & \textbf{-49.4\%} & -47.3\% \\
\end{tabular}
\caption{Ablation study of \lstinline{meld}. The table shows
  percentage reduction in gate count achieved by the version of
  \algname{}, called \algnameminus{} that uses simply concatenation
  instead of the \lstinline{meld} algorithm compared with \voqc{} and
  the original \algname{}.
%
The measurements show
that with the \lstinline{meld} algorithm, our \algname{} optimizer reduces gate counts better than using \voqc{} alone
or simply splitting the circuit into segments and optimize them using \voqc{} separately.
}    \label{fig:main-ablation}
\end{figure}


==> fig/tab-main-result-clifft.tex <==
\begin{table}[]
\small
\begin{tabular}{cccccccc}
                        &        &               & \multicolumn{2}{c}{Relative T Gate Reduction} & \multicolumn{3}{c}{Time(s)}    \\ \cmidrule(lr){4-5} \cmidrule(lr){6-8}  
Benchmarks              & Qubits & Input T Count & Feynman               & OAC                   & Feynman  & OAC     & Speedup   \\\midrule{}
\multirow{4}{*}{hwb}    & 8      & 5887          & -25.7\%               & -25.7\%               & 4.10     & 3.30    & 24.1\%    \\
                        & 10     & 29939         & -29.8\%               & -29.8\%               & 250.77   & 26.98   & 829.4\%   \\
                        & 11     & 84196         & -31.3\%               & -31.3\%               & 4767.30  & 87.81   & 5329.0\%  \\
                        & 12     & 171465        & -34.1\%               & -34.1\%               & 21880.36 & 262.93  & 8221.7\%  \\\midrule{}
\multirow{3}{*}{gf}     & 32     & 7168          & -28.6\%               & -28.6\%               & 3.96     & 3.89    & 1.8\%     \\
                        & 64     & 28672         & -28.6\%               & -28.3\%               & 71.24    & 66.51   & 7.1\%     \\
                        & 128    & 114688        & -28.6\%               & -28.4\%               & 5156.62  & 2812.72 & 83.3\%    \\\midrule{}
\multirow{2}{*}{grover} & 11     & 12005         & -32.1\%               & -32.1\%               & 0.42     & 1.08    & -61.1\%   \\
                        & 15     & 80514         & -32.1\%               & -32.1\%               & 5.85     & 10.09   & -42.0\%   \\\midrule{}
\multirow{2}{*}{hhl}    & 7      & 61246         & -31.2\%               & -31.2\%               & 409.78   & 17.81   & 2200.3\%  \\
                        & 9      & 565183        &                       & -34.1\%               & -        & 382.86  &           \\\midrule{}
\multirow{4}{*}{qft}    & 48     & 44803         & -20.2\%               & -20.2\%               & 195.10   & 45.77   & 326.2\%   \\
                        & 64     & 61027         & -20.3\%               & -20.3\%               & 531.45   & 80.73   & 558.3\%   \\
                        & 80     & 77251         & -20.3\%               & -20.3\%               & 1083.36  & 128.53  & 742.9\%   \\
                        & 96     & 93475         & -20.3\%               & -20.3\%               & 1931.88  & 197.97  & 875.9\%   \\\midrule{}
\multirow{4}{*}{shor}   & 12     & 20180         & -20.3\%               & -20.3\%               & 21.00    & 10.11   & 107.6\%   \\
                        & 14     & 70544         & -20.5\%               & -20.5\%               & 999.47   & 55.14   & 1712.6\%  \\
                        & 16     & 266060        & -20.6\%               & -20.6\%               & 28382.32 & 249.17  & 11290.9\% \\
                        & 18     & 1042184       &                       & -20.6\%               & -        & 2088.35 &           \\\midrule{}
avg                     &        &               & -26.1\%               & -26.2\%               &          &         & 1894.6\% 
\end{tabular}
    \caption{Comparison of running time and gate counts for Clifford+T gateset.}
    \label{tab:main-clifft}
\end{table}

==> fig/tab-main-result-time.tex <==
\begin{figure}[!ht]
    \centering
\begin{tabular}{cccccccc}
                          &        &            & \multicolumn{4}{c}{Time (s)}                       &                                                           \\\cmidrule(lr){4-7}
Benchmark                 & Qubits & Input Size & Quartz & Queso         & VOQC    & algname          & \begin{tabular}[c]{@{}c@{}}algname\\ speedup\end{tabular} \\\midrule{}
\multirow{4}{*}{boolsat}  & 28     & 75670      & 12h    & 12h           & 68.6    & \textbf{60.4}    & 1.14                                                      \\
                          & 30     & 138293     & 12h    & 12h           & 307.3   & \textbf{99.8}    & 3.08                                                      \\
                          & 32     & 262548     & 12h    & 12h           & 1266.2  & \textbf{292.8}   & 4.32                                                      \\
                          & 34     & 509907     & 12h    & 12h           & 6151.0  & \textbf{600.4}   & 10.24                                                     \\\midrule{}
\multirow{4}{*}{bwt}      & 17     & 262514     & 12h    & 12h           & 8303.1  & \textbf{1196.8}  & 6.94                                                      \\
                          & 21     & 402022     & 12h    & 12h           & 23236.8 & \textbf{2281.0}  & 10.19                                                     \\
                          & 25     & 687356     & 12h    & 12h           & 43200.0 & \textbf{5698.9}  & 7.58                                                      \\
                          & 29     & 941438     & 12h    & 12h           & 43200.0 & \textbf{11842.2} & 3.65                                                      \\\midrule{}
\multirow{4}{*}{grover}   & 9      & 8968       & 12h    & 12h           & 9.3     & \textbf{6.9}     & 1.35                                                      \\
                          & 11     & 27136      & 12h    & 12h           & 106.5   & \textbf{29.6}    & 3.59                                                      \\
                          & 13     & 72646      & 12h    & 12h           & 815.7   & \textbf{99.1}    & 8.23                                                      \\
                          & 15     & 180497     & 12h    & 12h           & 5743.2  & \textbf{320.3}   & 17.93                                                     \\\midrule{}
\multirow{4}{*}{hhl}      & 7      & 5319       & 12h    & 12h           & \textbf{0.3}     & 1.2     & 0.21                                                      \\
                          & 9      & 63392      & 12h    & 12h           & 74.1    & \textbf{31.6}    & 2.35                                                      \\
                          & 11     & 629247     & 12h    & 12h           & 14868.8 & \textbf{636.5}   & 23.36                                                     \\
                          & 13     & 5522186    & 12h    & Parsing Error & 43200.0 & \textbf{13165.3} & 3.28                                                      \\\midrule{}
\multirow{4}{*}{shor}     & 10     & 8476       & 12h    & OOM           & 8.8     & \textbf{5.3}     & 1.65                                                      \\
                          & 12     & 34084      & 12h    & 12h           & 179.9   & \textbf{38.5}    & 4.67                                                      \\
                          & 14     & 136320     & 12h    & 12h           & 3638.4  & \textbf{190.0}   & 19.15                                                     \\
                          & 16     & 545008     & 12h    & 12h           & 70475.2 & \textbf{943.0}   & 74.73                                                     \\\midrule{}
\multirow{4}{*}{sqrt}     & 42     & 79574      & 12h    & 12h           & \textbf{30.0}    & 123.8   & 0.24                                                      \\
                          & 48     & 186101     & 12h    & 12h           & \textbf{191.2}   & 341.3   & 0.56                                                      \\
                          & 54     & 424994     & 12h    & 12h           & 3946.5  & \textbf{852.6}   & 4.63                                                      \\
                          & 60     & 895253     & 12h    & 12h           & 43200.0 & \textbf{2108.0}  & 20.49                                                     \\\midrule{}
\multirow{4}{*}{statevec} & 5      & 31000      & 12h    & OOM           & \textbf{1.6}     & 5.0     & 0.33                                                      \\
                          & 6      & 129827     & 12h    & 12h           & 45.9    & \textbf{35.1}    & 1.31                                                      \\
                          & 7      & 526541     & 12h    & 12h           & 1812.2  & \textbf{202.4}   & 8.95                                                      \\
                          & 8      & 2175747    & 12h    & 12h           & 43200.0 & \textbf{2108.8}  & 20.49                                                     \\\midrule{}
\multirow{4}{*}{vqe}      & 12     & 11022      & 12h    & 12h           & \textbf{0.2}     & 1.5     & 0.10                                                      \\
                          & 16     & 22374      & 12h    & 12h           & \textbf{0.6 }    & 4.3     & 0.15                                                      \\
                          & 20     & 38462      & 12h    & 12h           & \textbf{2.0}     &8.9     & 0.23                                                      \\
                          & 24     & 59798      & 12h    & 12h           & \textbf{5.4}     & 17.3    & 0.32                                                      \\\midrule{}
avg                       &        &            &        &               &         &                  & 8.30
\end{tabular}

\caption{The figure shows the running time in seconds of the four optimizers, using gate count as the cost metric.
%
The column "\algname{} Speedup" is the speed of our  \algname{} with respect to \voqc{}, calculated as \voqc{} time divided by \algname{} time.
%
These measurements show that our optimizer \algname{} can be significantly faster, especially for large circuits ($8.3$x faster on average).
As \figref{main-gate-count} shows, these time improvements come without any loss in optimization quality.
%
These results suggest that local optimality approach to optimization of quantum circuits can be effective in practice.}
    %
    \label{fig:main-time}
\end{figure}

==> fig/tab-main-result.tex <==
\begin{figure}[!ht]
  \small
\begin{tabular}{ccccccc}
                          &        &            & \multicolumn{4}{c}{Optimizer}         \\\cmidrule(lr){4-7}
Benchmark                 & Qubits & Input Size & Quartz  & Queso   & VOQC    & \algname{} \\\midrule{}
\multirow{4}{*}{boolsat}  & 28     & 75670      & -41.1\% & -30.4\% & -83.2\% & \textbf{-83.7\%} \\
                          & 30     & 138293     & -23.5\% & -30.2\% & -83.3\% & \textbf{-83.7\%} \\
                          & 32     & 262548     & -6.9\%  & 0.0\%   & -83.3\% & \textbf{-83.5\%} \\
                          & 34     & 509907     & -2.9\%  & 0.0\%   & -83.3\% & \textbf{-83.4\%} \\\midrule{}
\multirow{4}{*}{bwt}      & 17     & 262514     & -8.7\%  & -0.1\%  & -30.0\% & \textbf{-31.2\%} \\
                          & 21     & 402022     & -3.1\%  & -0.1\%  & -38.4\% & \textbf{-40.0\%} \\
                          & 25     & 687356     & -0.8\%  & 0.0\%   & N.A.    & \textbf{-43.8\%} \\
                          & 29     & 941438     & -0.4\%  & 0.0\%   & N.A.    & \textbf{-44.5\%} \\\midrule{}
\multirow{4}{*}{grover}   & 9      & 8968       & -9.4\%  & -13.7\% & \textbf{-29.4\%} & \textbf{-29.4\%} \\
                          & 11     & 27136      & -9.5\%  & -9.6\%  & -29.9\% & \textbf{-30.0\%} \\
                          & 13     & 72646      & -9.6\%  & -0.3\%  & \textbf{-29.7\%} & \textbf{-29.7\%} \\
                          & 15     & 180497     & -9.6\%  & -0.2\%  & \textbf{-29.5\%} & \textbf{-29.5\%} \\\midrule{}
\multirow{4}{*}{hhl}      & 7      & 5319       & -26.6\% & -28.7\% & \textbf{-55.4\%} & -55.3\% \\
                          & 9      & 63392      & -24.4\% & -23.8\% & -56.3\% & \textbf{-56.5\%} \\
                          & 11     & 629247     & -1.1\%  & 0.0\%   & \textbf{-53.7\%} &\textbf{ -53.7\%} \\
                          & 13     & 5522186    & 0.0\%   & N.A.    & N.A.    & \textbf{-52.6\%} \\\midrule{}
\multirow{4}{*}{shor}     & 10     & 8476       & 0.0\%   & -5.4\%  & \textbf{-11.1\%} & -11.0\% \\
                          & 12     & 34084      & 0.0\%   & -3.8\%  & \textbf{-11.2\%} & \textbf{-11.2\%} \\
                          & 14     & 136320     & 0.0\%   & 0.0\%   & \textbf{-11.3\%} & -11.2\% \\
                          & 16     & 545008     & 0.0\%   & 0.0\%   & \textbf{-11.3\%} &\textbf{ -11.3\%} \\\midrule{}
\multirow{4}{*}{sqrt}     & 42     & 79574      & -16.2\% & -0.1\%  & \textbf{-33.0\%} &\textbf{ -33.0\%} \\
                          & 48     & 186101     & -15.2\% & 0.0\%   & \textbf{-32.7\%} & -32.6\% \\
                          & 54     & 424994     & -5.1\%  & 0.0\%   & \textbf{-32.4\%} & -32.3\% \\
                          & 60     & 895253     & -2.1\%  & 0.0\%   & N.A.    & \textbf{-34.3\%} \\\midrule{}
\multirow{4}{*}{statevec} & 5      & 31000      & -48.4\% & -74.5\% & -78.8\% & \textbf{-78.9\%} \\
                          & 6      & 129827     & -35.0\% & -29.7\% & \textbf{-78.4\%} & \textbf{-78.4\%} \\
                          & 7      & 526541     & -2.0\%  & -29.7\% & \textbf{-78.1\%} & \textbf{-78.1\%} \\
                          & 8      & 2175747    & -0.1\%  & 0.0\%   & N.A.    & \textbf{-78.7\%} \\\midrule{}
\multirow{4}{*}{vqe}      & 12     & 11022      & -35.4\% & -69.1\% & -63.0\% & \textbf{-69.5\%} \\
                          & 16     & 22374      & -33.7\% & -64.2\% & -60.1\% &\textbf{ -66.3\%} \\
                          & 20     & 38462      & -32.2\% & -60.8\% & -57.4\% & \textbf{-63.4\%} \\
                          & 24     & 59798      & -30.8\% & -36.4\% & -54.9\% & \textbf{-60.6\%} \\\midrule{}
avg                       &        &            & -13.6\% & -16.5\% & -48.1\% & \textbf{-49.4\%}
\end{tabular}
\caption{The figure shows percentage reduction in gate count achieved by the four optimizers.
%
The measurements show
that our \algname{} optimizer reduces gate counts better than all other optimizers.
%
Specifically, our \algname{} optimizer delivers a slight improvement on \voqc{}, which is the best among all the other optimizers.
%
Given that our \algname{} optimizer is faster than all other optimizers (\figref{main-time}), these experiments show that local optimality approach can improve performance without any loss in optimization quality.
%
These results suggest that local optimality approach to optimization of quantum circuits can be effective in practice.
}    \label{fig:app-main-gate-count}
\end{figure}

==> implementation.tex <==


\myparagraph{\quartz{} and \queso{}.}
\quartz{} and \queso{} are state of the art tools for synthesizing
circuit equivalence rules and using them to optimize circuits ~\cite{queso-2023, quartz-2022}.
%
The tools differ in their approach to rule synthesis,
but their algorithms for applying the rules for circuit optimization are similar.
%
To optimize circuits,
they execute a search algorithm by maintaining a search queue of candidate circuits.
%
At each step,
they pop a circuit from the queue and rewrite parts of the circuit using
their respective equivalence rules.
%
Then, they insert the new circuits back to the queue and repeat the process
until the queue becomes empty.
%
Since the number of circuits to consider grows exponentially with the size of the circuit,
both tools use ``beam search'',
 a search algorithm that limits the size of the search
queue and appropriately drops circuits after the limit is reached.
%
By limiting the size of the search queue,
\quartz{} and \queso{} ensure that
the space usage is linear in the size of circuit
(they only store a fixed number of circuits).
%
Their running time is exponential
and they provide a timeout functionality,
allowing their users to halt optimization after a certain amount of time.
%
Using this graph search approach with timeouts,
the tools have delivered excellent reductions in gate count
across a range of benchmarks and different gate sets~\cite{queso-2023, quartz-2022}.
%

\myparagraph{\feyntool{}.}
\feyntool{} is an optimizer from the ``Feynman''\footnote{https://github.com/meamy/feynman} toolkit
for quantum circuits that uses the path integral model of quantum computation to analyze and optimize circuits~\cite{amy2019formal}.
%
This path integral model encodes the state transition performed by a quantum circuit with a
sum over all possible paths between two given states.
%
The model is used by the \feyntool{} optimizer to generate a \emph{phase polynomial}
of a circuit on which the optimizer performs a \emph{phase folding} optimization.
The optimization merges phase gates
acting on the same set of computational paths.
%
Phase folding is a powerful technique for optimizing phase gates such as the $\mathsf{S}$ gate,
the $\mathsf{Z}$ gate, and the most expensive $\mathsf{T}$ gate~\cite{t-depth}.
%
Furthermore, the algorithm terminates in polynomial time,
making it a practical choice for optimizing large circuits.


% However, both optimizers deliver poor time scalability,
% because the number of the circuits that need to be considered
% increases exponentially with the size
% of the circuits and so does the running time.
% %
% For instance,
% \quartz{} takes more than $24$ hours on a circuit of size $48$.
% %
% \queso{} takes eighteen seconds to terminate on this circuit,
% and its running time jumps to an hour on a circuit of size 96 (a $20$x increase),
% which further jumps to around six hours for a circuit of size 326 (a $6$x increase).
% %
% For this reason,
% both tools implement a timeout facility,
% allowing the users to stop optimization at will.
% %
% Using this graph search approach with timeouts,
% the tools have delivered excellent reductions in gate count
% across a range of benchmarks and different gate sets.
%

% Because of the exponential time complexity,
% we run both tools with a timeout and
% take the best circuit it finds within the given time.


\myparagraph{\voqc{}.}
VOQC~\cite{hietala2021verified} is
a formally verified optimizer for quantum circuits,
implemented using Coq.

It takes as input quantum programs written in SQIR,
a quantum intermediate representation also developed by the authors.
VOQC implements several optimization passes inspired by state-of-the-art unverified optimizers~\cite{Nam_2018},
including not propagation, Hadamard gate reduction,
single- and two-qubit gate cancellation, and rotation merging. 
The optimizations are proved correct with respect to SQIR's denotational semantics.


% \myparagraph{Using optimizers with \coam{}.}
% We implement the \coam{} algorithm in SML and allow using existing optimizers as oracles.
% %
% Because the language allows for cross-language calls to C++,
% we only require a C++ wrapper to use an optimizer.
% %
% The wrapper implements the function $\mathsf{optimize}$,
% which takes a circuit in QASM format as input
% and returns an optimized circuit in as output.
% %

% %
% Because \quartz{} is written in C++,
% it was straightforward to use it in our implementation.
% %
% As an optimization,
% we pre-load the circuit equivalence rules of the \quartz{} optimizer
% and use them across different calls to it.
% %
% This removes the overhead of repeated file I/O.
% %

% The optimizer \queso{} is written in Java and we implement
% a C++ wrapper that manages the Java runtime and interfaces with our \coam{} implementation.
% %
% Our \coam{} implementation makes cross-language function calls the C++ wrapper,
% which, in turn, calls into the Java runtime,
% which executes \queso{} on the circuit.
% %
% The other implementation details are similar to \quartz{}.

% The \feyntool{} optimizer is written in Haskell
% and we write a C++ wrapper that invokes it via the operating system.
% %
% Specifically, to invoke \feyntool{} on a subcircuit, the wrapper
% writes the QASM representation to a file,
% calls \feyntool{} by using a system call,
% and reads the output.
%
%
% With more engineering efforts,
% it is possible to make the integration more efficient by
% by writing a C wrapper around Haskell and directly calling it from our implementation.
% %
% We leave this to future work.
%




% and does not naturally work with our implementation,
% because our
% implementation language does not cross-operate with Haskell.
% %
% We integrate \feyntool{} via the operating system.
%
%

% Because the overhead is large and difficult amortize by increasing
% subcircuit sizes, our integration with \feyntool{} incurs significant
% overhead.
% %
% Nevertheless, this integration demonstrates the feasibility of
% integrating with existing optimizers either through cross-language
% interoperability features (when feasible) or through systems calls.
%


% \myparagraph{Granularity optimization.}


==> intro-old.tex <==
\ur{BIG TODO: introduced two notions of optimality, absolute and relative.  propogate.}

\ur{Intro + Abst: base --> oracle}
\ur{Feynman: what it its complexity, at least quad it seems?  What guarantee does it have?  Heuristic?  }
\ur{Meta: would be worth re-org'in section.  Make Omega optimality its own section and then describe SOAM.}
\ur{IMPORTANT: one sticking point for me was what kind of properties can SOAM optimize (in this paper).  We optimize gate count and T-count.  These are different enough, the question arises.  Can we formulate in terms of some algebra?  Associative property of splits or something? }
\ur{Meta: in the previous submission, we focused on ``scaling'' existing optimizers.  We now have changed our motivation to be more broader (local opt).  But the paper still has some sections using the prev motivation (like intro to soam section).}
\ur{Implementation: do not talk about ``integrating'' an existing optimizer but using it as an oracle for SOAM.  Ideally, we do not want to ``integrate'' and want this to be simple. }
Quantum computing shows significant potential in compute-intensive
domains that remain challenging for classical computers, including,
for example, the simulation of chemical and physical
processes~\cite{y+variational-quantum-2019}, combinatorial
optimization~\cite{hk-inspired-2002}, and machine
learning~\cite{b+quantum-learning-2017}.
%
This promise, coupled with advances in understanding and exploiting
the physics of subatomic particles, has advanced the field of quantum computing
rapidly over the past decade.
%
On the algorithms front, important quantum algorithms, which are
typically expressed as quantum circuits consisting of logical gates,
have been developed for key problems~\cite{deutsch1992rapid,shor1994algorithms,grover1996fast,bernstein1997quantum}.
%
On the architectures front, a variety of technologies have been
proposed for developing quantum computers, some capable of running
circuits with hundreds of qubits or depth-100 gate operations,
have become operational~\cite{k+evidence-2023, moses2023race, wurtz2023aquila}.
%
For example, IBM's Osprey quantum processor has 433 superconducting
qubits, and Atom computing has recently announced a quantum
computer with 1,180 neutral-atom qubits.

% Because modern quantum hardware supports a limited number of gates or operations,
Running a quantum algorithm on modern quantum hardware requires
``compiling'' the logical circuit representation of the algorithm to
the gate set for the target hardware~\cite{chong2017programming, tket-2020}.
%
A key step in this compilation process is the optimization of the
logical quantum circuit to reduce, for example, the number of all and
possibly certain kinds of gates such as T-gates, which are expensive.
%
Optimizing quantum circuits, however, is a formidable challenge.
%
It is known that finding the optimal circuit that is equivalent to a
given circuits is QMA hard~\cite{janzing2003identity} and thus it is
unlikely (unless the polynomial hierarchy collapses) that we will be
able to achieve fully optimal circuits efficiently.
%

%% Many state-of-the art circuit optimization tools optimize the circuit
%% by incrementally applying a basis set of (optimizing) transformations
%% to the circuit~\cite{n+large-2018,qiskit-2019,tket-2020,quartz-2022,queso-2023}.
%% %
%% Because this approach can take a  optimizations

%% Given enough time, such algorithms could find a globally optimal
%% circuit.
%% %
%% But in reality, they can take a long time (hours or days) even for
%% circuits with a few hundred gates.
%% %

%
%% These optimizers therefore are typically used under a time-out
%% (usually of hours) that terminates the optimization process when the
%% time-out occurs.
%
%% Earlier quantum optimizers relied on human beings to manually
%% construct this basis set of optimizing
%% transformations~\cite{n+large-2018}.
%% %
%% More recent research showed that it is possible to automate this process,
%% by developing algorithms that construct this basis set~\cite{quartz-2022, queso-2023} and
%% then using the basis set to optimize the circuit.
%% %
%% To optimize,
%% these approaches search for matching subcircuits in the basis set and replace them
%% with their optimized counterparts.
%%
%% These advances have led to important improvements in optimization quality
%% but they all have a key limitation: they do not scale beyond small
%% circuits, typically consisting of hundreds of gates.
%% %
Given that today's NISQ-era quantum computers have hundreds of qubits
and given the advances in improving coherence
times~\cite{preskill2018quantum}, it is currently feasible to execute
large quantum circuit with thousands of gates~\cite{k+evidence-2023}.
%
It is expected that further engineering improvements will lead to
successful execution of even larger circuits, even before the
fault-tolerant era.
%
These advances and the proven QMA-hardness of the quantum optimization
problem thus raise an important question: how can we improve the
efficiency, effectiveness, and scale of quantum circuit optimization?

In this paper, we propose two notions of local optimality
and develop efficient and effective optimization techniques that
produce locally optimal quantum circuits.
%
%
Given an integer $\Omega$, our first notion of local optimality,
called $\Omega$-optimality, requires each $\Omega$-deep subcircuit of
a circuit to be fully optimal.
%
Our second notion of local optimality, called relative local
optimality, relaxes local optimality by requiring the subcircuits to be
optimal only \defn{relative} to a given optimizer---i.e.,
the subcircuits may not be further optimized by the given optimizer
(though they may not be fully optimal).
%
Relative local optimality is a more practical notion
because achieving full optimality even for small subcircuits can be expensive.
%
Furthermore, the notion allows us to use our optimization techniques for existing optimizers
that do not guarantee full optimality.

To ensure local optimality, we present an algorithm that uses a given
``small circuit'' optimizer, which we call the ``oracle'' (optimizer),
to optimize small circuits.
%
For large input circuits, the algorithm partitions the circuit into
smaller subcircuits and recursively optimizes each subcircuit,
%
using the oracle only for the small circuits.
%
The algorithm then ``melds'' the optimized subcircuits to construct an
optimized circuit.
%
Since each subcircuit is optimized in isolation, the meld operation
cannot simply join the optimized results, because doing so would offer
no optimality guarantee: the seam conjoining two optimized subcircuits
may give rise to further optimizations that simple joining would miss.
%
Our algorithm therefore melds the optimized subcircuits together by
propagating optimizations from one subcircuit into the other until it achieves
convergence over the whole circuit.
%
Crucially, it only uses the oracle optimizer on small, $\Omega$-deep
subcircuits.
%


Under some reasonable assumptions for the cost function being
optimized---that the cost functions are non-negative and are integer
valued, and that they are additive under circuit concatenation
operation---we show that our \coam{} algorithm ensures local
optimality or relative local optimality (depending on the oracle
optimizer being used).
%
Furthermore, we prove that even though the
algorithm melds circuits at many levels of the recursive partitions,
and each meld operation may require many oracle calls to join circuits optimally,
the \coam{} algorithm makes linear number of calls (in the
size of the circuit) to the oracle optimizer.

\ur{The bound is  a  bit sloppy here. Improve }

We show that our algorithm is practical by implementing it and
applying it to three different state of the art optimizers:
%
Feynman~\cite{amy2019formal},
%
Quartz~\cite{quartz-2022}, and
%
Queso~\cite{queso-2023}.
%
We evaluate the resulting optimizers by considering a variety of
quantum circuits, ranging from moderate to large circuits.
%
The experiments confirm that our optimizers runs efficiently in
practice and can optimize circuits with many thousands gates
reasonably quickly.


The contributions of the paper are the following:
\begin{itemize}

\item A local optimality criterion, called $\Omega$-optimality for quantum circuit optimization.

\item An efficient algorithm for quantum circuit optimization that ensures local optimality.

\item The proofs that the algorithm guarantees local optimality and is efficient.

\item A practical implementation of the algorithm.

\item Applications of \coam{} algorithm to three existing optimizers.

\item An empirical evaluation that confirms the theoretical runtime and the quality guarantees and shows the scalability benefits of local optimality.

\end{itemize}


%% Guaranteed linear worst-case optimization time by itself is not
%% interesting for quantum circuit optimization---after all, a simple
%% algorithm that simply applies up to a linear number of optimizations
%% achieves the same bound.
%% %
%% What is also important is to ensure some degree of quality for the
%% optimized circuit.
%% %
%% For our algorithm, we show that the optimized circuits (output)
%% are \defn{locally optimal} with respect to the oracle being used in
%% the sense that applying the oracle to any (contiguous) subcircuit of
%% the optimized circuit yields no improvements.



%% Quantum circuit optimization problem requires optimizing a quantum
%% circuit by for example improving the the number of all or some
%% selected gates, .e.g., ``CNOT'' gates and ``T'' gates.
%% %
%% Existing quantum circuit optimizers either take as input a number of
%% ``optimizing transformations'', each of which transfor a small circuit
%% to another equivalent, and more optimized circuit, or discover such
%% optimizing transformations automatically.
%% %
%% Given a set of such (optimizing) transformations, circuit optimizers
%% apply the transformations to subcircuits of a circuit, replacing each
%% subcircuit with an equivalent but more optimized one.
%% %
%% Because there are a very large, typically exponentially many, number
%% of subcircuits to consider, quantum circuit optimizers do not scale
%% beyond relatively small circuits, consisting for example of a few
%% thousand gates (even less perhaps), without of course sacrificing on
%% the quality of the overall optimization.
%% %
%% It has been not known how quantum circuit optimization may be scaled
%% to larger circuits.


%% In this paper, we propose a optimization algorithm for quantum
%% circuits that scales to large circuits.
%% %
%% Our algorithm takes an optimizer that works on ``small'' circuits
%% (e.g., tens or hundreds of gates) and a circuit to be optimized.
%% %
%% It then recursively partition the circuit into small subcircuits,
%% optimizes the small circuits with the given optimizer, and melds the
%% optimized subcircuits.
%% %
%% To ensure optimality of the resulting circuit, our meld operation
%% considers the interactions along the seam of the optimized circuits
%% being meld.
%% %
%% We prove two key properties for our algorithm:
%% %
%% 1) it guarantees \emph{local optimality}---the output circuit cannot be
%% furether optimized by applying the given optimizer to any subcircuit,
%% %
%% 2) it scalables---it works within a worst-case time bound of $O(n)$
%% where $n$ is the size of the input circuit.
%% %

%% We implement our algorithm and apply it to a number of large circuits.
%% %
%% Our experiments show that the techniques do indeed scale linearly in
%% the size of the circuit and can successfully optimize circuits with
%% many thousands of gates.
%% %
%% Compared to existing art, our techniques can result in significant
%% improvements in circuit quality by using reasonable time and compute
%% resources.


==> linearity.tex <==
\subsection{\coam{} scales linearly with the size of circuits}
\input{fig/linearity.tex}
\label{sec:linear}

We show that the \coam{} algorithm requires only linear time
by measuring its execution time across different sizes of benchmarks.
%
For this experiment, we use $\quartzt{0.06}$ as our oracle
(i.e., each sub circuit is optimized by calling \quartz{} for a duration of $0.06$ seconds).
%
We consider four quantum algorithms: Grover, VQE, QPE, and QFT,
and plot the results in \figref{linear}.
%
The Y-axis shows the execution time and the X-axis shows the size of benchmarks.
%
We vary the size of circuits by changing the number of qubits in the corresponding algorithms.

The plots show that the execution time scales linearly
across sizes ranging from a few hundreds of gates to circuits as large as $0.14$ millions
of gates.
%
For example,
in case of the VQE algorithm,
the \coam{} algorithm takes around five seconds for the smallest circuit of size two thousand,
and takes around 300 seconds for the largest circuit of size one hundred thousand ($136000$ precisely).
%
We provide the data points for our plots and the plot for the HHL family in our Supplementary.
%

==> methodology.tex <==

\label{sec:methodology}

%
% The optimizer \coamwith{\feyntool{}} optimizes for the T count of circuits
% and the optimizers \coamwith{\quartz{}}, and \coamwith{\queso{}} optimize the gate count.


% The optimizer \coamwith{\feyntool{}} runs with a default segment size $\Omega = 120$.
% This segment size delivers the best running times and circuit quality.
%
For \coamwith{\feyntool}, we choose a default segment size of $\Omega = 120$,
which we found delivers the best running times and circuit quality.
%
% In \secref{vary-segment},
% we present an experiment that considers different values of $\Omega$,
% which shows that a variety of segment sizes deliver similar output quality in comparable running times.
%
We study the impact of $\Omega$ in more detail in \secref{var-segment}, and,
in particular, observe that a variety of segment sizes deliver similar output
quality in comparable running times.
%
In \secref{comp-feyn},
we evaluate the optimizer \coamwith{\feyntool{}}
and show that it guarantees $\Omega-$optimality in short running times,
especially because \feyntool{}, being a polynomial-time optimizer,
finishes quickly for small circuits~\cite{amy2019formal}.

Unlike \feyntool{},
the \quartz{} and \queso{} optimizers require exponential time
and do not terminate quickly for small circuits.
%
For instance,
\quartz{} takes more than $24$ hours on a circuit of size $48$.
%
\queso{} takes 18 seconds to terminate on the same circuit,
and its running time increases to an hour on a circuit of size 96 (a $20\times$ increase),
which further increases to around six hours for a circuit of size 326.
%
Expecting long termination times,
both optimizers provide a timeout functionality,
enabling users to halt optimization within a timeout.

Using \quartz{} and \queso{} with \coam{},
our goal is to guarantee $\Omega-$optimality relative to a timeout,
where we can show that the optimizers cannot improve any $\Omega-$segment
of the circuit within a given amount of time.
%
To achieve this,
we run the algorithm with a timeout policy.
%
The timeout policy, parameterized by  a ``per-gate'' timeout $t$,
allows \quartz{}/\queso{} to optimize a segment $W$,
until they do not find further optimizations for $\sizeof{W}*t$ seconds.
%
When this time has elapsed,
the output segment is optimal w.r.t. \quartz{}/\queso{}, at least for $\sizeof{W}*t$ seconds.
%
The timeout policy works because once a segment is optimized under the policy,
it cannot be further optimized with the same policy,
because running the optimizers again for $\sizeof{W}*t$ seconds will not find any optimizations.
%
We use \quartzt{t} and \quesot{t} to represent the optimizers \quartz{} and \queso{}
with the timeout policy.
%
We use them to get the following guarantees.
%

We develop the optimizer \coamwith{\quartzt{t}},
which returns $\Omega-$optimal circuits relative to the optimizer $\quartzt{t}$.
%
$\Omega-$optimality relative to \quartzt{t} guarantees that running \quartz{} on
a segment $W$ of depth $\Omega$ does not discover any optimizations in time $\sizeof{W} * t$.
%
For this optimizer,
we choose the segment depth $\Omega = 6$
because (by default) \quartz{} uses
equivalence rules for circuits up to size $6$~\cite{quartz-2022}.
%
By setting the segment depth to $6$,
our optimizer feeds all segments of size $6$ to \quartz{},
giving it enough scope to discover optimizations.
%
To analyze the performance of \coamwith{\quartzt{t}},
we run it to completion on all benchmarks
and record the output quality and running time.
%
We then run vanilla \quartz{} for the same amount of time and examine
the difference in the number of optimizations.
%
\secref{comp-quartz} shows the result of this experiment with $t = 0.01s$.

% When studying the optimizers \coamwith{\quartz{}} and \coamwith{\queso{}},
% we found that they have huge running times,
% even when $\Omega$ is small
% (for $\Omega = 4$,
% we tested that \coamwith{\queso{}} runs for at least ten hours on a benchmark with $5000$ gates).
% %
% This is because both $\quartz{}$ and $\queso{}$ are exponential time algorithms
% and do not terminate quickly for small circuits.
% %
% However, both tools deliver excellent optimizations
% even when stopped early with a timeout.
% %
% To utilize their optimizations in a scalable fashion,
% we define the optimizers \quartzt{t} and \quesot{t} that implement a timeout policy.
%

The optimizer \coamwith{\quesot{t}} runs similarly
and guarantees that on any $\Omega-$segment $W$ of the output circuit,
running \queso{} for time $\sizeof{W} * t$ does not yield any optimizations.
%
We choose the segment depth to $6$, because the rules in \queso{} (for the Nam gate set),
are of size $6$ and segments of depth $6$ give \queso{} enough scope to apply its optimizations.
%
To evaluate \coamwith{\quesot{t}},
we run it to completion on all benchmarks,
recording the output quality and running time.
%
Then, we run standard \queso{} for the same amount of time on each benchmark
and study the difference in the number of optimizations.
%
\secref{comp-queso} shows the result of this experiment with $t = 0.005s$.


% \paragraph{\coam{} configurations.}
% %
% For all our experiments, we set the segment depth of \coam{} to $6$,
% i.e., $\Omega = 6$.
% %
% We choose this value because
% it aligns with the default optimization behavior of \quartz{},
% as it only focuses on sub circuits of size $6$ at any optimization step.
% %
% As described in the \quartz{} paper,
% the size $6$ is a sweet spot for it,
% since increasing this size hinders time performance,
% and decreasing it harms circuit optimizations~\cite{quartz-2022, queso-2023}.
% %
% By setting the segment depth to $6$,
% our algorithm feeds all subcircuits of size $6$ to \quartz{}
% giving it enough scope to apply its optimizations.
% %
% \footnote{We note that this size $6$ is for the Nam gate set that we use in this paper.}

% Using this segment depth, we consider three configurations
% of \coam{}, each with a different timeout for the oracle.
% %
% We choose these timeouts to cover multiple orders of magnitude for oracle
% timeouts, specifically by giving the oracle $0.01$s, $0.1$s, and
% $1$s (respectively) per unit of $\Omega$.
% %
% \begin{itemize}

% \item \coamwith{\quartzt{0.06}}
% refers to our implementation of \coam{} with \quartz{} running as oracle
% where each call to \quartz{} is capped to complete in 0.06 seconds.

% \item \coamwith{\quartzt{0.6}}: \coam{} with \quartz{} oracle,
% with upto 0.6 seconds per call.

% \item \coamwith{\quartzt{6}}: \coam{} with \quartz{} oracle,
% with upto 6 seconds per call.

% % \item \coamwith{\quesot{1}} refers to our implementation of \coam{} with \queso{} running
% % as oracle where each call to \queso{} is capped to complete in 1 second.
% % \footnote{1 second is the minimum timeout \queso{} supports.}
% \end{itemize}

% We note that our integration with \quartz{}
% introduces overhead to the running time
% of our algorithm
% because each call to \quartz{} changes the circuit representation
% and also pays for the initialization cost of \quartz{}.
% %
% To mitigate this overhead,
% we send subcircuits of size $10*\Omega*n$ to \quartz{},
% instead of the size $2*\Omega*n$ described in the algorithm,
% where $\Omega$ represents \coam{}'s parameter and $n$ is the
% number of qubits.
% %
% By sending larger circuits to \quartz{},
% we ensure that the overhead does not dominate
% the time to execute one function call to \quartz{}.
% %
% %This reduces the number of calls and thus reduces the cross-language
% %overhead.
% %
% When the per call timeout is larger (i.e, 0.6 seconds, or 6 seconds),
% we send subcircuits of
% size $2*\Omega*n$.

% We also cache the rules used by quartz to reduce this overhead.
% \ur{I did not understand the last sentence with 2Omega.}

% \jr{revisit}



% The \queso{} optimizer~\cite{queso-2023}, which is written in Java, does
% not naturally
% %
% We therefore integrate \queso{} via the operating system.
% %
% Specifically, to invoke \queso{} on a subcircuit, our \coam{}
% implementation writes the QASM representation to a file and
% calls \queso{} by using a system call.
% %
% This system call, in turn, writes its output to another file, which
% our \coam{} implementation reads.
% %
% Because the overhead is large and difficult amortize by increasing
% subcircuit sizes, our integration with \queso{} incurs significant
% overhead.
% %
% Nevertheless, this integration demonstrates the feasibility of
% integrating with existing optimizers either through cross-language
% interoperability features (when feasible) or through systems calls.
% %

% For this reasons, we compare with \queso{} only on a few benchmarks.
%
% \ur{This last sentence does not sound right.  It can be interpreted as ``the results were not good, so we are not showing you everything'' }

%% We then run vanilla \quartz{} on the whole circuit
%% for the same end-to-end time as our algorithm
%% and compare the circuit quality.
%% %
%% We perform this experiment with three different timeouts ($t = 0.06$s, $0.6$s, $6$s),
%% each of which increases the end-to-end running time ten fold.
%






==> model.tex <==
\label{sec:model}

% For optimizers that are unable to scale for large circuits,
% it means that any improvements beyond $\Omega-$optimality
% would come with a steep cost to the running time of circuit optimization


% $\Omega-$optimality is a good quality target
% because it implies that there are no easy optimizations left.
% %
% Any improvements beyond $\Omega-$optimality
% would come with a steep cost to the running time of circuit optimization.
% %

We describe the quantum circuit model that we assume throughout the
paper and define two local optimality properties on this model.
%
The properties capture the intuitive notion that many
optimizations involve gates that are closely positioned in a quantum
circuit, e.g., an optimization may replace a small subcircuit of 10
gates with a circuit with 4 gates.

\myparagraph{Circuit Model.}
We model a circuit $C = \langle L_0, L_2, \ldots L_{d-1}\rangle$ as a
sequence of layers $L_i$, where each layer contains a (non-empty) set
of gates that operate on disjoint qubits.
%
In this model, we can split and concatenate circuits by splitting and
concatenating the underlying layer sequences.
%
We define the \defn{depth} of a circuit as the number of layers
and the \defn{size} of a circuit $C$, denoted $|C|$, as the total number of gates.
% Our algorithm optimizes the circuit at the granularity of
% subcircuits we call \emph{segments}.
%
A \defn{segment} is a contiguous subsequence of layers of the circuit.
%
We use the python style notation $C[i : j]$ to represent a segment containing
layers  $L_i\dots L_{j - 1}$ from circuit $C$.
%
The depth of a segment is the number of layers and its size is the cumulative
gate count across those layers.
%
%
We define a $\boldsymbol{k}$\defn{-segment} as a segment of depth $k$.
%
Note that the size of a $k$-segment is at most $k \cdot n$,
where $n$ is the number of qubits in the circuit.

%
To define local optimality, we use the number of layers, or depth, as
the notion of distance for locality.
%
Specifically, we say that a circuit is locally optimal with respect to
a cost, if all segments of the circuit smaller than a desired depth
are optimal with respect to that cost.
%
%% \ur{Might want to add something about vertical but could also hold
%%   off: we allow all qubits to interact because this is common. }

\begin{definition}[Local Optimality]
  A circuit is \defn{$\boldsymbol{\mathit{\Omega}}$-optimal} with
  respect to a given cost function when every segment of depth less than or equal to
  $\Omega$ is optimal with respect to that cost.
\end{definition}

Though easier than global optimality,
achieving local optimality could also be difficult because producing the best circuit
for a given $\Omega-$segment can still be expensive.
%
Thus, it is more practical to define a relaxed, ``relative''
local optimality notion that does not insist on full optimality of the subcircuits,
and instead, requires each such subcircuit to be optimal relative to
a given oracle optimizer.
%

% \myparagraph{$\boldsymbol{\Omega}$-optimality.}
% Given an input circuit $C = \langle L_1, L_2, \ldots L_d\rangle$,
% the algorithm returns an optimized circuit $C'$ represented as
% $\langle L'_1, L'_2, \ldots L'_{d'}\rangle$.
% %
% This optimized circuit satisfies two properties:
% (1) the number of layers $d'$ in circuit $C'$ is bounded by the number of layers
% $d$ in circuit $C$,
% and
% (2) $C'$ is $\Omega$-optimal, according to the following definition.
%
\begin{definition}[Relative Local Optimality]
  A circuit is \defn{$\boldsymbol{\mathit{\Omega}}$-optimal}
  \defn{relative} to an oracle optimizer if the oracle can not improve
  any segment of depth $\Omega$ or smaller.
\end{definition}

\input{fig/fig-overlap}

To illustrate the definition of local optimality,
\figref{overlap} shows a circuit in the layer representation.
%
The figure defines an $\Omega-$segment $W_i = C[i:i + \Omega]$,
starting at layer $i$ and including $\Omega$ layers from
$i$ to $i + \Omega - 1$.
%
If all segments $W_i$ for $0 \leq i \leq D - \Omega$ are optimal relative to the oracle,
then the circuit is $\Omega-$optimal.
%
We can therefore verify if the circuit $C$ is $\Omega$-optimal by
checking that each of the at most $(D - \Omega + 1)$ segments is optimal
by using an oracle for relative optimality.
%



The notion of relative local optimality is practical,
as it defines a quality criterion that can be used with many existing optimizers.
%
When an optimizer does not scale to large circuits,
we can use relative $\Omega-$optimality as the goal of optimization.



\myparagraph{A Lower Bound on Local Optimality.}
%
This leaves open the question of whether there is a general purpose algorithm for local
optimality that works for all oracles
and whether such an algorithm could be practical.
%
We prove a lower bound stating that such an algorithm would
require at least linear time in the size of the circuit.

\begin{theorem}[Local Optimality Requires Linear Time]
  Consider a circuit $C$ over $n$ qubits with depth $D$ and a cost
  function.  for any $\Omega > 1$ and $D > 1$, finding a circuit that
  is equivalent to $C$ but that is $\Omega$- optimal with respect to
  the cost function requires $\bigomega(|C|)$, i.e., linear time in
  the size of the circuit.
\end{theorem}
\begin{proof}
Consider any gate in the circuit $C$, because $\Omega > 1$ and $D >
1$, this gate is part of at least one $\Omega$-segment and the segment
might be suboptimal, e.g., if the gate is before/after a
gate in the segment that is its inverse.
%
An algorithm guaranteeing local optimality
must therefore check each gate and possibly the gates
that are nearby that gate.
%
Because checking a gate requires constant time, any algorithm that
guarantees local optimality requires linear time in the size of the
circuit.
\end{proof}

% Our goal is to design an algorithm that produces circuits that satisfy local optimality
% relative to existing practical optimizers.

% For a given fixed, $\Omega$, and family of circuits whose number of
% qubits are bounded by a constant, running the optimization on
% $\Omega$-depth circuits takes constant time asymptotically.
% %
% Because each verification call takes constant time and there are a
% polynomial number of calls that require verification, the local
% optimality problem is in NP for circuits with constant number of
% qubits.
% %
% A similar argument applies to oracle optimizers and the relative local
% optimality problem is also in NP for circuits with constant number of
% qubits.
% %
% (Recall that, in contrast, circuit optimization problem is QMA-hard.)






%% Because optimizing large segments/circuits is a challenging problem,
%% improving an $\Omega-$optimal circuit incurs a steep cost to the running time,
%% making $\Omega-$optimality a good quality goal.
%% %
%% $\Omega-$optimality implies that all optimizations that are relatively easy
%% for a given optimizer have been performed.
%% %
%% Our goal is to achieve $\Omega-$optimality by using the oracle on small segments.
%% %
%% We assume the following about the oracle.
%% % specifically we invoke the oracle on a circuit only if its contained within a segment of depth $2\Omega$.
%% %
%% % This way, the size of an oracle query is bounded by $2n\Omega$ gates for $n$ qubits.


%% %
%% Relative $\Omega-$optimality guarantees that all $\Omega-$segments
%% of a circuit are optimal w.r.t. an oracle optimizer.
%% %
%% The number of $\Omega-$segments in a circuit of depth $d$ is $(d - \Omega + 1)$.
%% %
%% By guaranteeing that all $\Omega$-segments are optimal, relative
%% $\Omega$-optimality ensures that the only way for the optimizer to
%% improve the circuit further is to consider large segments (of depth
%% greater than $\Omega$).
%% %
%% Because optimizing large segments/circuits is a challenging problem,
%% improving an $\Omega-$optimal circuit incurs a steep cost to the running time,
%% making $\Omega-$optimality a good quality goal.
%% %
%% $\Omega-$optimality implies that all optimizations that are relatively easy
%% for a given optimizer have been performed.
%% %
%% Our goal is to achieve $\Omega-$optimality by using the oracle on small segments.
%% %
%% We assume the following about the oracle.
%% % specifically we invoke the oracle on a circuit only if its contained within a segment of depth $2\Omega$.
%% %
%% % This way, the size of an oracle query is bounded by $2n\Omega$ gates for $n$ qubits.



%

% As illustrated in \figref{overlap},
% this covering guarantees that every $\Omega$-segment is contained within some $2\Omega$-segment.
% %
% If the oracle does not improve any $2\Omega$-segment,
% then the oracle has certified all $\Omega-$segments to be optimal
% and the circuit is $\Omega$-optimal.
% %
% Since the number of $2\Omega$-segments is bounded by circuit size,
% the time cost of checking $\Omega$-optimality is bounded by the circuit size.
% %
% In the next subsection,
% we describe the \coam{} algorithm that in fact
% achieves $\Omega-$optimality in linear time.
% %

% Given a circuit,
% we can verify if it is $\Omega-$optimal
% by covering the circuit in many overlapping $2\Omega$-segments and querying
% the oracle on each such segment.
% %
% %

% %




% the time cost of the algorithm for checking $\Omega-$optimality
% is linear in circuit size because the number of oracle calls is bounded by circuit size.
%

%


\myparagraph{Additive Cost Functions.}
Our definitions of local optimality and relative local optimality make
no assumptions on the cost function.
%
In the rest of the paper, we focus our attention on cost functions
that map circuits to natural numbers.
%
Most interesting cost functions satisfy this constraint, e.g., the
total number of gates in a circuit, total weight of the gates where
weight could denote some property such as the time units needed for
that gate, or the depth of the circuit, etc.
%
If costs are not natural numbers, we can scale them (by additing and
multiplying with appropriately chosen constants) to obtain natural
numbers.

In our algorithm for computing local optimality, we assume that cost
functions are additive under circuit concatenation.
%
\begin{definition}[Additive Cost Functions]
\label{def:additive-cost}

We say that a cost function $\kwcost{\cdot}$ from circuits to costs is
additive if the function maps circuits to positive natural numbers
such that the cost of the concatenation of any two circuits $C_1$ and
$C_2$ is equal to the cost of individual circuits, i.e.,
\[
\kwcost{\circuitcon{C_1}{C_2}} = \kwcost{C_1} +  \kwcost{C_2}.
\]
\end{definition}


%% We assume that the cost function that is additive w.r.t.
%% circuit concatenation,
%% i.e., for any circuits $C_1$ and $C_2$,
%% $\costof{\lstinline{concat}(C_1, C_2)} = \costof{C_1} + \costof{C_2}$.
%% %
%% For simplicity, we assume that the cost function computes integer costs.
%% %
%% Most practical cost functions can be multiplied by a large constant
%% to approximate fractional costs.

%% In our model, one way to achieve $\Omega-$optimality is by
%% improving the $\Omega$-segments of a circuit using the oracle
%% and repeating until we reach a fixed point where all of them are optimal.
%% %
%% The repetitions can only occur $\costof{C}$ times because each oracle optimization
%% reduces the cost function by at least one (the cost function is integer valued).
%% %
%% Because the maximum number of repetitions is $\costof{C}$
%% and each repetition can use the oracle at most $\sizeof{C}$ times,
%% we can achieve $\Omega$-optimality within $\sizeof {C} * \costof{C}$ calls to the oracle.
%% %
%% In contrast, the SOAM algorithm achieves $\Omega$-optimality in $O(\sizeof{C} + \costof{C})$ calls
%% by carefully tracking optimal segments and propagating the optimizations among them.


%

% because a segment of with $2 \cdot \Omega$ can only contain that many gates.
%




% Our algorithm's time complexity and quality assurance rely on two assumptions.
% %
% For the time complexity,
% we assume that the oracle takes constant time to optimize its input.
% %
% The assumption is realistic because the the algorithm only invokes the oracle on fixed-depth segments,
% thereby establishing an upper bound on the circuit size processed by the oracle.
% %
% For our quality guarantee, we assume that the oracle does not increase the
% size of the its input (i.e., it optimizes gate-count), and similarly does not
% increase the depth of its input.
% %
% Formally, for an input circuit $C$, if the oracle outputs circuit $C'$,
% then $|C'| \leq |C|$ and $\textit{depth}(C') \leq \textit{depth}(C)$.

% To facilitate split and meld operations on the circuit,
% the algorithm represents a circuit $C = \langle L_1, L_2, \ldots L_d\rangle$ as a sequence of
% layers $L_i$, where each layer contains a set of gates that operate on disjoint qubits.
% %
% In this representation,
% the algorithm can split and concatenate circuits
% by splitting and concatenating the underlying layer sequences.
% %
% Empty layers are deleted.
% %
% We define the \defn{depth} of a circuit as the number of layers
% and the \defn{size} of a circuit $C$, denoted $|C|$, as the total number of gates.
% %

% %
% We define a \defn{segment} as a contiguous subsequence of layers.
% %
% The \defn{width} of a segment is the number of layers, and the
% \defn{size} of a (sub)circuit $C$, denoted $|C|$, is the total number of gates,
% i.e., $|C| = \sum_i |L_i|$.








% Note that we can check $\Omega$-optimality in linear time,
% i.e., in $O(\sizeof{C})$ time,
% by covering the circuit in many overlapping $2\Omega$-segments and querying
% the oracle on each such segment.
% %
% As illustrated in \figref{overlap},
% this covering guarantees that every $\Omega$-segment is contained within some $2\Omega$-segment.
% %
% If the oracle does not improve any $2\Omega$-segment,
% then the oracle has certified all $\Omega-$segments to be optimal
% and the circuit is $\Omega$-optimal.
% %
% %
% It is also easy to create an $\Omega$-optimal circuit in $O(\sizeof {C} * \costof{C})$ time,
% by repeatedly calling the oracle on all $2\Omega$-segments
% until we reach a fixed point where there are no segments optimized.
% %
% This repetition can only occur $\sizeof{C}$ times because each one reduces the gate count by at least one,
% thereby reaching the fixed point in $O(\sizeof {C} * \costof{C})$ time.
% %

% In contrast, the SOAM algorithm achieves $\Omega$-optimality in $O(\sizeof{C} + \costof{C})$ time
% by carefully propagating the optimizations among segments.



==> oracle.tex <==
Researchers have proposed many techniques for optimizing quantum circuits,


To optimize quantum circuits,
researchers have proposed substitution-based algorithms,
algorithms that substitute components of a circuit with equivalent components, reducing the size of the circuit.
%
Many such algorithms rely on a partial function
that maps circuits to equivalent circuits.
%
The algorithms apply the partial function to the original circuit by
identifying a sub circuit which is in the domain of the partial function
and substituting the sub circuit with the corresponding value of that function.
%
The partial function is applied repeatedly,
until the function is exhausted,
or a terminating condition (defined by ad-hoc heuristics) is satisfied.
%
We refer to such algorithms as \defn{substitution oracles},
and call the corresponding partial function \defn{transformer}.
%
Formally,
an oracle $\mathcal{O}$ takes a circuit $\mathsf{C}$, a transformer $\mathsf{t}$,
and returns a sub circuit $\mathsf{C}'$ such that $\mathsf{C}' = \mathcal{O}(\mathsf{t}, \mathsf{C})$.


The main problem with oracles that have been designed is
that they scale poorly with the size of the circuit.
%
Each time....


We define the \defn{width} of a transformer $\mathsf{t}$,
denoted as $\Omega(\mathsf{t})$, as
the maximum size of the circuit in the domain of the transformer.
%
We say that a transformer is $\defn{greedy}$ if it always maps a circuit to a smaller circuit.
%

Given a greedy transformer $\mathsf{t}$ and oracle $\mathcal{O}$,
we design an algorithm that makes a \emph{succinct} number of \emph{precise} calls to the oracle,
and transforms a circuit $\mathsf{C}$ to another circuit $\mathsf{C'}$ such that it is optimal w.r.t.
the oracle and the transformer, i.e, $\mathcal{O}(t, \mathsf{C'}) = \mathsf{C'}$.
%
To achieve this,
our algorithm uses the oracle on circuits of size $O(\Omega(t))$,
and only makes $O(\lvert\mathsf{C}\rvert  + k)$ calls to the oracle,
where $k$ is the number of optimizations ($\lvert\mathsf{C}\rvert - \lvert\mathsf{C'}\rvert$).
%
Crucially, the number of calls to the oracle scales linearly with the size of the circuit
and the number of optimizations.



==> plots_greedy.tex <==
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.4\linewidth]{plots/gf.greedyscatter.png }\quad
	\includegraphics[width=0.4\linewidth]{plots/hhl.greedyscatter.png}\quad
\caption{Time vs. Size plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.4\linewidth]{plots/qft.greedyscatter.png}\quad
	\includegraphics[width=0.4\linewidth]{plots/vqe.greedyscatter.png}
\caption{Time vs. Size plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.4\linewidth]{plots/grover.greedyscatter.png}\quad
	\includegraphics[width=0.4\linewidth]{plots/qaoa.greedyscatter.png}\quad
\caption{Time vs. Size plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.4\linewidth]{plots/shor.greedyscatter.png}
\caption{Time vs. Size plots}
\end{figure*}


==> plots_greedy_cliff.tex <==
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.4\linewidth]{plots/gf.greedyscatter.clifft.png }\quad
\caption{Time vs. Size plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.4\linewidth]{plots/qft.greedyscatter.clifft.png}\quad
	\includegraphics[width=0.4\linewidth]{plots/vqe.greedyscatter.clifft.png}
\caption{Time vs. Size plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.4\linewidth]{plots/grover.greedyscatter.clifft.png}\quad
	\includegraphics[width=0.4\linewidth]{plots/qaoa.greedyscatter.clifft.png}\quad
\caption{Time vs. Size plots}
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.4\linewidth]{plots/shor.greedyscatter.clifft.png}
\caption{Time vs. Size plots}
\end{figure*}



==> stretch-eval.tex <==
\section{\queso{} comparison}


%





% %
% We integrate the \queso{} optimizer into our algorithm as an oracle
% and impose a one second time out for each call.
% %
% We note that \queso{} does not follow the given timeout strictly
% and often takes longer to run and return the result (around $4/5$ seconds per call).

% To evaluate the algorithm,
% we run it with \queso{} and compute the final circuit
% and the overall execution time, excluding time for file I/O (\secref{impl}).
% %
% Then, we execute default \queso{} on the whole circuit for the same total runtime
% and compare the quality of circuits produced.
% %
% For this experiment,
% we filter benchmarks based on their sizes and
% opt for benchmarks whose sizes are less than ten thousand gates.
% %
% This size limitation arises from file I/O overheads which make restrict our ability
% to run larger circuits within reasonable times.

% \figref{comp-queso} shows the results of the evaluation for seven benchmarks
% coming from four families of algorithms.
% %
% The ``QS'' column denotes \queso{} and the ``S'' column represents the \coam{} algorithm
% using \queso{} as the oracle.
% %
% In all cases, the \coam{} approach generates smaller circuits than the baseline \queso{}.
% %
% Similar to the case with \quartz{} (\secref{quartz}),
% we observe that the gap between the \coam{} approach and default \queso{} increases
% with circuit size.
% %
% Foe example,
% in the grover family,
% the ratio of optimization rate between \coam{} and \queso{}
% increases from $1.14$x for grover\_n7 to $1.4$x in grover\_n9.
% %
% For the circuit vqe\_n12,
% which is the largest circuit on the table,
% the final circuit size is $0.78$ times smaller compared to \queso{},
% which demonstrates the scalability of the \coam{} approach.
% %
% On average,
% the algorithm's circuits are $0.92$x smaller than those generated by \queso{}
% and the algorithm makes $1.27$x as many optimizations per second.
% %

\begin{figure*}
  \centering
  \input{fig/prelimqueso.0.01.tex}
  \caption{The figure compares the performance of $\coamt{\quartzt{0.06}}$ against standard \queso{}.
  The label ``S'' represents $\coamt{\quartzt{0.06}}$ and the label ``QS'' represents \queso{}.
  %
  The figure compares the circuit sizes (lower is better) and the optimization rates (higher is better) of both approaches.
  %
  The optimization rate measures the number of optimizations performed per second of execution.
  %
  The figure also shows the improvement factor $QS/S$ for circuit size and $S/QS$ for optimization rate,
  quantifying the improvement achieved by \coam{}.
  %
  The Time column takes the time it takes to run both of them.
  %
  \queso{} sometimes runs longer because its timeout functionality is not very precise.
  %
  }
  \label{fig:comp-low-queso}
\end{figure*}



In this section,
we compare the circuit quality by the \coam{} algorithm with configurations \coamwith{\quartzt{0.06}}
and \coamwith{\quartzt{0.6}} against the standard \queso{} optimizer.
%
Our methodology is the same,
for each configuration we take the running time,
and then execute \queso{} with the same running time.
%

We note that even though \queso{} implements a timeout facility,
it does not adhere to it.
%
We observed that the tool takes an unpredictable amount of time
taking as much as $200$x the given timeout.
%
To address this,
we changed the code in \queso{}, making it check timeouts more eagerly.
%
Though our changes reduced the unpredictability,
there is some difference in the running time with \queso{} running
longer than our algorithm.
%
We note that our algorithm never runs for a larger time.
%

\figref{comp-low-queso} compares the configuration \coamwith{\quartzt{0.06}}
with \queso{}, when given the same timeout.
%
We observe that in three cases \queso{} generates a better quality circuit,
but it also takes more time.
%
In twelve cases, our algorithm generates better quality circuits,
and these cases correspond to larger sized circuits,
showcasing the scalability benefits of our approach.
%
On average, our algorithm generates smaller circuits by a factor of $1.18$x
and its average optimization rate is $5$x compared to \queso{}.
%

\figref{comp-med-queso} similarly compares the configuration  \coamwith{\quartzt{0.06}}.




\begin{figure*}
  \centering
  \input{fig/prelimqueso.0.1.tex}
  \caption{The figure compares the performance of $\coamt{\quartzt{0.6}}$ against standard \queso{}.
  The label ``S'' represents $\coamt{\quartzt{0.06}}$ and the label ``QS'' represents \queso{}.
  %
  The figure compares the circuit sizes (lower is better) and the optimization rates (higher is better) of both approaches.
  %
  The optimization rate measures the number of optimizations performed per second of execution.
  %
  The figure also shows the improvement factor $QS/S$ for circuit size and $S/QS$ for optimization rate,
  quantifying the improvement achieved by \coam{}.
  %
  The Time column takes the time it takes to run both of them.
  %
  \queso{} sometimes runs longer because its timeout functionality is not very precise.
  %
  }
  \label{fig:comp-med-queso}
\end{figure*}

